Navigating the Kaleidoscope of COVID-19 Misinformation Using Deep Learning

Irrespective of the success of the deep learning-based mixed-domain transfer learning approach for solving various Natural Language Processing tasks, it does not lend a generalizable solution for detecting misinformation from COVID-19 social media data. Due to the inherent complexity of this type of data, caused by its dynamic (context evolves rapidly), nuanced (misinformation types are often ambiguous), and diverse (skewed, fine-grained, and overlapping categories) nature, it is imperative for an effective model to capture both the local and global context of the target domain. By conducting a systematic investigation, we show that: (i) the deep Transformer-based pre-trained models, utilized via the mixed-domain transfer learning, are only good at capturing the local context, thus exhibits poor generalization, and (ii) a combination of shallow network-based domain-specific models and convolutional neural networks can efficiently extract local as well as global context directly from the target data in a hierarchical fashion, enabling it to offer a more generalizable solution.

==> 2.LiteratureSurvey.tex <==
\section{Literature Survey} 

% a) ML based health misinformation and Covid misinformation detection approaches 

  

% - Shahi 2020 (FakeCovid) 

  

% - Cui 2020 (CoAID) 

  

% - Hossain 2020 (CovidLies) 

  

% and other covid related papers that you studied. 

  

  

% b) NLP methods 

  

% Review all NLP papers that you studied. Don't miss any 

  

% include this: 

% Lu-2020-VGCN-BERT- Augmenting BERT with Graph Embedding for Text Classification 

  

  

% For each paper address the following: 

  

% - Brief summary of the paper  

  

% - Main limitation in solving the covid misinformation classification problem 

  

% - Wherever possible connect the current paper to the next paper 

In this chapter, we discuss the Machine Learning (ML) based main research approaches for detecting misinformation on social media related to health and COVID-19.  

  

The ML approaches involve two steps: creating text embedding and performing supervised classification. Specifically, text embeddings are created using NLP techniques, then a supervised classifier is used to detect misinformation data. Importantly, much of the effort in misinformation detection is invested in creating the labeled dataset. 


Below we describe the main papers that contribute towards labeled dataset creation, text embedding, and supervised classification. 

  

\subsection{Health Misinformation} 

  

% - Kinsora's main contribution is to create a labeled dataset for general health misinformation. 

  

As aforementioned, the COVID-19 causes an `infodemic' which draws many researchers' attentions to exploring methods that can effectively detect COVID-19 related misinformation. Before the COVID-19 virus appears, however, there are already many ML-based types of researches that have been conducted for health misinformation detection. It is also noteworthy that the quality of a dataset used for misinformation detection is quite important. Particularly, Kinsora et al.\cite{Kinsora:2017} develops a small labeled dataset that contains misinformative posts collected from a medical forum, and it also includes other features other than the content of posts, which are proven to be useful for improving detection accuracy in their study. Their dataset is useful for studying general health misinformation, but it is not applicable to be used for classifying a dataset that contains texts about newly discovered diseases (i.e., COVID-19). Besides, it is easier to label general health misinformation posts since there existed many experts who have conducted comprehensive studies on diseases or viruses that have been discovered before.  

  

\subsection{COVID-19 Misinformation} 

  

For COVID-19 misinformation, creating a labeled dataset is significantly more challenging. Due to the diversity of misinformation and the speed of its evolution, it is a tall task for the experts to label data correctly. 

  

Hossain et al. \cite{hossain-etal-2020-covidlies} build a dataset called COVIDLIES that contains COVID-19 related tweets, which are collected from March to April 2020 and categorized as Agree, Disagree, and No Stance. Each tweet is also paired with a known misconception that is extracted manually from Wikipedia COVID-19 related articles. A label of a tweet is Agree if it agrees with the misconception, Disagree if it disagrees with the misconception, and No Stance if it expresses no stance to the misconception. Another dataset created by Shahi et al.\cite{shahifakecovid} is a multilingual dataset named FakeCovid, which only contains news articles collected from 04/01/2020 to 15/05/2020. This dataset contains a total of 5128 articles written in 40 different languages, and only 40.8\% of articles are in the English language.  

  

For both COVIDLIES and FakeCovid datasets, one of their limitations is that they only contain one type of data source, where COVIDLIES is built based on tweets and FakeCovid is based on news articles. Another limitation is that both datasets only include a month of data, which is not sufficient to detect COVID-19 misinformation due to the fact that the words used related to COVID-19 are changed from time to time. Therefore, another comprehensive COVID-19 dataset is created by Cui et al.\cite{cui2020coaid} called CoAID. It contains COVID-19 related tweets, replies, news articles, and ground truth labels. The tweets consist of two parts: news-related tweets and claims of tweets, and tweet replies under those tweets or news articles. The dataset also includes four different months of data. See more details in section \ref{coaid}. However, compared to FakeCovid, the content of CoAID and COVIDLIES datasets is not preprocessed, and the sizes are reduced since some tweets cannot be retrieved because they are deleted or unauthorized to fetch during the collecting process.  



The above datasets are used to train Supervised classifiers (i.e., Support Vector Machine or Logistic Regression) by authors, but the classifiers require the text data to be embedded. Therefore, NLP techniques are used to embed text data. 

  

\subsection{Text Embedding Techniques and Classification} 

  

% - Word2Vec and GloVe: text embedding 

  

% - BERT and its variants: text embedding and classification 

  

% - Text GCN: text embedding and classification 

  

The NLP techniques are being widely used in creating text embeddings. In 2013, Mikolov et al.\cite{mikolov2013efficient} introduces Word2Vec models that can produce high-quality representations of words, which are CBOW and Skip-gram model. The difference between CBOW and Skip-gram model is that CBOW uses context to predict the current word, while Skip-gram uses the current word to predict surrounding words. In 2014, another word representation called GloVe is created by Pennington et al.\cite{pennington-etal-2014-glove}, which is different from Word2Vec models since GloVe uses count-based methods while Word2Vec models are prediction-based methods. In other words, word representations of GloVe are based on global word-word co-occurrence counts, while Word2Vec tries to capture co-occurrence one window at a time.  

  

Both Word2Vec and GloVe methods can capture semantic and syntactic relationships of a language. However, they are unable to carry contextual information. Hence, in recent years, new word representation techniques are being developed so that contextual information can be captured. The ELMo created by Peters et al.\cite{peters2018deep} is one of the techniques that can capture the contextual relationship. It uses a bidirectional language model (biLSTM), where the states from higher-level LSTM can capture word meaning and lower-level LSTM can capture syntax. The combination of both states generated from high and lower-level LSTM is the final rich word representation. Meanwhile, another state-of-the-art technique named BERT was invented by Devlin et al.\cite{devlin2019bert}, which uses transformers techniques. More details about transformers are provided in the following section \ref{bert}. BERT model shows that transfer learning using pretrained model can be fine-tuned to obtain decent performances for different downstream tasks. However, BERT model is limited to capturing global information. Therefore, a new method called Text GCN is developed by Yao et al.\cite{yao2018graph} that can capture high-order neighborhood information because it can explicitly model global word co-occurrence. It is different from other GCN models because it produces a heterogeneous graph where documents and words are nodes. Its limitation is that it could not train using the unlabeled dataset, fast generate embeddings and predict for unseen documents\cite{yao2018graph}. 

  

Additionally, there are many other methods developed based on BERT to obtain better performance. Specifically, Liu et al.\cite{liu2019roberta} creates a better recipe for training BERT, which is called RoBERTa. There are four modifications made to improve BERT, which are: longer training time with more data; no next sentence prediction; longer sequences are used for training; and using dynamic masking technique. Therefore, RoBERTa requires more data and time for training. Another variant of BERT is called ALBERT created by Lan et al.\cite{lan2020albert}, which utilizes two parameter-reduction techniques that can address the memory limitation issues. The two parameter-reduction techniques are a factorized embedding parameterization and cross-layer parameter sharing. See more details in Section \ref{albert}.  

  

% Transformers have a potential of learning longer-term dependency, but are limited by a fixed-length context in the setting of language modeling. the model lacks necessary contextual information needed to well predict the first few symbols, leading to inefficient optimization and inferior performance. 

  

% As a consequence of the fixed context length, the model cannot capture any longer-term dependency beyond the predefined context length.  

  

%In addition, the fixed-length segments are created by selecting a consecutive chunk of symbols without respecting the sentence or any other semantic boundary. 

  

% Transformer-XL that enables learning dependency beyond a fixed length without disrupting temporal coherence. 

%we introduce a simple but more effective relative positional encoding formulation that generalizes to attention lengths longer than the one observed during training. 

In the meantime, there are researches focusing on improving the Transformer\cite{attention}. Specifically, the transformer-based language modeling (e.g., BERT) has a fixed-length length context setting, which creates fixed-length segments by selecting a consecutive set of symbols without considering the whole sentence or semantic boundary \cite{dai2019transformerxl}. This setting makes the model unable to obtain longer-term dependency that can cause inefficient optimization and poorer performance\cite{dai2019transformerxl}. In 2019, a new Transformer called Transformer-XL (Transformer-Extra Long) is created by Dai et al.\cite{dai2019transformerxl} which can learn longer-term dependency without damaging the temporal coherence and they also create a relative positional encoding scheme that helps solve the fixed-length context issue. In 2020, a Transformer-XL based model called XLNet is developed by Yang et al.\cite{yang2020xlnet}, which is a generalized autoregressive (AR) pretraining method. It combines the advantage of AR models and BERT and avoids their weaknesses. For instance, AR language modeling does not suffer from input noise, while BERT can better capture bidirectional context. Moreover, XLNet utilizes the techniques from Transformer-XL (e.g., relative positional encoding) to improve the performance for pretraining.  

These variants of BERT model made an improvement in different aspects of BERT. However, they do not address the issue that BERT is limited to capturing global information. A model called VGCN-BERT is created by Lu et al.\cite{lu2020vgcnbert} that integrates GCN into BERT, which combines the advantages of BERT and GCN to create an enriched representation of words for classification. VGCN-BERT model uses multiple layers of attention mechanism on a graph word embedding, which is built based on word embedding and vocabulary graph. The word embedding and vocabulary graph embedding is concatenated if they have a high semantic correlation. The limitation of VGCN-BERT model is that it only accepts lexical relations (i.e., vocabulary graph) of a language. 

  

\subsection{Model Description}  

  

\begin{itemize} 

   

\item Word2Vec 

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/word2vec-architectures.png} 

  \caption{Left is CBOW Architecture and Right is Ski-gram Model Architecture. \cite{mikolov2013efficient}} 

  \label{fig:w2v} 

\end{figure} 

  

The Word2Vec is an algorithm that takes text corpus as inputs and outputs vector representations of each word that contains semantic and syntactic relationships between each word. There are two different architectures based on Word2Vec, which are CBOW (continuous bag-of-words) model and Skip-gram (continuous skip-gram) model. Figure \ref{fig:w2v} shows architectures of CBOW and Ski-gram. It is obvious to observe the difference between CBOW and Skip-gram, in which the CBOW model combines the continuous distributed representations of context to predict the current word, while the Skip-gram model creates the distributed representation of the current word to predict its surrounding words. For example, if the training input is ‘I like trees’, then CBOW model creates vector representations of the context ‘I’ and ‘trees’ to predict the current word ‘like’, while Skip-gram model creates vector representation of the current word ‘like’ to predict the context ‘I’ and ‘trees’.  

  

In addition, the distance between the current word and predicted word within a sentence is a hyperparameter called window size. In other words, if the window size is larger, more neighbor words of the current word will be taken into account during training. For instance, if the training input is ‘I am eating apples and bananas now’ and the current word is ‘apples’, and the window size is 2, then the context of the current word is [eating, and]. If the window size is 4, then the context is [am, eating, and, bananas]. A larger window size will increase the training time.  

  

\item GloVe  

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/Glove-architecture.png} 

  \caption{The Architecture of GloVe Model. \cite{liu_zhang_li_yan_2019}} 

  \label{fig:glove} 

\end{figure} 

  

  

Another model that can capture semantic and syntactic relationships is the GloVe model. GloVe is an unsupervised learning algorithm that can produce a word vector space with a meaningful substructure by training on aggregated global word-word co-occurrence counts \cite{pennington-etal-2014-glove}. 

  

The GloVe model is different from other models that also use the statistic of word occurrences because of its weighted least squares regression with the new cost functions, which can address the problem of rare co-occurrences that are noisy and carry less information.  

  

The cost function \cite{pennington-etal-2014-glove} looks as follows:  

  

$J = \sum_{i,j=1}^{V} f(X_{ij})(w^T_i \tilde{w} + b_i + \tilde{b_j} - log{X_{i,j}})^2$, 

  

%where X is the word-word co-occurrence counts, $X_{i,j}$ is the number of times that word j appears in the context of word I, V is the size of vocabulary of a corpus, $b$ and $\tilde{b}$ are biases, $w \in \mathbb{R}^d$ are word vectors, and $\tilde{w} \in \mathbb{R}^d$ are context word vectors. The difference between $w$ and $\tilde{w}$ is their random initializations.  

  

This weighting function also has the following properties: 

\begin{enumerate} 

  \item $f(0)=0.$ If f is viewed as a continuous function, $lim_{x\rightarrow0}f(x)log^2x$ is finite. 

  \item $f(x)$ should be non-decreasing in order to avoid that rare co-occurrences are overweighted. 

  \item $f(x)$ should be relatively small for large value of x, in order to avoid that frequent co-occurrences are overweighted.  

\end{enumerate} 

  

The following $f(x)$ usually works well: 

  

%$ 
%
%f(x)= \begin{cases} 
%
%(x/x_max)^\alpha, & x > x_max \\ 
%
%1, & otherwise 
%
%\end{cases} 
%
%$ 

  

Figure \ref{fig:glove} shows the architecture of the GloVe model. Specifically, the GloVe model takes one-hot representations of words as input and uses word embedding matrices as weighted matrices to output vectors that are inner products of word vectors.  

  

\item ELMo 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/ELMo_architecture.png} 

  \caption{The Architecture of ELMo Model. \cite{devlin2019bert}} 

  \label{fig:elmo} 

\end{figure} 

  

ELMo stands for Embeddings from Language Models, which is a bidirectional language model with a feature-based approach \cite{peters2018deep}. It can capture semantic, syntactic, and contextual relationships because ELMo takes the entire input sentence into account before assigning each word a representation or an embedding. 

  

From figure \ref{fig:elmo}, ELMo uses two bidirectional LSTMs, where one is trained from left to right and another is trained from right to left, to produce contextual embeddings. In other words, using two bidirectional LSTMs in training allow the model to learn the word and previous words in the sentence so that the result embeddings can carry contextual information. For example, the following two sentences - ‘The plane already took off’ and ‘His major is plane geometry’ - both contains the word ‘plane’, but the meanings of word ‘plane’ are different due to different context. Therefore, the embeddings that ELMo produced for the word ‘plane’ would be different when the surrounding words are different. 

  

\item BERT 

\label{bert} 

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/BERT-framework.png} 

  \caption{The Architecture of BERT Framework. \cite{devlin2019bert}} 

  \label{fig:bert-fw} 

\end{figure} 

  

BERT stands for Bidirectional Encoder Representations from Transformers, which is a self-attention-based model that can also capture semantic, syntactic, and contextual relationships. The BERT framework contains two parts: pretraining and fine-tuning. The pretraining step is to train the model on the unlabeled dataset, and the fine-tuning part is to fine-tune all the parameters using a labeled dataset. For different tasks, the fine-tuning models are also different. Figure \ref{fig:bert-fw} shows the question-answering model as an example of BERT framework. It is noticeable that the parameters of BERT model are initialized in the pretraining step, then are fine-tuned using a labeled dataset. 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/BERT-architecture.png} 

  \caption{The Architecture of BERT Model. \cite{devlin2019bert}} 

  \label{fig:bert-archi} 

\end{figure} 

  

Figure \ref{fig:bert-archi} shows the architecture of BERT model. BERT model uses a multi-layer bidirectional transformer encoder, where the transformers architecture is shown in figure \ref{fig:transformer}. Specifically, the left part of the Transformer's architecture is the encoder that takes an input sequence of symbol representation and produces a 512-dimensional representation for each word. The right part of the transformers is the decoder that has one more layer than the encoder and has masked multi-head attention which handles the output of the encoder.  

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/Transformer-architecture.png} 

  \caption{The Architecture of Transformers. \cite{attention}} 

  \label{fig:transformer} 

\end{figure} 

  

The multi-head attention contains several scaled dot-product attention layers that run in parallel as shown in figure \ref{fig:multihead}. The scaled dot-product attention takes 3 inputs - Q, K, and V - where Q is a matrix containing a set of queries, K is a matrix containing a set of keys, and V is a matrix containing a set of values. The goal of the attention function is to map a query and a set of key-value pairs to an output. As for the masked multi-head attention in the decoder, the masking is to prevent comparing a word to itself and words located after it \cite{devlin2019bert}. In other words, the prediction for the word at position $i$ is only dependent on the previous outputs at a position less than $i$. 

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/multi-head attention.png} 

  \caption{Multi-head Attention Mechanism. \cite{attention}} 

  \label{fig:multihead} 

\end{figure} 

Additionally, both encoder and decoder are composed of a stack of N identical layers and positional encoding. The positional encoding is vectors that represent the position of a word in the sentence, which allows the model to access each word’s position.  

  

\item ALBERT 

\label{albert} 

  

ALBERT stands for A Lite BERT, whose architecture is similar to BERT, which uses a transformer encoder with GELU nonlinearities \cite{lan2020albert} and has fewer parameters than BERT. Therefore, the training speed for ALBERT is much faster than a traditional BERT.  

  

Specifically, ALBERT utilizes the following two parameter-reduction techniques: a factorized embedding parameterization and cross-layer parameter sharing \cite{lan2020albert}. The first technique is to break down the large embedding matrix into two smaller matrices, which can avoid significantly increase the parameter size of the embeddings when growing the hidden state size. The second technique shares parameters between certain layers to prevent the parameter from growing with the depth of the network. Both techniques reduce the number of parameters considerably and do not severely impact the performance of BERT.  

  

Furthermore, another difference between ALBERT and BERT is that BERT uses an additional loss named next-sentence prediction (NSP), while ALBERT uses a sentence-order prediction (SOP) loss. More specifically, NSP is a binary classification loss for predicting whether two segments show consecutively in the original text \cite{lan2020albert}. Positive examples are created by taking consecutive sentences from the training text corpus. Negative examples are created by pairing sentences from a different corpus. Both positive and negative samples are sampled with equal probability \cite{lan2020albert}. The SOP loss uses the same technique as BERT (i.e., passing two consecutive segments from the same document) for positive examples, but for negative examples, it swaps the order of the same two consecutive segments as positive examples. This allows the model to learn differences between discourse-level coherence properties \cite{lan2020albert}. 

  

\item RoBERTa 

  

RoBERTa stands for Robustly optimized BERT pretraining Approach, where its architecture is also smilier to BERT, which uses a transformer architecture. However, there are mainly four modifications that make RoBERTa different from BERT, which are \cite{liu2019roberta}:  

\begin{enumerate} 

  \item The model trains longer using more data and bigger batches. 

  \item The Next Sentence Prediction (NSP) task from BERT is removed. 

  \item The model trains on longer inputs.

  \item The model uses a dynamic masking strategy.

\end{enumerate} 

  

More specifically, the dynamic masking strategy is to create the masking pattern every time when a sequence is fed to the model. This strategy allows the model to not use the same mask for each training in each epoch, and it slightly improves the performance of the model. The NSP, described in the ALBERT, is removed because removing NSP slightly improves the performance during the training procedure. 

  

\item XLNet 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/XLNet-architecture.png} 

  \caption{The Architecture of Two-Stream Self-Attention for Target-Aware Representations. \cite{attention}} 

  \label{fig:xlnet} 

\end{figure} 

  

XLNet is a generalized autoregressive (AR) pretraining model that uses a permutation language modeling objective, which allows XLNet to retain the advantages of AR models and capture bidirectional contexts \cite{yang2020xlnet}. The conventional AR language model uses the context word to predict the next word, but the context word can be choosing only from the left or right of the predicted word. In other words, AR models cannot use left and right contexts at the same time. For instance, to predict the word ‘plane’ in the sentence ‘The air plane took off’, either [‘the’,’air’] or [‘took’,’off] can be used for the AR models. However, AR models are good at generating context tasks because such tasks normally focus on one direction. And since AR models do not rely on any input corruption, the input noise does not affect the AR models \cite{yang2020xlnet}. 

  

As for the permutation language modeling objective, its architecture is shown in figure \ref{fig:xlnet} that it trains with two-stream attention. The two-stream attentions are the content stream attention and the query stream attention. Specifically, Figure \ref{fig:xlnet} (a) shows content stream attention, which is the same as the standard self-attention. It calculates the content representation that encodes both context and context of the predict target. Figure \ref{fig:xlnet} (b) shows query stream attention, which calculates the query representation that does not include the content representation of the predict target. In addition, the attention mask is used to permute the factorization order. In figure \ref{fig:xlnet} (c), there are two masks: content mask and query mask. Both masks are matrices, but the difference is that the diagonal elements in the content mask can see themselves but cannot see themselves in the query mask.  

  

\item Text GCN 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/text-gcn-schematic.png} 

  \caption{The schematic of Text GCN. \cite{yao2018graph}} 

  \label{fig:text-gcn} 

\end{figure} 

  

Text GCN stands for Text Graph Convolutional Network, which is a graph neural network-based method for text classification that can capture the global relationship. A GCN model is a multi-layer neural network that can perform directly on a graph and generate embedding vectors of nodes based on the information from their neighbors \cite{yao2018graph}. For Text GCN, its input is a one-hot vector that represents every word or document. Then, using those vectors to create a heterogeneous text graph that has word nodes and document nodes and is fed into a two-layer GCN. The node embeddings of the second layer have the same size as the labels set and are fed into a softmax classifier \cite{yao2018graph}.  

  

In addition, edges between two different word nodes (word-word edge) are created by using word co-occurrence information, and edges between a document and a word (document-word edge) are created by using word frequency and word’s document frequency. Therefore, the global word co-occurrence can be modeled. The weights of word-word edges are calculated using the point-wise mutual information (PMI) that can measure word associations \cite{yao2018graph}.  

  
Figure \ref{fig:text-gcn} shows an example of a schematic of Text GCN, where the nodes that begin with “O” are document nodes and others are word nodes, the black bold edges are document-word edges and the gray thin edges are the word-word edges, R(x) in the word document representation means the embedding of x and different colors mean different classes \cite{yao2018graph}. 

  

\item VGCN-BERT 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/vgcn.png} 

  \caption{The Workflow of VGCN-BERT. \cite{lu2020vgcnbert}} 

  \label{fig:vgcn} 

\end{figure} 

  

VGCN-BERT(Vocabulary Graph Convolutional Network BERT) is the model that integrates VGCN into BERT. Since BERT can capture the contextual information and GCN can capture global information about the vocabulary, VGCN-BERT combines those advantages to produce a better representation for classification.  

  

Figure \ref{fig:vgcn} shows processes of VGCN-BERT. Specifically, there are 5 phases. The first phase creates word embeddings for the input sentence, and the next phase creates a vocabulary graph. The vocabulary graph is built using normalized point-wise mutual information (NPMI), where the range of NPMI value is $[-1,1]$ \cite{lu2020vgcnbert}. Positive NPMI values mean a strong semantic correlation between words, while negative NPMI values imply little or no semantic correlation \cite{lu2020vgcnbert}. In addition, the vocabulary graph only extracts and embeds the part that is relevant to the input. Phase 3 produces a graph enriched embedding that contains both word embeddings and graph embeddings generated from previous phases. In Phase 4, multi-layers of self-attention are performed on the graph enriched embedding so that word embeddings and graph embedding can interact with each other. Phase 5 feeds the final embedding generated at the last layer to a fully connected layer for classification.  

\end{itemize} 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/model-comparsion.PNG} 

  \caption{The Abilities of Each Model. *OOV stands for out of vocabulary.} 

  \label{fig:comparison} 

\end{figure} 

  

Figure \ref{fig:comparison} concludes each model's abilities. All models can capture semantic and syntactic relationships, but only GloVe, Text GCN and VGCN-BERT can capture global information. 

==> 2021-EMNLP-Camera Ready/1.Introduction.tex <==
\section{Introduction}
\label{intro}


Since the start of the Coronavirus or COVID-19 pandemic, online social media (e.g., Twitter) has become a conduit for rapid propagation of misinformation \cite{johnson2020covid19}. Although misinformation is considered to be created without the intention of causing harm \cite{Lazer1094}, it can wreak havoc on society \cite{Ciampagliapub.1093084646, neuman_2020,hamilton_2020} and disrupt democratic institutions \cite{Ciampaglia_Mantzarlis_Maus_Menczer_2018}. Misinformation in general, and COVID-19 misinformation in particular, has become a grave concern for the policymakers due to its fast propagation via online social media. A recent study shows that the majority of the COVID-19 social media data is rife with misinformation \cite{brennen_simon_howard_nielsen_2020}. The first step towards preventing misinformation is to \textbf{detect misinformation} in a timely fashion. 


Building automated systems for misinformation detection from social media data is a Natural Language Processing (NLP) task. Various deep learning models have been successfully employed for this type of NLP task of text classification \cite{Kim:2014,Conneau:2017, Wang:2017, Tai:2015, Zhou:2016}. These models learn language representations from a domain, which are then used as numeric features in supervised classification. Due to the prohibitive cost of acquiring labeled data on COVID-19 misinformation, training deep learning models directly using the target data is not a suitable approach. 


%These models implement two steps, i.e., representing language via numeric embeddings, then performing supervised classification. Due to the prohibitive cost of acquiring labeled data on COVID-19 misinformation, training deep learning models using the target data is not a suitable approach. 


\paragraph{Background.} An alternative approach for detecting COVID-19 misinformation from \textbf{small labeled data} is transfer learning \cite{hossain-etal-2020-covidlies}. The dominant paradigm of transfer learning employs a \textbf{mixed-domain} strategy in which representations learned from a general domain (source data) by using domain-agnostic models are transferred into a specific domain (target data) \cite{Pan:2009}. Specifically, it involves creating a pre-trained model (PTM) that learns embedded representations from general-purpose unlabeled data, then adapting the model for a downstream task using the labeled target data \cite{Minaee:2021, Qiu:2020}. 

Two types of neural networks can be used to create PTMs, i.e., shallow and deep. The shallow models such as Word2Vec \cite{mikolov2013efficient} and GloVe \cite{pennington-etal-2014-glove} learn word embeddings that capture semantic, syntactic, and some global relationships \cite{Levy:2014, Srinivasan:2019} of the words from the source text using their co-occurrence information. However, these PTMs do not capture the context of the text \cite{Qiu:2020}. On the other hand, deep PTMs can learn contextual embeddings, i.e., language models \cite{Yoav:2017}. 

Two main approaches for creating deep PTMs are based on sequential and non-sequential models. The sequential Recurrent Neural Network \cite{Pengfei:2016} based model such as ELMo (Embeddings from Language Models) \cite{peters2018deep} is equipped with long short-term memory to capture the local context of a word in sequential order. The non-sequential Transformer \cite{Vaswani:2017} based models such as OpenAI GPT (Generative Pre-training) \cite{Radford:2018}, BERT (Bidirectional Encoder Representation from Transformer) \cite{devlin2019bert}, and XLNet \cite{yang2020xlnet} utilize the attention mechanism \cite{Bahdanau:2016} for learning universal language representation from general-purpose very large text corpora such as Wikipedia and BookCorpus \cite{devlin2019bert} as well as from web crawls \cite{liu2019roberta}. While GPT is an autoregressive model that learns embeddings by predicting words based on previous predictions, BERT utilizes the autoencoding technique based on bi-directional context modeling \cite{Minaee:2021}. XLNet leverages the strengths of autoregressive and autoencoding PLMs \cite{yang2020xlnet}. 

Unlike the Transformer-based deep PTMs, the shallow Word2Vec and GloVe as well as the deep ELMo PTMs are used only as feature extractors. These features are fed into another model for the downstream task of classification, which needs to be trained from scratch using the target data. The deep PTM based mixed-domain transfer learning has achieved state-of-the-art (SOTA) performance in many NLP tasks including text classification \cite{Minaee:2021}.  

Irrespective of the success of the mixed-domain SOTA transfer learning approach for text classification, there has been no study to understand how effective this approach is for navigating through the kaleidoscope of COVID-19 misinformation. Unlike the curated static datasets on which this approach is tested \cite{Minaee:2021}, the dynamic landscape of the COVID-19 social media data has not been fully explored. Some key properties of the COVID-19 data hitherto identified are: (i) The COVID-19 misinformation spreads faster on social media than any other form of health misinformation \cite{johnson2020covid19}. As a consequence, the misinformation narrative evolves rapidly \cite{cui2020coaid}. (ii) The COVID-19 misinformation categories are heavily-skewed \cite{cui2020coaid, memon2020characterizing} and fine-grained \cite{memon2020characterizing}. (iii) The COVID-19 social media misinformation types are often ambiguous (e.g., fabricated, reconfigured, satire, parody)  \cite{brennen_simon_howard_nielsen_2020} and categories may not be mutually exclusive \cite{memon2020characterizing}. These properties pose a unique challenge for the mixed-domain SOTA transfer learning approach for creating an effective solution to the COVID-19 misinformation detection problem. 

Previously, it has been shown that the transfer learning approach generalizes poorly when the domain of the source dataset is significantly different from that of the target dataset \cite{peters2019tune}. On the other hand, \textbf{domain-specific models (DSM)}, which learn representations from domains that are similar to the target domain, provide a generalizable solution for the downstream NLP task \cite{beltagy2019scibert, Lee:2019, Gu:2021}. These models are better at capturing the context of the target domain. However, the efficacy of the DSM-based approach for addressing the COVID-19 misinformation detection problem has not also been investigated. 

\vspace{3.00mm}
\noindent \textbf{In this paper}, we conduct a systematic extensive study to understand the \textbf{scope and limitations} of the mixed-domain transfer learning approach as well as the DSM-based approach to detect COVID-19 misinformation on social media. We use both shallow and deep PTMs for the mixed-domain transfer learning experimentations. The deep PTMs include BERT, XLNet, and two variants of BERT, i.e., RoBERTa \cite{liu2019roberta} and ALBERT \cite{lan2020albert}. While these attention mechanism-based Transformer models are good at learning contextual representations, their ability to learn \textbf{global relationships} among the words in the source text is limited \cite{lu2020vgcnbert}.


The DSMs used in our study are based on shallow architectures. We argue that shallow architectures can be trained efficiently using the limited available domain data. Specifically, we pre-train the DSMs using the small social media data on COVID-19. The shallow DSM-based approach is examined in \textbf{two dimensions: graph-based DSM and non-graph DSM}. The graph-based Text GCN \cite{yao2018graph} model can explicitly capture the \textbf{global relationships} (from term co-occurrence) by leveraging the graph structure of the text. It creates a heterogeneous word document graph with words and documents as nodes for the whole corpus, and turns document classification problem into a node classification problem. We include another graph-based model in our study, i.e., the VGCN-BERT \cite{lu2020vgcnbert}. It combines the strength of Text GCN (to capture global relationships) and BERT (to capture local relationships).


The non-graph DSM models such as Word2Vec and GloVe can mainly capture \textbf{local relationships} among the words of the source text, represented in the latent space of their word embeddings. For extracting \textbf{global relationships} from these embeddings, we utilize a Convolutional Neural Network (CNN). Specifically, we use the word embeddings as input features to a CNN with a one-dimensional kernel \cite{Kim:2014}, which then learns global relationships as high-level features. We \textbf{hypothesize} that the local and global relationships should improve the generalization capability of the non-graph DSM+CNN approach.



%complement the non-graph DSMs by taking their learned word embeddings for training a shallow Convolutional Neural Network (CNN) with the one-dimensional kernel for extracting local patterns amenable to text classification .


%We investigate \textbf{three DSM-based models} that use content co-occurrence information for learning the embeddings, which are Word2Vec \cite{mikolov2013efficient}, GloVe \cite{pennington-etal-2014-glove}, and Text GCN \cite{yao2018graph}. While the Text GCN is a \textbf{graph-based} model that explicitly captures the global relationships (from term-co-occurrence) by leveraging the graph structure of the text, the first two non-graph models mainly capture local relationships among the terms in the text. Both Word2Vec and GloVe provide just the embeddings, which we then use to train a shallow Convolutional Neural Network (CNN) with the one-dimensional kernel for extracting local patterns amenable to text classification \cite{Kim:2014}. On the other hand, the Text GCN creates a heterogeneous word document graph with words and documents as nodes for the whole corpus, and turns document classification into a node classification problem. Another graph-based model that we use in this study is the VGCN-BERT \cite{lu2020vgcnbert} that combines the strength of Text GCN (to capture global relationship) and BERT (to capture local relationship).

We evaluate the \textbf{generalizability} of the above-mentioned diverse array of NLP techniques via a set of studies that explore \textbf{various dimensions of the COVID-19 data}. We focus on the Twitter social media platform because of its highest number of news-focused users \cite{hughes_wojcik_2020}. In addition to analyzing the tweet messages, we use online news articles referred to in the tweets. Our study spans along multiple dimensions of the COVID-19 data that include temporal dimension (the context in the dataset evolves), length dimension (short text such as tweets vs. lengthy text such as news articles), size dimension (small dataset vs. large dataset), and classification-level dimension (binary vs. multi-class data). 


\paragraph{Contributions.} We design a novel study for examining the generalizability of a diverse set of deep learning NLP techniques on the multi-dimensional space of COVID-19 online misinformation landscape. Our main contributions are as follows.


\begin{itemize}

  \item We identify the unique challenges for the deep learning based NLP techniques to detect misinformation from COVID-19 social media data. 
  
  \item We argue that an effective model for this type of data must capture both the local and the global context of the domain in its latent space of embeddings.
    
  \item We show that the mixed-domain deep learning SOTA transfer learning approach is not always effective. 
  
  \item We find that the shallow CNN classifier initialized with word embeddings learned via the non-graph DSMs is more effective across most of the dimensions of the COVID-19 data space, especially when the labeled target data is small.
  
  \item We \textbf{explain} why the Transformer-based mixed-domain transfer learning approach is not effective on COVID-19 data as well as why the non-graph DSM+CNN may offer a more generalizable solution.

\end{itemize}


The rest of the paper is organized as follows. In section 2, we present the diverse NLP techniques, analyze the multi-dimensional datasets, and describe the study design. Results obtained from the experiments are provided in section 3 followed by a detailed analysis. Section 4 presents the conclusion. Appendix provides related work, additional analysis of the datasets, and experiment setting.


%In the appendix, we discuss the related work and provide an additional analysis of the dataset. Finally, we report the experimental setting and training statistics.



==> 2021-EMNLP-Camera Ready/2.LiteratureSurvey.tex <==
\section{Literature Survey} 

% a) ML based health misinformation and Covid misinformation detection approaches 

  

% - Shahi 2020 (FakeCovid) 

  

% - Cui 2020 (CoAID) 

  

% - Hossain 2020 (CovidLies) 

  

% and other covid related papers that you studied. 

  

  

% b) NLP methods 

  

% Review all NLP papers that you studied. Don't miss any 

  

% include this: 

% Lu-2020-VGCN-BERT- Augmenting BERT with Graph Embedding for Text Classification 

  

  

% For each paper address the following: 

  

% - Brief summary of the paper  

  

% - Main limitation in solving the covid misinformation classification problem 

  

% - Wherever possible connect the current paper to the next paper 

In this chapter, we discuss the Machine Learning (ML) based main research approaches for detecting misinformation on social media related to health and COVID-19.  

  

The ML approaches involve two steps: creating text embedding and performing supervised classification. Specifically, text embeddings are created using NLP techniques, then a supervised classifier is used to detect misinformation data. Importantly, much of the effort in misinformation detection is invested in creating the labeled dataset. 


Below we describe the main papers that contribute towards labeled dataset creation, text embedding, and supervised classification. 

  

\subsection{Health Misinformation} 

  

% - Kinsora's main contribution is to create a labeled dataset for general health misinformation. 

  

As aforementioned, the COVID-19 causes an `infodemic' which draws many researchers' attentions to exploring methods that can effectively detect COVID-19 related misinformation. Before the COVID-19 virus appears, however, there are already many ML-based types of researches that have been conducted for health misinformation detection. It is also noteworthy that the quality of a dataset used for misinformation detection is quite important. Particularly, Kinsora et al.\cite{Kinsora:2017} develops a small labeled dataset that contains misinformative posts collected from a medical forum, and it also includes other features other than the content of posts, which are proven to be useful for improving detection accuracy in their study. Their dataset is useful for studying general health misinformation, but it is not applicable to be used for classifying a dataset that contains texts about newly discovered diseases (i.e., COVID-19). Besides, it is easier to label general health misinformation posts since there existed many experts who have conducted comprehensive studies on diseases or viruses that have been discovered before.  

  

\subsection{COVID-19 Misinformation} 

  

For COVID-19 misinformation, creating a labeled dataset is significantly more challenging. Due to the diversity of misinformation and the speed of its evolution, it is a tall task for the experts to label data correctly. 

  

Hossain et al. \cite{hossain-etal-2020-covidlies} build a dataset called COVIDLIES that contains COVID-19 related tweets, which are collected from March to April 2020 and categorized as Agree, Disagree, and No Stance. Each tweet is also paired with a known misconception that is extracted manually from Wikipedia COVID-19 related articles. A label of a tweet is Agree if it agrees with the misconception, Disagree if it disagrees with the misconception, and No Stance if it expresses no stance to the misconception. Another dataset created by Shahi et al.\cite{shahifakecovid} is a multilingual dataset named FakeCovid, which only contains news articles collected from 04/01/2020 to 15/05/2020. This dataset contains a total of 5128 articles written in 40 different languages, and only 40.8\% of articles are in the English language.  

  

For both COVIDLIES and FakeCovid datasets, one of their limitations is that they only contain one type of data source, where COVIDLIES is built based on tweets and FakeCovid is based on news articles. Another limitation is that both datasets only include a month of data, which is not sufficient to detect COVID-19 misinformation due to the fact that the words used related to COVID-19 are changed from time to time. Therefore, another comprehensive COVID-19 dataset is created by Cui et al.\cite{cui2020coaid} called CoAID. It contains COVID-19 related tweets, replies, news articles, and ground truth labels. The tweets consist of two parts: news-related tweets and claims of tweets, and tweet replies under those tweets or news articles. The dataset also includes four different months of data. See more details in section \ref{coaid}. However, compared to FakeCovid, the content of CoAID and COVIDLIES datasets is not preprocessed, and the sizes are reduced since some tweets cannot be retrieved because they are deleted or unauthorized to fetch during the collecting process.  



The above datasets are used to train Supervised classifiers (i.e., Support Vector Machine or Logistic Regression) by authors, but the classifiers require the text data to be embedded. Therefore, NLP techniques are used to embed text data. 

  

\subsection{Text Embedding Techniques and Classification} 

  

% - Word2Vec and GloVe: text embedding 

  

% - BERT and its variants: text embedding and classification 

  

% - Text GCN: text embedding and classification 

  

The NLP techniques are being widely used in creating text embeddings. In 2013, Mikolov et al.\cite{mikolov2013efficient} introduces Word2Vec models that can produce high-quality representations of words, which are CBOW and Skip-gram model. The difference between CBOW and Skip-gram model is that CBOW uses context to predict the current word, while Skip-gram uses the current word to predict surrounding words. In 2014, another word representation called GloVe is created by Pennington et al.\cite{pennington-etal-2014-glove}, which is different from Word2Vec models since GloVe uses count-based methods while Word2Vec models are prediction-based methods. In other words, word representations of GloVe are based on global word-word co-occurrence counts, while Word2Vec tries to capture co-occurrence one window at a time.  

  

Both Word2Vec and GloVe methods can capture semantic and syntactic relationships of a language. However, they are unable to carry contextual information. Hence, in recent years, new word representation techniques are being developed so that contextual information can be captured. The ELMo created by Peters et al.\cite{peters2018deep} is one of the techniques that can capture the contextual relationship. It uses a bidirectional language model (biLSTM), where the states from higher-level LSTM can capture word meaning and lower-level LSTM can capture syntax. The combination of both states generated from high and lower-level LSTM is the final rich word representation. Meanwhile, another state-of-the-art technique named BERT was invented by Devlin et al.\cite{devlin2019bert}, which uses transformers techniques. More details about transformers are provided in the following section \ref{bert}. BERT model shows that transfer learning using pretrained model can be fine-tuned to obtain decent performances for different downstream tasks. However, BERT model is limited to capturing global information. Therefore, a new method called Text GCN is developed by Yao et al.\cite{yao2018graph} that can capture high-order neighborhood information because it can explicitly model global word co-occurrence. It is different from other GCN models because it produces a heterogeneous graph where documents and words are nodes. Its limitation is that it could not train using the unlabeled dataset, fast generate embeddings and predict for unseen documents\cite{yao2018graph}. 

  

Additionally, there are many other methods developed based on BERT to obtain better performance. Specifically, Liu et al.\cite{liu2019roberta} creates a better recipe for training BERT, which is called RoBERTa. There are four modifications made to improve BERT, which are: longer training time with more data; no next sentence prediction; longer sequences are used for training; and using dynamic masking technique. Therefore, RoBERTa requires more data and time for training. Another variant of BERT is called ALBERT created by Lan et al.\cite{lan2020albert}, which utilizes two parameter-reduction techniques that can address the memory limitation issues. The two parameter-reduction techniques are a factorized embedding parameterization and cross-layer parameter sharing. See more details in Section \ref{albert}.  

  

% Transformers have a potential of learning longer-term dependency, but are limited by a fixed-length context in the setting of language modeling. the model lacks necessary contextual information needed to well predict the first few symbols, leading to inefficient optimization and inferior performance. 

  

% As a consequence of the fixed context length, the model cannot capture any longer-term dependency beyond the predefined context length.  

  

%In addition, the fixed-length segments are created by selecting a consecutive chunk of symbols without respecting the sentence or any other semantic boundary. 

  

% Transformer-XL that enables learning dependency beyond a fixed length without disrupting temporal coherence. 

%we introduce a simple but more effective relative positional encoding formulation that generalizes to attention lengths longer than the one observed during training. 

In the meantime, there are researches focusing on improving the Transformer\cite{attention}. Specifically, the transformer-based language modeling (e.g., BERT) has a fixed-length length context setting, which creates fixed-length segments by selecting a consecutive set of symbols without considering the whole sentence or semantic boundary \cite{dai2019transformerxl}. This setting makes the model unable to obtain longer-term dependency that can cause inefficient optimization and poorer performance\cite{dai2019transformerxl}. In 2019, a new Transformer called Transformer-XL (Transformer-Extra Long) is created by Dai et al.\cite{dai2019transformerxl} which can learn longer-term dependency without damaging the temporal coherence and they also create a relative positional encoding scheme that helps solve the fixed-length context issue. In 2020, a Transformer-XL based model called XLNet is developed by Yang et al.\cite{yang2020xlnet}, which is a generalized autoregressive (AR) pretraining method. It combines the advantage of AR models and BERT and avoids their weaknesses. For instance, AR language modeling does not suffer from input noise, while BERT can better capture bidirectional context. Moreover, XLNet utilizes the techniques from Transformer-XL (e.g., relative positional encoding) to improve the performance for pretraining.  

These variants of BERT model made an improvement in different aspects of BERT. However, they do not address the issue that BERT is limited to capturing global information. A model called VGCN-BERT is created by Lu et al.\cite{lu2020vgcnbert} that integrates GCN into BERT, which combines the advantages of BERT and GCN to create an enriched representation of words for classification. VGCN-BERT model uses multiple layers of attention mechanism on a graph word embedding, which is built based on word embedding and vocabulary graph. The word embedding and vocabulary graph embedding is concatenated if they have a high semantic correlation. The limitation of VGCN-BERT model is that it only accepts lexical relations (i.e., vocabulary graph) of a language. 

  

\subsection{Model Description}  

  

\begin{itemize} 

   

\item Word2Vec 

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/word2vec-architectures.png} 

  \caption{Left is CBOW Architecture and Right is Ski-gram Model Architecture. \cite{mikolov2013efficient}} 

  \label{fig:w2v} 

\end{figure} 

  

The Word2Vec is an algorithm that takes text corpus as inputs and outputs vector representations of each word that contains semantic and syntactic relationships between each word. There are two different architectures based on Word2Vec, which are CBOW (continuous bag-of-words) model and Skip-gram (continuous skip-gram) model. Figure \ref{fig:w2v} shows architectures of CBOW and Ski-gram. It is obvious to observe the difference between CBOW and Skip-gram, in which the CBOW model combines the continuous distributed representations of context to predict the current word, while the Skip-gram model creates the distributed representation of the current word to predict its surrounding words. For example, if the training input is ‘I like trees’, then CBOW model creates vector representations of the context ‘I’ and ‘trees’ to predict the current word ‘like’, while Skip-gram model creates vector representation of the current word ‘like’ to predict the context ‘I’ and ‘trees’.  

  

In addition, the distance between the current word and predicted word within a sentence is a hyperparameter called window size. In other words, if the window size is larger, more neighbor words of the current word will be taken into account during training. For instance, if the training input is ‘I am eating apples and bananas now’ and the current word is ‘apples’, and the window size is 2, then the context of the current word is [eating, and]. If the window size is 4, then the context is [am, eating, and, bananas]. A larger window size will increase the training time.  

  

\item GloVe  

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/Glove-architecture.png} 

  \caption{The Architecture of GloVe Model. \cite{liu_zhang_li_yan_2019}} 

  \label{fig:glove} 

\end{figure} 

  

  

Another model that can capture semantic and syntactic relationships is the GloVe model. GloVe is an unsupervised learning algorithm that can produce a word vector space with a meaningful substructure by training on aggregated global word-word co-occurrence counts \cite{pennington-etal-2014-glove}. 

  

The GloVe model is different from other models that also use the statistic of word occurrences because of its weighted least squares regression with the new cost functions, which can address the problem of rare co-occurrences that are noisy and carry less information.  

  

The cost function \cite{pennington-etal-2014-glove} looks as follows:  

  

$J = \sum_{i,j=1}^{V} f(X_{ij})(w^T_i \tilde{w} + b_i + \tilde{b_j} - log{X_{i,j}})^2$, 

  

%where X is the word-word co-occurrence counts, $X_{i,j}$ is the number of times that word j appears in the context of word I, V is the size of vocabulary of a corpus, $b$ and $\tilde{b}$ are biases, $w \in \mathbb{R}^d$ are word vectors, and $\tilde{w} \in \mathbb{R}^d$ are context word vectors. The difference between $w$ and $\tilde{w}$ is their random initializations.  

  

This weighting function also has the following properties: 

\begin{enumerate} 

  \item $f(0)=0.$ If f is viewed as a continuous function, $lim_{x\rightarrow0}f(x)log^2x$ is finite. 

  \item $f(x)$ should be non-decreasing in order to avoid that rare co-occurrences are overweighted. 

  \item $f(x)$ should be relatively small for large value of x, in order to avoid that frequent co-occurrences are overweighted.  

\end{enumerate} 

  

The following $f(x)$ usually works well: 

  

%$ 
%
%f(x)= \begin{cases} 
%
%(x/x_max)^\alpha, & x > x_max \\ 
%
%1, & otherwise 
%
%\end{cases} 
%
%$ 

  

Figure \ref{fig:glove} shows the architecture of the GloVe model. Specifically, the GloVe model takes one-hot representations of words as input and uses word embedding matrices as weighted matrices to output vectors that are inner products of word vectors.  

  

\item ELMo 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/ELMo_architecture.png} 

  \caption{The Architecture of ELMo Model. \cite{devlin2019bert}} 

  \label{fig:elmo} 

\end{figure} 

  

ELMo stands for Embeddings from Language Models, which is a bidirectional language model with a feature-based approach \cite{peters2018deep}. It can capture semantic, syntactic, and contextual relationships because ELMo takes the entire input sentence into account before assigning each word a representation or an embedding. 

  

From figure \ref{fig:elmo}, ELMo uses two bidirectional LSTMs, where one is trained from left to right and another is trained from right to left, to produce contextual embeddings. In other words, using two bidirectional LSTMs in training allow the model to learn the word and previous words in the sentence so that the result embeddings can carry contextual information. For example, the following two sentences - ‘The plane already took off’ and ‘His major is plane geometry’ - both contains the word ‘plane’, but the meanings of word ‘plane’ are different due to different context. Therefore, the embeddings that ELMo produced for the word ‘plane’ would be different when the surrounding words are different. 

  

\item BERT 

\label{bert} 

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/BERT-framework.png} 

  \caption{The Architecture of BERT Framework. \cite{devlin2019bert}} 

  \label{fig:bert-fw} 

\end{figure} 

  

BERT stands for Bidirectional Encoder Representations from Transformers, which is a self-attention-based model that can also capture semantic, syntactic, and contextual relationships. The BERT framework contains two parts: pretraining and fine-tuning. The pretraining step is to train the model on the unlabeled dataset, and the fine-tuning part is to fine-tune all the parameters using a labeled dataset. For different tasks, the fine-tuning models are also different. Figure \ref{fig:bert-fw} shows the question-answering model as an example of BERT framework. It is noticeable that the parameters of BERT model are initialized in the pretraining step, then are fine-tuned using a labeled dataset. 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/BERT-architecture.png} 

  \caption{The Architecture of BERT Model. \cite{devlin2019bert}} 

  \label{fig:bert-archi} 

\end{figure} 

  

Figure \ref{fig:bert-archi} shows the architecture of BERT model. BERT model uses a multi-layer bidirectional transformer encoder, where the transformers architecture is shown in figure \ref{fig:transformer}. Specifically, the left part of the Transformer's architecture is the encoder that takes an input sequence of symbol representation and produces a 512-dimensional representation for each word. The right part of the transformers is the decoder that has one more layer than the encoder and has masked multi-head attention which handles the output of the encoder.  

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/Transformer-architecture.png} 

  \caption{The Architecture of Transformers. \cite{attention}} 

  \label{fig:transformer} 

\end{figure} 

  

The multi-head attention contains several scaled dot-product attention layers that run in parallel as shown in figure \ref{fig:multihead}. The scaled dot-product attention takes 3 inputs - Q, K, and V - where Q is a matrix containing a set of queries, K is a matrix containing a set of keys, and V is a matrix containing a set of values. The goal of the attention function is to map a query and a set of key-value pairs to an output. As for the masked multi-head attention in the decoder, the masking is to prevent comparing a word to itself and words located after it \cite{devlin2019bert}. In other words, the prediction for the word at position $i$ is only dependent on the previous outputs at a position less than $i$. 

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/multi-head attention.png} 

  \caption{Multi-head Attention Mechanism. \cite{attention}} 

  \label{fig:multihead} 

\end{figure} 

Additionally, both encoder and decoder are composed of a stack of N identical layers and positional encoding. The positional encoding is vectors that represent the position of a word in the sentence, which allows the model to access each word’s position.  

  

\item ALBERT 

\label{albert} 

  

ALBERT stands for A Lite BERT, whose architecture is similar to BERT, which uses a transformer encoder with GELU nonlinearities \cite{lan2020albert} and has fewer parameters than BERT. Therefore, the training speed for ALBERT is much faster than a traditional BERT.  

  

Specifically, ALBERT utilizes the following two parameter-reduction techniques: a factorized embedding parameterization and cross-layer parameter sharing \cite{lan2020albert}. The first technique is to break down the large embedding matrix into two smaller matrices, which can avoid significantly increase the parameter size of the embeddings when growing the hidden state size. The second technique shares parameters between certain layers to prevent the parameter from growing with the depth of the network. Both techniques reduce the number of parameters considerably and do not severely impact the performance of BERT.  

  

Furthermore, another difference between ALBERT and BERT is that BERT uses an additional loss named next-sentence prediction (NSP), while ALBERT uses a sentence-order prediction (SOP) loss. More specifically, NSP is a binary classification loss for predicting whether two segments show consecutively in the original text \cite{lan2020albert}. Positive examples are created by taking consecutive sentences from the training text corpus. Negative examples are created by pairing sentences from a different corpus. Both positive and negative samples are sampled with equal probability \cite{lan2020albert}. The SOP loss uses the same technique as BERT (i.e., passing two consecutive segments from the same document) for positive examples, but for negative examples, it swaps the order of the same two consecutive segments as positive examples. This allows the model to learn differences between discourse-level coherence properties \cite{lan2020albert}. 

  

\item RoBERTa 

  

RoBERTa stands for Robustly optimized BERT pretraining Approach, where its architecture is also smilier to BERT, which uses a transformer architecture. However, there are mainly four modifications that make RoBERTa different from BERT, which are \cite{liu2019roberta}:  

\begin{enumerate} 

  \item The model trains longer using more data and bigger batches. 

  \item The Next Sentence Prediction (NSP) task from BERT is removed. 

  \item The model trains on longer inputs.

  \item The model uses a dynamic masking strategy.

\end{enumerate} 

  

More specifically, the dynamic masking strategy is to create the masking pattern every time when a sequence is fed to the model. This strategy allows the model to not use the same mask for each training in each epoch, and it slightly improves the performance of the model. The NSP, described in the ALBERT, is removed because removing NSP slightly improves the performance during the training procedure. 

  

\item XLNet 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/XLNet-architecture.png} 

  \caption{The Architecture of Two-Stream Self-Attention for Target-Aware Representations. \cite{attention}} 

  \label{fig:xlnet} 

\end{figure} 

  

XLNet is a generalized autoregressive (AR) pretraining model that uses a permutation language modeling objective, which allows XLNet to retain the advantages of AR models and capture bidirectional contexts \cite{yang2020xlnet}. The conventional AR language model uses the context word to predict the next word, but the context word can be choosing only from the left or right of the predicted word. In other words, AR models cannot use left and right contexts at the same time. For instance, to predict the word ‘plane’ in the sentence ‘The air plane took off’, either [‘the’,’air’] or [‘took’,’off] can be used for the AR models. However, AR models are good at generating context tasks because such tasks normally focus on one direction. And since AR models do not rely on any input corruption, the input noise does not affect the AR models \cite{yang2020xlnet}. 

  

As for the permutation language modeling objective, its architecture is shown in figure \ref{fig:xlnet} that it trains with two-stream attention. The two-stream attentions are the content stream attention and the query stream attention. Specifically, Figure \ref{fig:xlnet} (a) shows content stream attention, which is the same as the standard self-attention. It calculates the content representation that encodes both context and context of the predict target. Figure \ref{fig:xlnet} (b) shows query stream attention, which calculates the query representation that does not include the content representation of the predict target. In addition, the attention mask is used to permute the factorization order. In figure \ref{fig:xlnet} (c), there are two masks: content mask and query mask. Both masks are matrices, but the difference is that the diagonal elements in the content mask can see themselves but cannot see themselves in the query mask.  

  

\item Text GCN 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/text-gcn-schematic.png} 

  \caption{The schematic of Text GCN. \cite{yao2018graph}} 

  \label{fig:text-gcn} 

\end{figure} 

  

Text GCN stands for Text Graph Convolutional Network, which is a graph neural network-based method for text classification that can capture the global relationship. A GCN model is a multi-layer neural network that can perform directly on a graph and generate embedding vectors of nodes based on the information from their neighbors \cite{yao2018graph}. For Text GCN, its input is a one-hot vector that represents every word or document. Then, using those vectors to create a heterogeneous text graph that has word nodes and document nodes and is fed into a two-layer GCN. The node embeddings of the second layer have the same size as the labels set and are fed into a softmax classifier \cite{yao2018graph}.  

  

In addition, edges between two different word nodes (word-word edge) are created by using word co-occurrence information, and edges between a document and a word (document-word edge) are created by using word frequency and word’s document frequency. Therefore, the global word co-occurrence can be modeled. The weights of word-word edges are calculated using the point-wise mutual information (PMI) that can measure word associations \cite{yao2018graph}.  

  
Figure \ref{fig:text-gcn} shows an example of a schematic of Text GCN, where the nodes that begin with “O” are document nodes and others are word nodes, the black bold edges are document-word edges and the gray thin edges are the word-word edges, R(x) in the word document representation means the embedding of x and different colors mean different classes \cite{yao2018graph}. 

  

\item VGCN-BERT 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/vgcn.png} 

  \caption{The Workflow of VGCN-BERT. \cite{lu2020vgcnbert}} 

  \label{fig:vgcn} 

\end{figure} 

  

VGCN-BERT(Vocabulary Graph Convolutional Network BERT) is the model that integrates VGCN into BERT. Since BERT can capture the contextual information and GCN can capture global information about the vocabulary, VGCN-BERT combines those advantages to produce a better representation for classification.  

  

Figure \ref{fig:vgcn} shows processes of VGCN-BERT. Specifically, there are 5 phases. The first phase creates word embeddings for the input sentence, and the next phase creates a vocabulary graph. The vocabulary graph is built using normalized point-wise mutual information (NPMI), where the range of NPMI value is $[-1,1]$ \cite{lu2020vgcnbert}. Positive NPMI values mean a strong semantic correlation between words, while negative NPMI values imply little or no semantic correlation \cite{lu2020vgcnbert}. In addition, the vocabulary graph only extracts and embeds the part that is relevant to the input. Phase 3 produces a graph enriched embedding that contains both word embeddings and graph embeddings generated from previous phases. In Phase 4, multi-layers of self-attention are performed on the graph enriched embedding so that word embeddings and graph embedding can interact with each other. Phase 5 feeds the final embedding generated at the last layer to a fully connected layer for classification.  

\end{itemize} 

  

\begin{figure}[h] 

  \centering 

  \includegraphics[width=\linewidth]{figures/model-comparsion.PNG} 

  \caption{The Abilities of Each Model. *OOV stands for out of vocabulary.} 

  \label{fig:comparison} 

\end{figure} 

  

Figure \ref{fig:comparison} concludes each model's abilities. All models can capture semantic and syntactic relationships, but only GloVe, Text GCN and VGCN-BERT can capture global information. 

==> 2021-EMNLP-Camera Ready/2.Related.tex <==
\section{Related Work} 






%While in image recognition a DL model only manipulates the spatial relationship in the input feature space within a small region, the sequential nature of the text data necessitates capturing the text both locally and globally. 


Solving Natural Language Processing (NLP) tasks using Deep Learning (DL) based models is a challenging venture. Unlike computer vision problems in which deep learning supervised model can learn expressive representations directly from raw pixels of the input data while performing a discrimination task, the deep learning based supervised NLP systems cannot use raw text input while solving NLP tasks. The text input data needs to be encoded with latent representations or embeddings. These embeddings are learned by neural models from general-purpose unlabeled data using the self-supervised learning approach \cite{Tendle:2021}. The embeddings must capture the multi-dimensional relationships of the text components, which are non-contextual and contextual relationships. The non-contextual relationship includes syntactic relationships and semantic relationships. On the other hand, the contextual relationship includes dynamic representations of words, which requires embeddings to capture the local and global relationships of the words. 

%Unlike in image recognition problems where a DL model can directly use raw pixel input for learning high-level representations, text input in NLP tasks cannot be directly used for learning. At first, the discrete input symbols of the text need to be mapped into a numeric embedded space.

Sequence DL models such as Recurrent Neural Network (RNN) have been used to learn the local context of a word in sequential order \cite{Sutskever:2014}. RNNs process text as a sequence of words for capturing word dependencies and text structures. However, they suffer from two limitations. First, they are unable to create good representations due to the uni-directional processing \cite{peters2018deep}. Second, these models struggle with capturing long-term dependency \cite{Hochreiter:1997}. These two issues were partially resolved by introducing the bi-directional LSTM model \cite{Schuster:1997}. This model was combined with two-dimensional max-pooling in \cite{Zhou:2016} for capturing text features. In addition to this type of chain-structured LSTM, tree-structured LSTM such as the Tree-LSTM model was developed for learning rich semantic representations \cite{Tai:2015}. Irrespective of the progress harnessed by RNN-based models, they do not perform well in capturing global relationships (i.e., long-term dependencies) among the words of the source text. Also, training this type of model on large data is inefficient.


An efficient approach for some NLP tasks such as text classification is a shallow Convolutional Neural Network (CNN) with a one-dimensional convolutional kernel \cite{Kim:2014}. This model is good at capturing local patterns such as key phrases in the text. However, it does not work effectively if the weights of the input layer are initialized randomly \cite{Kim:2014}. It was shown to be effective only in transfer learning in which, first, word embeddings are created using a self-supervised pre-trained model (PTM) such as Word2Vec \cite{mikolov2013efficient}, then the CNN uses its single layer of convolution on top of the word embeddings to learn high-level representations. 


The use of PTMs for mixed-domain transfer learning ushered in a new era in NLP \cite{Qiu:2020}. The PTMs are created from general-purpose unlabeled data by using the self-supervised learning technique. In general, the SSL technique learns representations by predicting a hidden property of the input from the observable properties \cite{LeCun:2021}. Two types of PTMs are used in NLP: (i) PTMs that are feature extractors, i.e., learn word embeddings \cite{mikolov2013efficient, pennington-etal-2014-glove, peters2018deep}, which are used as input to another model for solving a downstream NLP task \cite{Kim:2014}, and (ii) PTMs that learn language models and the same PTM is adapted (fine-tuned) for solving downstream NLP tasks \cite{devlin2019bert}. The feature extractor PTMs such as Word2Vec  \cite{mikolov2013efficient}, GloVe  \cite{pennington-etal-2014-glove}, and ELMo \cite{peters2018deep} are based on both shallow and deep neural network architectures. While shallow Word2Vec and GloVe models learn non-contextual word embeddings from unlabeled source data, the deep ELMo model  is good for creating contextual embeddings. Features learned from these PTMs are used as input to another neural network for solving a downstream NLP task using labeled target data. 


Both Word2Vec and GloVe learn word embeddings from their co-occurrence information. While Word2Vec leverages co-occurrence within the local context, GloVe utilizes global word-to-word co-occurrence counts from the entire corpus. Word2Vec is a shallow feed-forward neural network-based predictive model that learns embeddings of the words while improving their predictions within the local context. On the other hand, GloVe is a count-based model that applies dimensionality reduction on the co-occurrence count matrix for learning word embeddings. These two models are good at capturing syntactic as well as semantic relationships. Although they can capture some global relationships between words in a text \cite{Levy:2014, Srinivasan:2019}, their embeddings are context-independent. Thus, these two models are not good at language modeling. A language model can predict the next word in the sequence given the words that precede it \cite{Yoav:2017}, which requires it to capture the context of the text. The deep architecture feature extractor PTM ELMo (Embeddings from Language Models) \cite{peters2018deep} learns contextualized word embeddings, i.e., it maps a word to different embedding vectors depending on their context. It uses two LSTMs in the forward and backward directions to encode the context of the words. The main limitation of this deep PTM is that it is computationally complex due to its sequential processing of text. Thus, it is prohibitively expensive to train using a very large text corpus. Another limitation of this model, which also applies to feature extractor PTMs in general, is that for solving downstream NLP tasks we need to train the entire model, except for the input embedding layer, from scratch.


The above two limitations of the feature extractor PTMs are addressed by a very deep architecture-based Transformer model \cite{Vaswani:2017}. Unlike the feature extractor sequential PTMs, Transformer is a non-sequential model that uses self-attention \cite{Bahdanau:2016} to compute an attention score for capturing the influence of every word on other words in a sentence or document. This process is parallelized, which enables training deep Transformer models efficiently using very large text corpus such as Wikipedia and BookCorpus \cite{devlin2019bert} as well as web crawls \cite{liu2019roberta}.


There are two main types of Transformer-based deep PTMs: autoregressive and autoencoding. The OpenAI GPT (Generative Pre-training) \cite{Radford:2018} is an autoregressive model that learns embeddings by predicting words based on previous predictions. Specifically, it is a uni-directional model that predicts words sequentially in a text. On the other hand, BERT \cite{devlin2019bert} utilizes the autoencoding technique based on bi-directional context modeling. Specifically, for training, it uses a masked language modeling (MLM) task. The MLM randomly masks some tokens in a text sequence, then it predicts the masked tokens by learning the encoding vectors. 

Variants of BERT such as RoBERTa  \cite{liu2019roberta} and ALBERT \cite{lan2020albert} were proposed to improve its effectiveness as well as efficiency. RoBERTa (Robustly optimized BERT) improves the effectiveness of BERT by using several strategies that include the following. It trains the model longer using more data, lengthy input, and larger batches. It uses a dynamic masking strategy and removes BERT's Next Sentence Prediction (NSP) task. ALBERT (A Lite BERT) improves the efficiency of BERT by employing fewer parameters, which increases its training speed. 

There have been attempts such as in XLNet \cite{yang2020xlnet} to integrate the strengths of the autoregressive and autoencoding Transformer techniques. XLNet is an autoregressive model that uses a permutation language modeling objective. This allows XLNet to retain the advantages of autoregressive models while leveraging the benefit of the autoencoding models, i.e., to capture the bi-directional context.  


Irrespective of the state-of-the-art (SOTA) performance of the deep PTM based mixed-domain transfer learning approach on many NLP tasks \cite{Minaee:2021}, this approach is not suitable for detecting misinformation from COVID-19 social media data. It generalizes poorly when the domain of the source dataset used to create the PTMs is significantly different from that of the target dataset \cite{peters2019tune}. One solution to this generalizability problem is to create a PTM using data that shares context similar to the target domain, i.e., pre-train a domain-specific model (DSM). This type of model encodes the context of the target domain more effectively to provide a generalizable solution for the downstream task \cite{beltagy2019scibert, Lee:2019, Gu:2021}. However, pre-training a deep architecture-based DSM (e.g., BERT) for the COVID-19 misinformation detection task in a timely fashion could be infeasible as it requires collecting a large amount of COVID-19 social media data, which must cover the diverse landscape of COVID-19 misinformation. While there was an effort to create such a deep DSM using COVID-19 tweets in \cite{Muller:2020}, capturing the dynamic context of the pandemic requires the collection of various types of social media data at a large scale. 

Thus, to create DSMs for the COVID-19 domain using quickly collectible small data, shallow architecture based PTMs such as Word2Vec and GloVe are suitable. However, as mentioned earlier, these PTMs are context-independent and are not good at capturing the global relationships well. To compensate for these shortcomings, we used the extracted features from the Word2Vec and GloVe DSMs  for training a one-dimensional convolutional kernel-based CNN similar to the shallow architecture given in \cite{Kim:2014}. The CNN learns global relationships by extracting local patterns in a hierarchical fashion by convolving over the word embeddings. 

Another type of DSM we used is graph-based that leverages the linguistic-aware graph structure of the text for learning contextual representations, then uses those representations to solve a downstream NLP task. The main intuition driving the graph-based technique is that by modeling the vocabulary graph, it will be possible to encode global relationships in the embeddings. Text GCN (Text Graph Convolutional Network) \cite{yao2018graph} is a graph-based model that explicitly captures the global term-co-occurrence information by leveraging the graph structure of the text. It models the global word co-occurrence by incorporating edges between words as well as edges between a document and a word. Word-word edges are created by using word co-occurrence information and word-document edges are created by using word frequency and word-document frequency. Its input is a one-hot vector representation of every word in the document, which is used to create a heterogeneous text graph that has word nodes and document nodes. These are fed into a two-layer GCN (Graph Convolutional Network) \cite{Kipf:2016} that turns document classification into a node classification problem.





Although Text GCN is good at convolving the global information in the graph, it does not take into account local information such as word orders. To address this issue, Text GCN was combined with BERT, which is good at capturing local information. The resulting model is VGCN-BERT \cite{lu2020vgcnbert}. BERT captures the local context by focusing on local word sequences, but it is not good at capturing global information of a text. It learns representations from a sentence or a document. However, it does not take into account the knowledge of the vocabulary. Thus its language model may be incomplete. On the other hand, Text GCN captures the global vocabulary information. The VGCN-BERT aims to capture both local and global relationships by integrating GCN with BERT. Both the graph embeddings and word embeddings are fed into a self-attention encoder in BERT.  When the classifier is trained, these two types of embeddings interact with each other through the self-attention mechanism. As a consequence, the classifier creates representations by fusing global information with local information in a guided fashion.





==> 2021-EMNLP-Camera Ready/3.Method.tex <==
\section{Method}
 

First, we describe how we obtained various PTMs and created DSM embeddings for different models as well as how we fine-tuned/trained the classifiers for the studies. Then, we discuss the datasets and the study design. 

\subsection{Mixed-Domain Transfer Learning}
\label{tlm}
%In transfer learning, there are two steps. First, we get the pretrained embeddings, then we either fine-tune the pretrained model or use the embeddings to train a classifier. We get the pretrained embeddings from the following models: BERT, ELMo, Word2Vec, GloVe, as well as from variants of BERT and Transformer such as RoBERTa, ALBERT, and XLNet.

%In transfer learning, there are two steps. First, we get the pretrained embeddings, then we either fine-tune the pretrained model or use the embeddings to train a classifier. 

We use the following PTMs: BERT, RoBERTa, ALBERT, XLNet, ELMo, Word2Vec, and GloVe. 

\textbf{Deep PTMs: }We get the BERT base model (uncased) for sequence classification from the Hugging Face library \cite{wolf-etal-2020-transformers}. The embedding vectors are 768-dimensional. This BERT PTM adds a single linear layer on top of the BERT base model. The pretrained weights of all hidden layers of the PTM and the randomly initialized weights of the top classification layer are adapted during fine-tuning using a target dataset. The XLNet is obtained from the Hugging Face library \cite{wolf-etal-2020-transformers} and fine-tuned similar to BERT. Its embedding vectors are 768-dimensional. The RoBERTa (obtained from \cite{wolf-etal-2020-transformers}) and ALBERT (obtained from  \cite{maiya2020ktrain}) are used by first extracting embeddings from their final layer and then adding linear layers. While the RoBERTa embeddings are 768-dimensional, the ALBERT embeddings are 128-dimensional.


\textbf{Shallow PTMs: }We get the ELMo embeddings from TensorFlow-Hub \cite{tensorflow2015-whitepaper}. Each embedding vector has a length of 1024. The Word2Vec embeddings are obtained from Google Code \cite{google}. The embedding vectors are 300-dimensional. We get the GloVe pretrained 300-dimensional embeddings from \cite{pennington-etal-2014-glove}.

\textbf{CNN:} The ELMo, Word2Vec, and GloVe embeddings are used to train a CNN classifier with a single hidden layer \cite{Kim:2014}. The first layer is the embedding layer. Its dimension varies based on the dimension of pretrained embeddings. The second layer is the one-dimensional convolution layer that consists of 100 filters of dimension 5 x 5 with ``same'' padding and ReLU activation. The third layer is a one-dimensional global max-pooling layer, and the fourth layer is a dense layer with 100 units along with ReLU activation. The last layer is the classification layer with softmax activation. We use this setting for the CNN architecture as it was found empirically optimal in our experiments. We use cross-entropy as loss function, Adam as the optimizer, and a batch size of 128. The embedding vectors are kept fixed during the training \cite{Kim:2014}.



%Specifically, for pretrained BERT, XLNet, and RoBERTa, we download them directly from the transformer library \cite{wolf-etal-2020-transformers}. By following the guideline of transformer documentation, we are able to conveniently fine-tune BERT and XLNet models using a custom dataset (e.g., CoAID May data), and then test the fine-tuned models on a different dataset (e.g., CoAID July data). As for RoBERTa, we create a classifier on the top of pretrained RoBERTa model so that we can fine-tune RoBERTa as well as perform the classification task. This classifier has 5 layers, where the first layer is a dropout layer with a 0.4 0f dropout rate and the second layer is a linear layer with 768 of input size and 64 of output size. The third layer is a norm layer that normalizes the input and shape of output is the same as the input, and the fourth layer is another dropout layer with the same dropout rate as the previous dropout layer. The last layer is another linear layer with 64 of input size and 2 of output size. For the RoBERTa training process, firstly, we only train those linear layers by freezing the parameters of pretrained RoBERTa, and we use Adamw as an optimizer with 1e-4 of learning rate. Then we unfreeze those parameters and train both layers and RoBERTa, and use the same optimizer with 2e-6 of learning rate. Additionally, we download the ALBERT model from the Ktrain library \cite{maiya2020ktrain}, and train it with 3 epochs, 3e-5 of the learning rate, and 6 of batch size. 


\subsection{Domain-Specific Model (DSM) based Learning}

We create the DSMs using two approaches: graph-based and non-graph. For the graph-based approach, we use the following models: Text GCN and VGCN-BERT. For training the Text GCN model, we pre-process the data as follows. First, we clean the text by removing stop words and rare words whose frequencies are less than 5. Then, we build training, validation, and test graphs using the cleaned text. Finally, we train the GCN model using training and validation graphs and test the model using a test graph. During the training, early stopping is used.


For training the VGCN-BERT model, first, we clean the data that includes removing spaces, the special symbols as well as URLs. Then, the BERT tokenizer is used to create BERT vocabulary from the cleaned text. The next step is to create training, validation, and the test graphs. The last step is training the VGCN-BERT model. During the training, the model constructs embeddings from word and vocabulary GCN graph. 


For the non-graph approach, we create embeddings from the target dataset by using the Word2Vec and GloVe models. First, we pre-process the raw text data by converting the text (i.e., a list of sentences) into a list of lists containing tokenized words. During tokenization, we convert words to lowercase, remove words that are only one character, and lemmatize the words. We add bigrams that appear 10 times or more to our tokenized text. The bigrams allow us to create phrases that could be helpful for the model to learn and produce more meaningful representations. Then, we feed our final version of the tokenized text to the Word2Vec and the GloVe model for creating embeddings. After we obtain the embeddings, we use them to train the CNN classifier described in the previous sub-section, except that the domain-specific word embeddings are adapted during the training. 



%We use the skip-gram implementation of the Word2Vec model with 2 as window size, train it for 100 epochs, with min count 2 (total frequency of words lower than 2 are ignored), and use 0.01 as the threshold to randomly downsample higher-frequency words. For the GloVe model, we use a window size of 2, a learning rate of 0.05, and train the model for 100 epochs. The dimension of both Word2Vec and GloVe embeddings is 300. After we obtain the embeddings, we use them to train the CNN classifier described in the previous sub-section, except that the word embeddings are adapted during the training. 





\subsection{Dataset}

We use two COVID-19 datasets for the study, i.e., CoAID \cite{cui2020coaid} and CMU-MisCov19 \cite{memon2020characterizing}. 

The CoAID dataset contains two types of data: true information and misinformation. We use this dataset to investigate the generalizability of the models along three dimensions.

\begin{itemize}
    

    \item \textbf{Temporal dimension}: Train a model using data from an earlier time, then test its generalizability at different times in the future.
    
    \item \textbf{Size dimension}: Train models by varying the size of the training dataset.
    
    \item \textbf{Length dimension}: Train models by varying the length of the samples, e.g., tweet (short-length data) and news articles (lengthy data).  
    
   % \item Context dimension: Use tweets with replies to provide contextual information
    
\end{itemize}




The CMU-MisCov19 dataset is used to analyze a model's performance in fine-grained classification. 



%Besides, the sizes of both datasets are reduced because during the process of scraping tweets using Twitter API, some were deleted or not authorized to fetch. 

\subsubsection{CoAID: Binary Classification}



%\begin{figure}[!htb]
%  \centering
%  \includegraphics[width=\linewidth]{figures/tweets.png}
%  \caption{CoAID: Distribution of Tweets.}
%  \label{fig:coaid-tweet}
%\end{figure}
%
%\begin{figure}[!htb]
%  \centering
%  \includegraphics[width=\linewidth]{figures/reply.png}
%  \caption{CoAID: Distribution of Replies.}
%  \label{fig:coaid-reply}
%\end{figure}
%
%\label{coaid}
%\begin{figure}[!htb]
%  \centering
%  \includegraphics[width=\linewidth]{figures/news.png}
%  \caption{CoAID: Distribution of News Articles.}
%  \label{fig:coaid-news}
%\end{figure}

The CoAID dataset \cite{cui2020coaid} is used for binary classification since it has only two labels: 0 for misinformation and 1 for true information. This dataset contains two types of data: online news articles on COVID-19 and tweets related to those articles. Datasets of these two categories were collected at four different months in 2020: May, July, September, and November. Thus, the total number of CoAID datasets is 8. The class distribution is \textbf{heavily skewed} with significantly more true information samples than misinformation samples. Sample distribution per class (both for the tweets and news articles) is given in the appendix.

%There is also a reply tweet subset that includes replies to the original tweets.

%as shown in figure \ref{fig:coaid-tweet}, \ref{fig:coaid-reply}, and \ref{fig:coaid-news} 

%Figure \ref{fig:coaid-tweet}, \ref{fig:coaid-reply}, and \ref{fig:coaid-news} show the distributions of tweets, replies, and news articles, respectively. For tweets and replies, the sizes of May and July data are larger than that of September and November. Also, each category contains significantly more true information than misinformation. Thus, the CoAID data is heavily skewed.




\subsubsection{CMU-MisCov19: Fine-Grained Classification}

The CMU-MisCov19 dataset contains 4,573 annotated tweets \cite{memon2020characterizing}. The tweets were collected on three days in 2020: March 29, June 15, and June 24. The categories are fine-grained comprising of 17 classes with \textbf{skewed distribution}. This dataset does not have any true information category. Its sample distribution per class is given in the appendix.


%shown in Figure \ref{fig:cmu}

%\begin{figure}[!htb]
%  \centering
% % \includegraphics[width=\linewidth]{figures/cmu.png}
%  %\includegraphics[width=\linewidth]{figures/CMU-class-distribution-names.png} 
%  \includegraphics[width=\linewidth]{figures/CMU-class-distribution.png} 
%  \vspace{-4.00 mm}
%  \caption{CMU-MisCov19 Dataset: Class distribution.}
%  \vspace{-5.00 mm}
%  \label{fig:cmu}
%\end{figure}


%The CMU-MisCov19 dataset contains 4,573 annotated tweets, comprising 3629 users with an average of 1.24 tweets per user \cite{memon2020characterizing}.


%Figure \ref{fig:cmu} shows the number of tweets collected for each category. It is clear that the number of tweets for each category varies. Class 8 (calling out or correction) has the most tweets, while class 3 (true treatment) has 0 tweets which makes sense since there was no real treatment at that time. 


%\begin{enumerate}
%  \item Irrelevant: tweets that do not mention COVID-19.
%  \item Conspiracy: tweets that endorse a conspiracy story.
%  \item True treatment: tweets that endorse treatments verified by organizations such as the World Health Organization (WHO) or the Center of Disease Control and Prevention (CDC). 
%  \item True prevention: tweets that explicitly endorse a prevention method verified by WHO or CDC, etc.
%  \item Fake cure: tweets that endorse an unverified cure.
%  \item Fake treatment: tweets that endorse an unverified treatment.
%  \item False fact or prevention: tweets that implicitly or explicitly endorse a method or mention a false fact about COVID-19.
%  \item Calling out or correction: tweets that call out or report fake-related news, fake cures, or conspiracy theories. 
%  \item Sarcasm or satire: tweets that contain signs of satire or a clear job about fake cures or conspiracies. 
%  \item True public health response: tweets that contain a statement and link out to the official websites (e.g., CDC or WHO) which the statement can be verified. 
%  \item False public health response: tweets that contain a statement and link out to a website which the statement cannot be verified. 
%  \item Politics: tweets that implicitly comment on or provide commentary on actions taken by politicians.
%  \item Ambiguous or hard to classify: tweets that have no clear intention and can be classified as any of the previous categories. 
%  \item Commercial activity or promotion: tweets that include a company advertising or selling COVID-19-related products (e.g., face masks).
%  \item Emergency or emergency response: tweets that mention a viable emergence response.
%  \item News: tweets that cannot be classified in any of other categories and include a news story as well as a link to news websites.
%  \item Panic buying: tweets that talk about panic buying in the context of COVID-19.
%\end{enumerate}




%Figure \ref{fig:cmu} shows the number of tweets collected for each category. It is clear that the number of tweets for each category varies. Class 8 (calling out or correction) has the most tweets, while class 3 (true treatment) has 0 tweets which makes sense since there was no real treatment at that time. 


\subsection{Context Evolution in the COVID-19 Social Media Data}


We use the CoAID dataset to understand whether the context of the COVID-19 text evolves. To detect a change in the context over time, we investigate how the distribution of the high-frequency terms evolve for the two categories of the data: tweets and news articles. For each category, we select the top 10 high-frequency words from the 4 non-overlapping datasets belonging to 4 subsequent months, i.e., May, July, September, and November in 2020. Our goal is to determine whether there exists a temporal change in the distribution of high-frequency words.

%(ii) Which category of the data exhibits larger temporal change?



%We want to understand whether the context encoded in the CoAID datasets evolves over time. For this, we analyze the change in the temporal pattern in the word distribution. We focus on high-frequency words and see how they evolve over time. A significant change in the distribution of the high-frequency words reflects the shift in the context in a dataset.  
%
%More specifically, we investigate how the distribution of the high-frequency terms evolve for the 3 categories of the data: tweets, tweets \& replies, and news articles. For each category, we select the top 10 high-frequency words from the 4 non-overlapping datasets belonging to 4 subsequent months, i.e., May, July, September, and November in 2020. Our goal is to determine: 
%
%\begin{itemize}
%    \item Whether there exist temporal changes in the distribution of high-frequency words?
%    \item Which category of the data exhibits larger temporal change?
%\end{itemize}


%Specifically, we create wordcloud images which are based on words in each CoAID dataset in order to visually observe the most frequent words appeared in thos dataset. Figure \ref{fig:may-new-wordcloud}, \ref{fig:july-new-wordcloud}, \ref{fig:sept-new-wordcloud}, and \ref{fig:nove-new-wordcloud} are created using CoAID news articles. Figure \ref{fig:may-tweet-wordcloud}, \ref{fig:july-tweet-wordcloud}, \ref{fig:sept-tweet-wordcloud} and \ref{fig:nove-tweet-wordcloud} are created using CoAID Tweet dataset. Figure \ref{fig:may-tweetreply-wordcloud}, \ref{fig:july-tweetreply-wordcloud}, \ref{fig:sept-tweetreply-wordcloud}, and \ref{fig:nove-tweetreply-wordcloud} are created using CoAID tweet and reply data.

%To facilitate this word-frequency-based analysis, we also create word clouds. A word cloud is a visual representation of words. Higher frequency words are shown in larger fonts in proportion to their frequency.

%We also create charts to demonstrate the frequency of top 10 words for each dataset. We notice that for Tweet and Reply, the high-frequency words noticeably changed over the time. For example, May tweets are more related to the COVID-19, but Novmeber tweets involve the conversation about former president Trump and campaign. As for the news articles, there seems no obvious changes of word used in the articles.



%\subsubsection{Tweet: Study of Context Evolution}

Figure \ref{tweet-top10} shows context evolution in the tweets category. We see that during May, the two high-frequency words were covid and coronavirus. The frequent words represent broader concepts such as health, disease, spread, etc. However, over time the context shifted towards more loaded terms. For example, in July two new high-frequency words, such as mask and support, emerged. Then, in September words like contact, school, child, and travel became prominent. Finally, during November, we observe \textbf{a sharp change} in the nature of the frequent words. Terms with strong political connotations (e.g., trump, fauci, campaign, and vaccine) started emerging. The evolution in the high-frequency words indicates a temporal shift in the context in the tweets dataset. We observe similar context evolution in the news articles dataset, reported in the Appendix with additional analysis.

%which is also evidenced in the word clouds in Figure \ref{tweet-wordcloud}.

%Although there is context shifting in the Tweet dataset, some words are used each month. For instance, the word covid appears in each month, and also has the highest frequency for all months. Besides, the gap between the highest-frequency word and the high-frequency words is not big for September and November as compared to that for May and July.   


\begin{figure}[!htb]
    \begin{center}
        \subfigure[May]{\label{tweet-may}\includegraphics[width=2.80in]{figures/coaid-may-tweet-frequency.png}} \quad \vspace{-3.00mm}	
        \subfigure[July]{\label{tweet-july}\includegraphics[width=2.80in]{figures/coaid-july-tweet-frequency.png}} \\	 
        \subfigure[September]{\label{tweet-sept}\includegraphics[width=2.80in]{figures/coaid-sept-tweet-frequency.png}} \quad \vspace{-3.00mm}
        \subfigure[November]{\label{tweet-nov}\includegraphics[width=2.80in]{figures/coaid-nove-tweet-frequency.png}} \quad 


        %\vspace{-4.00mm}		
        \caption{CoAID (Tweets): Frequency of top 10 words in four datasets from four subsequent months.}
	 \vspace{-5.00mm}			
        \label{tweet-top10}
    \end{center}
\end{figure}


%
%\begin{figure}[!htb]
%    \begin{center}
%        \subfigure[May]{\label{tweet-wordcloud-may}\includegraphics[width=2.50in]{figures/CoAID-May-Tweet-WordCloud.png}} \quad	
%        \subfigure[July]{\label{tweet-wordcloud-july}\includegraphics[width=2.50in]{figures/CoAID-July-Tweet-WordCloud.png}} \\	
%        \subfigure[September]{\label{tweet-wordcloud-sept}\includegraphics[width=2.50in]{figures/CoAID-Sept-Tweet-WordCloud.png}} \quad
%        \subfigure[November]{\label{tweet-wordcloud-nov}\includegraphics[width=2.50in]{figures/CoAID-Nove-Tweet-WordCloud.png}} \quad
%        \caption{CoAID: Tweets Word Cloud}
%        \label{tweet-wordcloud}
%    \end{center}
%\end{figure}



%\subsubsection{Tweet \& Reply: Study of Context Evolution}
%
%Figure \ref{tweet-reply-top10} shows that by including replies, the highest frequency word for September is changed to the word mask, while for other months it is still the same. At the same time, new high-frequency words appear for each month, especially for July. More specifically, for May, a new word test has a high frequency. For July, news words such as like, school, and need have high frequencies. For September and November, a new word people has a high frequency. Additionally, the frequency of the top 4 words in November is greatly increased than that of other high-frequency words after including replies.
%
%Although there are new words that appeared after including replies, the frequency pattern between tweet only and tweet+frequency is not changed significantly for May and July, in which May still has two obvious high-frequency words and July has one highest frequency word. It is also noticeable that from figure \ref{tweet-reply-wordcloud}, the word cloud of May Tweet+Reply is slightly different from that of May Tweet, while other months' word clouds have more obvious differences. 


%\begin{figure}[htb!]
%    \begin{center}
%        \subfigure[May]{\label{tweet-reply-may}\includegraphics[width=2.50in]{figures/coaid-may-tweet-reply-frequency.png}} \quad	
%        \subfigure[July]{\label{tweet-reply-july}\includegraphics[width=2.50in]{figures/coaid-july-tweet-reply-frequency.png}} \\	
%        \subfigure[September]{\label{tweet-reply-sept}\includegraphics[width=2.50in]{figures/coaid-sept-tweet-reply-frequency.png}} \quad
%        \subfigure[November]{\label{tweet-reply-nov}\includegraphics[width=2.50in]{figures/coaid-nove-tweet-reply-frequency.png}} \quad
%        \caption{CoAID: Tweets \& Replies Frequency of Top 10 Words}
%        \label{tweet-reply-top10}
%    \end{center}
%\end{figure}


%\begin{figure}[htb!]
%    \begin{center}
%        \subfigure[May]{\label{tweet-reply-wordcloud-may}\includegraphics[width=2.50in]{figures/CoAID-May-Tweet-Reply-WordCloud.png}} \quad	
%        \subfigure[July]{\label{tweet-reply-wordcloud-july}\includegraphics[width=2.50in]{figures/CoAID-July-Tweet-Reply-WordCloud.png}} \\	
%        \subfigure[September]{\label{tweet-reply-wordcloud-sept}\includegraphics[width=2.50in]{figures/CoAID-Sept-Tweet-Reply-WordCloud.png}} \quad
%        \subfigure[November]{\label{tweet-reply-wordcloud-nov}\includegraphics[width=2.50in]{figures/CoAID-Nove-Tweet-Reply-WordCloud.png}} \quad
%        \caption{CoAID: Tweets \& Replies Word Cloud}
%        \label{tweet-reply-wordcloud}
%    \end{center}
%\end{figure}



%\subsubsection{News Articles: Study of Context Evolution}
%
%From Figure \ref{news-top10} we see that in the news articles datasets, the gap between the highest frequency word and the high-frequency words is much smaller as compared to that in the tweet and the tweet+reply datasets. However, we do observe a similar pattern in the change of context over time in the news articles datasets. For example, The May and July datasets have only 4 common high-frequency words: covid, coronavirus, health, data. In the July dataset, we observe the emergence of three new high-frequency words attack, security, and protect, which indicates a change in context. The context in the September dataset seems to be similar to that of the July dataset. These two datasets have 8 high-frequency words in common: covid, service, online, attack, security, health, information, coronavirus. The November dataset shares 7 common words with the September dataset: covid, service, online, attack, people, health, coronavirus. However, we notice an increase in the frequency in some words such as protect and attack. Also, a new word pandemic is seen to emerge. This shows a change in context. 
%
%%We gather similar observations about the context evolution from the word clouds in Figure \ref{news-wordcloud}.
%
%\begin{figure}[htb!]
%    \begin{center}
%        \subfigure[May]{\label{news-may}\includegraphics[width=2.50in]{figures/coaid-may-news-frequency.png}} \quad	
%        \subfigure[July]{\label{news-july}\includegraphics[width=2.50in]{figures/coaid-july-news-frequency.png}} \\	
%        \subfigure[September]{\label{news-sept}\includegraphics[width=2.50in]{figures/coaid-sept-news-frequency.png}} \quad
%        \subfigure[November]{\label{news-nov}\includegraphics[width=2.50in]{figures/coaid-nove-news-frequency.png}} \quad
%        \caption{CoAID: News Articles Frequency of Top 10 Words}
%        \label{news-top10}
%    \end{center}
%\end{figure}


%\begin{figure}[htb!]
%    \begin{center}
%        \subfigure[May]{\label{news-wordcloud-may}\includegraphics[width=2.50in]{figures/CoAID-May-News-WordCloud.png}} \quad	
%        \subfigure[July]{\label{news-wordcloud-july}\includegraphics[width=2.50in]{figures/CoAID-July-News-WordCloud.png}} \\	
%        \subfigure[September]{\label{news-wordcloud-sept}\includegraphics[width=2.50in]{figures/CoAID-Sept-News-WordCloud.png}} \quad
%        \subfigure[November]{\label{news-wordcloud-nov}\includegraphics[width=2.50in]{figures/CoAID-Nove-News-WordCloud.png}} \quad
%        \caption{CoAID: News Articles Word Cloud}
%        \label{news-wordcloud}
%    \end{center}
%\end{figure}

%A detailed analysis on the context evolution for each type of information is provided in the Appendix in chapter \ref{appendixA}.

















\subsection{Study Design}

We describe the design of the studies for comparing the NLP approaches for misinformation detection.

%For our Study 1 and Study 2, the category of replies in CoAID dataset is combined with the category of tweets. 

\subsubsection{Study 1}

Study 1 is designed to explore a model's generalizability in the \textbf{temporal dimension} of the data. We fine-tune/train a model using CoAID data collected from May 2020 and test it using data obtained from 3 different months in ``future'': July, September, and November. The following models are tested in this study: BERT (Mixed-domain Transfer Learning), ELMo (Mixed-domain Transfer Learning), Word2Vec (Mixed-domain Transfer Learning and DSM-based), GloVe (Mixed-domain Transfer Learning and DSM-based), Text-GCN (DSM-based), and VGCN-BERT (DSM-based).



\subsubsection{Study 2}

Study 2 is designed to test the performance of a model along the \textbf{length dimension}  of the data. We use both short-length data (tweets) and lengthy data (news articles). Specifically, we train a model using the CoAID Twitter dataset to understand a model's performance on the short-length data. Then, we train a model using the CoAID news articles dataset to study a model's performance on the lengthy data. The models used in this study are the same as in Study 1. 




\subsubsection{Study 3}

In study 3, we evaluate a model along the \textbf{size dimension}  of the data. We replicate studies 1 and 2 using a large target dataset, which is created by merging the datasets from May, July, and September. The November dataset is used as the test set. We experiment with two models for this study: BERT (Mixed-Domain Transfer Learning) and Word2Vec (DSM-based). 










\subsubsection{Study 4}

To further study the effectiveness of the Transformer-based mixed-domain transfer learning approach, we experiment with two variants of the BERT PTM, i.e., RoBERTa and ALBERT. In addition to this, we study the performance of an autoregressive model XLNet that induces the strength of BERT. For this study, we only use the news articles dataset.

%To further study the effectiveness of the Transformer-based mixed-domain transfer learning approach, we experiment with two variants of the BERT PTM, i.e., RoBERTa \cite{liu2019roberta} and ALBERT \cite{lan2020albert}. In addition to this, we study the performance of an autoregressive model XLNet \cite{yang2020xlnet} that induces the strength of BERT. These three PTMs are obtained from the Hugging Face library \cite{wolf-etal-2020-transformers}. For this study, we only use the news articles dataset.

\subsubsection{Study 5}

Study 5 is designed to test a model's performance on the fined-grained CMU-MisCov19 dataset. The models tested are the same as in Study 1.  


%\subsubsection{Study 4}
%
%Study 4 is focused solely on the BERT and Transformer based models. More specifically, we use pretrained embeddings obtained from variants of BERT and Transformer models such as RoBERTa, ALBERT, and XLNet.



==> 2021-EMNLP-Camera Ready/4.Results-Old.tex <==
\section{Results \& Analysis}

%Domain-Specific Pre-Trained Models (DSPTMs)

%We conduct extensive experiments to implement the studies described in the previous chapter. 
%
%The experiments for this research involve two steps: get the text embeddings (either from a pretrained model using a source dataset or create embeddings using the target dataset) and fine-tune or train a classifier. For the classifier model, we use CNN with 1D convolutional kernels. More specifically, in the transfer learning approach, we use the pretrained embeddings to fine-tune the model with the target data. We also use the pretrained embeddings to train a classifier. For the graph-based method, we create the graph embeddings using the target dataset, then train a classifier. Finally, for the target-based method, we create embeddings using the target dataset, then train a classifier. The experiments use diverse ML models.
%
%\begin{itemize}
%    \item Mixed-Domain Transfer Learning: we obtain the following PTMs - BERT, RoBERTa, ALBERT, XLNet, ELMo, Word2Vec, GloVe. Then, fine-tune the PTM (BERT, RoBERTa, ALBERT, XLNet) or fine-tune a CNN model using the embeddings from the PTM (ELMo, Word2Vec, GloVe)
%    
%    \item DSPTMs - Graph-based: Text GCN and VGCN BERT
%    
%    \item DSPTMs - Non-Graph: (a) for creating text embeddings, we use Word2Vec and GloVe; (b) then, using these embeddings train a single hidden layer CNN
%\end{itemize}
%
%We evaluate the performance of the models based on the accuracy, precision, recall, and f1 score. For each experiment, we average the results for 10 runs. The experiments are done using python's Scikit-learn \cite{scikit-learn} and TensorFlow 2.0 \cite{tensorflow2015-whitepaper} libraries. For training the Word2Vec model, we used the Gensim \cite{gensim} library. 

%\subsection{Experimental Setting}
%
%Table \ref{experimental_setting} and \ref{epochs} show the experimental setting for the studies. 
%
%\begin{table}[!htb]
%\caption{Experimental Setting}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|p{2.0cm}|p{2.0cm}|p{2.0cm}|p{2.4cm}|p{1.2cm}|p{1.7cm}|p{1.6cm}|}  
%\hline
%     					& Embedding Dimension 		& \# Hidden Layers 		& \# Neurons (hidden, final) 	& Batch Size 		& Optimizer 		& Learning Rate \\ \hline
%BERT         			&  768                   			&   12              			&      (768,2)                         	& 32           		& AdamW          	& 2e-5              \\ \hline
%ELMo         			& 1024                    			&   5               			&      (1024,2)                        	& 128           		& Adam          		& 0.001             \\ \hline
%RoBERTa      			& 768                    			&   12             			&      (768,2)                  		&  16          		& AdamW           	& 2e-6             \\ \hline
%ALBERT       			& 128                    			&   12             			&      (128,2)                        	& 6           			& Adam        		& 3e-5              \\ \hline
%XLNet        			& 768                    			&  12                			&      (768,2)                        	&  32          		& AdamW          	& 2e-5               \\ \hline
%Text GCN     			& 200                   			&   2              			&      (200,2)                      		& NA          		& Adam           		& 0.02            \\ \hline
%VGCN BERT    		& 216                    			&   18              			&      (216,2)                      		& 16           		& Adam           		& 2e-5            \\ \hline
%Word2Vec     			& 300                   			&   2              			&      (300,2)                      		& 128           		& Adam          		& 0.001              \\ \hline
%GloVe        			& 300                    			&   2               			&      (300,2)                       	& 128           		& Adam       		& 0.001               \\ \hline
%\end{tabular}}
%\label{experimental_setting}
% \end{center}
%\end{table}
%
%\begin{table}[!htb]
%\caption{Epochs: Datasets}
%\begin{center}
%\begin{tabular}{|l|l|}
%\hline
%                      			& Epochs 		\\ \hline
%CoAID (Tweet)         	& 5     		 \\ \hline
%CoAID (Tweet + Reply) 	& 4     		 \\ \hline
%CoAID (News Articles) 	& 10     		\\ \hline
%CMU-MisCov19          	& 10     		\\ \hline
%\end{tabular}
%\label{epochs}
%\end{center}
%\end{table}
%

%\subsection{Results}

We describe the results obtained from five studies. We evaluate the performance of the models based on the accuracy, precision, recall, and f1 score. For each experiment, we average the results for 10 runs. The experiments are done using python's Scikit-learn \cite{scikit-learn} and TensorFlow 2.0 \cite{tensorflow2015-whitepaper} libraries. For training the Word2Vec model, we used the Gensim \cite{gensim} library. 

%The description is divided into two parts, based on two datasets, i.e., CoAID (for binary classification) and CMU-MisCov19 (for fine-grained classification).

%\subsection{Binary Classification: CoAID Dataset}


%Table \ref{CoAID-Tweet}, Table \ref{CoAID-Reply}, and Table \ref{CoAID-news} show the results from studies 1 and 2. 



%Table \ref{CoAID-Tweet} and Table \ref{CoAID-news} show the results from studies 1 and 2. 


\begin{table*}[!htb]
\caption{Study 1 \& 2: CoAID - Tweet (Temporal \& Text Length Dimension)}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.942} &
  \multicolumn{6}{c|}{Accuracy = 0.990} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{BERT}} &
  \multicolumn{1}{l|}{0.981} &
  0.997 &
  0.989 &
  0.281 &
  {\color[HTML]{000000} 0.079} &
  0.116 &
  \multicolumn{1}{l|}{0.946} &
  0.996 &
  0.970 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{1.00} &
  0.990 &
  0.995 &
  0.500 &
  1.00 &
  0.670 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.941} &
  \multicolumn{6}{c|}{Accuracy = 0.990} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{ELMo}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.945} &
  0.995 &
  0.970 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.990} &
  1.00 &
  0.995 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.932} &
  \multicolumn{6}{c|}{Accuracy = 0.969} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.949} &
  0.980 &
  0.964 &
  0.20 &
  0.09 &
  0.12 &
  \multicolumn{1}{l|}{0.99} &
  0.979 &
  0.984 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.943} &
  \multicolumn{6}{c|}{Accuracy = 1.00} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  0.31 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  0.998 &
  0.971 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{1.00} &
  1.00 &
  1.00 &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
   {\color[HTML]{FE0000} {\ul \textbf{1.00}}}  \\ \hline
\multicolumn{19}{|c|}{\textbf{DSPTMs - Graph-based}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Text GCN}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.029 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.95 &
  1.00 &
  0.97 &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.99 &
  1.00 &
  0.99 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.971} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{VGCN-BERT}} &
  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  {\color[HTML]{FE0000} {\ul \textbf{0.495}}} &
  0.019 &
  0.035 &
  \multicolumn{1}{l|}{0.947} &
  0.999 &
  0.972 &
  {\color[HTML]{FE0000} {\ul \textbf{0.287}}} &
  0.029 &
  0.052 &
  \multicolumn{1}{l|}{0.994} &
  0.977 &
  0.984 &
  0.21 &
  0.389 &
  0.246 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSPTMs - Non-Graph}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.977} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.979} &
  0.997 &
  0.988 &
  0.11 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  1.00 &
  0.972 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.99} &
  1.00 &
  0.995 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.979} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  0.23 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  1.00 &
  0.972 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.99} &
  0.99 &
  0.99 &
  0.00 &
  0.00 &
  0.00 \\ \hline
\end{tabular}}
\end{center}
\label{CoAID-Tweet}
\end{table*}







%\begin{table*}[!htb]
%\caption{Study 1: CoAID - Tweet}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|c|c|c|c|c|c|c|cc}
%\cline{1-7}
%\textbf{Train: May}                 & \multicolumn{2}{c|}{\textbf{Test: July}}                                                                                                                                                                                 & \multicolumn{2}{c|}{\textbf{Test: September}}                                                                                                                                                                            & \multicolumn{2}{c|}{\textbf{Test: November}}                                                                                                                                                                             &  &  \\ \cline{1-7}
%                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          &  &  \\ \cline{1-7}
%\multirow{2}{*}{BERT}      & \multicolumn{2}{c|}{Accuracy = 0.978}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.942}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.981\\ 0.997\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.281\\ 0.079\\ 0.116\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.946\\ 0.996\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}1.000\\ 0.990\\ 0.995\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.500\\ 1.000\\ 0.670\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{ELMo}      & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.941}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 1.000\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.945\\ 0.995\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 1.000\\ 0.995\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.932}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.969}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 1.000\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 0.980\\ 0.964\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.200\\ 0.090\\ 0.120\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 0.979\\ 0.984\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%GloVe                      & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.943}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 1.000}                                                                                                                                                                           &  &  \\ \cline{1-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.999\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.310\\ 0.020\\ 0.030\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.946\\ 0.998\\ 0.971\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}1.000\\ 1.000\\ 1.000\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}1.000\\ 1.000\\ 1.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Graph Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &  &  \\ \cline{1-7}
%\multirow{2}{*}{Text-GCN}  & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 1.000\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.029\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.950\\ 1.000\\ 0.970\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.990\\ 1.000\\ 0.990\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{VGCN-BERT} & \multicolumn{2}{c|}{Accuracy = 0.978}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.971}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.999\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.495\\ 0.019\\ 0.035\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.947\\ 0.999\\ 0.972\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.287\\ 0.029\\ 0.052\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.994\\ 0.977\\ 0.984\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.210\\ 0.389\\ 0.246\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Target Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.977}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.997\\ 0.988\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.110\\ 0.020\\ 0.030\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.946\\ 1.000\\ 0.972\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 1.000\\ 0.995\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{GloVe}     & \multicolumn{2}{c|}{Accuracy = 0.978}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.999\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.230\\ 0.020\\ 0.030\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.946\\ 1.000\\ 0.972\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 0.990\\ 0.990\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\end{tabular}}
%\end{center}
%\label{CoAID-Tweet}
%\end{table*}
%

%\end{tabular}
% \end{table}
% \label{coaid-tweet}
% }

%For the July tweet test dataset (Table \ref{CoAID-Tweet}), VGCN-BERT has the highest precision, and BERT has the highest recall and f1 scores that are slightly better than other models. For September, the Text-GCN has outstanding performance for detecting misinformation, but its performance on true information is extremely poor. In addition, other models perform poorly on misinformation. For November, the transfer learning approach GloVe has an excellent performance on both true information and misinformation, where precision, recall, and f1 scores are 1. Text-GCN also has decent scores on misinformation, and BERT performance on both true information and misinformation is also good. However, we notice that no model performs well across three different test datasets. This observation \textbf{confirms hypothesis 2}, i.e., transfer learning is not robust when there is context change happened in the data. It also \textbf{confirms hypothesis 5}, i.e., the hybrid method VGCN-BERT does not significantly improve the performance as compared to BERT and Text-GCN.

Table \ref{CoAID-Tweet} and Table \ref{CoAID-news} show the results from studies 1 and 2. For the July tweet test dataset (Table \ref{CoAID-Tweet}), VGCN-BERT has the highest precision, and BERT has the highest recall and f1 scores. These scores are slightly better than other models. For September, the Text-GCN has outstanding performance for detecting misinformation, but its performance on true information is extremely poor. In addition to this, other models perform poorly on misinformation. For November, the GloVe-based transfer learning approach achieves an excellent performance on both true information and misinformation, where precision, recall, and f1 scores are 1. Text-GCN also has decent scores on misinformation. The performance of BERT on both true information and misinformation is also good. However, we notice that no model performs well across three different test datasets. Thus we see that \textbf{mixed-domain transfer learning is not robust when context of the data changes}. 

%We also notice that the hybrid method VGCN-BERT does not significantly improve the performance as compared to BERT and Text-GCN.



%\begin{table}[!htb]
%\caption{Study 1: CoAID - Tweet\&Reply}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|c|c|c|c|c|c|c|cc}
%\cline{1-7}
%\textbf{Train: May}                 & \multicolumn{2}{c|}{\textbf{Test: July}}                                                                                                                                                                                 & \multicolumn{2}{c|}{\textbf{Test: September}}                                                                                                                                                                            & \multicolumn{2}{c|}{\textbf{Test: November}}                                                                                                                                                                             &  &  \\ \cline{1-7}
%                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          &  &  \\ \cline{1-7}
%\multirow{2}{*}{BERT}      & \multicolumn{2}{c|}{Accuracy = 0.962}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.941}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.937}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.978\\ 0.983\\ 0.981\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.101\\ 0.078\\ 0.089\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 0.991\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.033\\ 0.006\\ 0.010\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.939\\ 0.967\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.049\\ 0.500\\ 0.088\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{ELMo}      & \multicolumn{2}{c|}{Accuracy = 0.977}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.949}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.994}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.977\\ 1.000\\ 0.988\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 1.000\\ 0.974\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.994\\ 1.000\\ 0.997\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.964}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.919}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.951}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.984\\ 0.982\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.160\\ 0.130\\ 0.150\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.948\\ 0.968\\ 0.958\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.020\\ 0.020\\ 0.020\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.954\\ 0.975\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.060\\ 0.500\\ 0.110\end{tabular}                                         &  &  \\ \cline{1-7}
%GloVe                      & \multicolumn{2}{c|}{Accuracy = 0.965}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.939}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.915}                                                                                                                                                                           &  &  \\ \cline{1-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.981\\ 0.983\\ 0.982\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.230\\ 0.210\\ 0.220\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.951\\ 0.987\\ 0.969\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.160\\ 0.050\\ 0.070\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.918\\ 0.956\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.040\\ 0.500\\ 0.070\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Graph Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &  &  \\ \cline{1-7}
%\multirow{2}{*}{Text-GCN}  & \multicolumn{2}{c|}{Accuracy = 0.977}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.949}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.994}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.977\\ 1.000\\ 0.988\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 1.000\\ 0.974\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.994\\ 1.000\\ 0.997\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{VGCN-BERT} & \multicolumn{2}{c|}{Accuracy = 0.976}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.942}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.987}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.978\\ 0.998\\ 0.988\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.282\\ 0.039\\ 0.067\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.950\\ 0.991\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.115\\ 0.015\\ 0.022\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.995\\ 0.992\\ 0.993\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.111\\ 0.194\\ 0.134\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Target Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.972}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.939}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.975}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.977\\ 0.994\\ 0.986\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.070\\ 0.020\\ 0.030\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 0.989\\ 0.969\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.995\\ 0.979\\ 0.987\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.070\\ 0.250\\ 0.110\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{GloVe}     & \multicolumn{2}{c|}{Accuracy = 0.962}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.939}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.984}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.977\\ 0.984\\ 0.981\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.060\\ 0.040\\ 0.050\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 0.989\\ 0.969\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.987\\ 0.992\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.180\\ 0.500\\ 0.270\end{tabular}                                         &  &  \\ \cline{1-7}
%\end{tabular}}
%\end{center}
%\label{CoAID-Reply}
%\end{table}


%Table \ref{CoAID-Reply} shows the result of the CoAID tweet and reply. For July, the transfer learning approach GloVe has the highest recall, and f1 scores for misinformation and VGCN-BERT has the highest precision. For September, the transfer learning approach GloVe has the highest precision, recall, and f1 scores for misinformation. For November, the transfer learning approaches BERT, GloVe, and Word2Vec as well as target-based approach GloVe has the highest recall score for misinformation. In addition, the target-based approach GloVe also has the highest precision and f1 score. However, there is \textbf{no single model that provides an effective solution for misinformation detection for all three different test datasets}. This result \textbf{confirms hypothesis 2}, i.e., the transfer learning approaches do not improve the performance significantly after we increase the training size. It also further \textbf{confirms hypothesis 5}, i.e., the hybrid method VGCN-BERT is slightly better than that of both BERT and Text-GCN for misinformation classification.






\begin{table*}[!htb]
\caption{Study 1 \& 2: CoAID - News Articles (Temporal \& Text Length Dimension))}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.646} &
  \multicolumn{6}{c|}{Accuracy = 0.503} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{BERT}} &
  \multicolumn{1}{l|}{0.814} &
  1.00 &
  0.898 &
  0.00 &
  {\color[HTML]{000000} 0.00} &
  0.00 &
  \multicolumn{1}{l|}{0.929} &
  0.676 &
  0.779 &
  0.018 &
  0.135 &
  0.036 &
  \multicolumn{1}{l|}{0.962} &
  0.511 &
  0.656 &
  0.009 &
  0.144 &
  0.009 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.559} &
  \multicolumn{6}{c|}{Accuracy = 0.973} &
  \multicolumn{6}{c|}{Accuracy = 0.985} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{ELMo}} &
  \multicolumn{1}{l|}{0.777} &
  0.642 &
  0.703 &
  0.11 &
  0.19 &
  0.14 &
  \multicolumn{1}{l|}{0.979} &
  0.993 &
  0.986 &
  {\color[HTML]{FE0000} {\ul \textbf{0.83}}} &
  0.64 &
  {\color[HTML]{FE0000} {\ul \textbf{0.72}}} &
  \multicolumn{1}{l|}{0.986} &
  0.99 &
  0.992 &
  0.88 &
  0.37 &
  0.52 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.851} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.98} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.846} &
  0.999 &
  0.916 &
  0.98 &
  0.20 &
  0.33 &
  \multicolumn{1}{l|}{0.948} &
  0.998 &
  0.972 &
  0.60 &
  0.06 &
  0.12 &
  \multicolumn{1}{l|}{0.98} &
  1.00 &
  0.99 &
  1.00 &
  0.11 &
  0.19 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.599} &
  \multicolumn{6}{c|}{Accuracy = 0.953} &
  \multicolumn{6}{c|}{Accuracy = 0.984} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.833} &
  0.635 &
  0.721 &
  0.22 &
  0.44 &
  0.29 &
  \multicolumn{1}{l|}{0.957} &
  0.995 &
  0.975 &
  0.73 &
  0.23 &
  0.35 &
  \multicolumn{1}{l|}{0.985} &
  0.999 &
  0.992 &
  {\color[HTML]{000000} 0.86} &
  {\color[HTML]{000000} 0.32} &
  0.46 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSPTMs - Graph-based}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.635} &
  \multicolumn{6}{c|}{Accuracy = 0.978} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Text GCN}} &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.81 &
  1.00 &
  0.90 &
  \multicolumn{1}{l|}{0.97} &
  0.633 &
  0.766 &
  0.095 &
  0.66 &
  0.165 &
  \multicolumn{1}{l|}{0.978} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.677} &
  \multicolumn{6}{c|}{Accuracy = 0.64} &
  \multicolumn{6}{c|}{Accuracy = 0.458} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{VGCN-BERT}} &
  \multicolumn{1}{l|}{0.971} &
  0.622 &
  0.758 &
  {\color[HTML]{000000} 0.356} &
  0.917 &
  0.513 &
  \multicolumn{1}{l|}{0.985} &
  0.628 &
  0.767 &
  {\color[HTML]{000000} 0.117} &
  0.839 &
  0.205 &
  \multicolumn{1}{l|}{0.989} &
  0.451 &
  0.619 &
  0.031 &
  0.778 &
  0.06 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSPTMs - Non-Graph}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.96} &
  \multicolumn{6}{c|}{Accuracy = 0.643} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.957} &
  0.984 &
  0.975 &
  {\color[HTML]{FE0000} {\ul \textbf{0.92}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.85}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.89}}} &
  \multicolumn{1}{l|}{0.977} &
  0.638 &
  0.772 &
  0.11 &
  {\color[HTML]{FE0000} {\ul \textbf{0.74}}} &
  0.19 &
  \multicolumn{1}{l|}{0.991} &
  0.99 &
  0.995 &
  {\color[HTML]{FE0000} {\ul \textbf{0.92}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.58}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.71}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.554} &
  \multicolumn{6}{c|}{Accuracy = 0.623} &
  \multicolumn{6}{c|}{Accuracy = 0.452} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.775} &
  0.637 &
  0.699 &
  0.10 &
  0.19 &
  0.13 &
  \multicolumn{1}{l|}{0.941} &
  0.641 &
  0.763 &
  0.05 &
  0.32 &
  0.09 &
  \multicolumn{1}{l|}{0.962} &
  0.457 &
  0.62 &
  0.01 &
  0.21 &
  0.02 \\ \hline
\end{tabular}}
\end{center}
\label{CoAID-news}
\end{table*}










%\begin{table*}[!htb]
%\caption{Study 1: CoAID - News Articles}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|c|c|c|c|c|c|c|cc}
%\cline{1-7}
%\textbf{Train: May}                 & \multicolumn{2}{c|}{\textbf{Test: July}}                                                                                                                                                                                 & \multicolumn{2}{c|}{\textbf{Test: September}}                                                                                                                                                                            & \multicolumn{2}{c|}{\textbf{Test: November}}                                                                                                                                                                             &  &  \\ \cline{1-7}
%                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          &  &  \\ \cline{1-7}
%\multirow{2}{*}{BERT}      & \multicolumn{2}{c|}{Accuracy = 0.814}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.646}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.503}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.814\\ 1.000\\ 0.898\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.929\\ 0.676\\ 0.779\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.018\\ 0.135\\ 0.036\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.962\\ 0.511\\ 0.656\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.009\\ 0.144\\ 0.009\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{ELMo}      & \multicolumn{2}{c|}{Accuracy = 0.559}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.973}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.985}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.777\\ 0.642\\ 0.703\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.110\\ 0.190\\ 0.140\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.993\\ 0.986\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.830\\ 0.640\\ 0.720\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.986\\ 0.999\\ 0.992\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.880\\ 0.370\\ 0.520\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.851}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.980}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.846\\ 0.999\\ 0.916\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.980\\ 0.200\\ 0.330\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.948\\ 0.998\\ 0.972\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.600\\ 0.060\\ 0.120\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.980\\ 1.000\\ 0.990\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}1.000\\ 0.110\\ 0.190\end{tabular}                                         &  &  \\ \cline{1-7}
%GloVe                      & \multicolumn{2}{c|}{Accuracy = 0.599}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.953}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.984}                                                                                                                                                                           &  &  \\ \cline{1-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.833\\ 0.635\\ 0.721\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.220\\ 0.440\\ 0.290\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.957\\ 0.995\\ 0.975\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.730\\ 0.230\\ 0.350\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.985\\ 0.999\\ 0.992\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.860\\ 0.320\\ 0.460\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Graph Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &  &  \\ \cline{1-7}
%\multirow{2}{*}{Text-GCN}  & \multicolumn{2}{c|}{Accuracy = 0.814}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.635}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.978}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.810\\ 1.000\\ 0.900\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.970\\ 0.633\\ 0.766\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.095\\ 0.660\\ 0.165\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.978\\ 1.000\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{VGCN-BERT} & \multicolumn{2}{c|}{Accuracy = 0.677}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.640}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.458}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.971\\ 0.622\\ 0.758\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.356\\ 0.917\\ 0.513\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.985\\ 0.628\\ 0.767\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.117\\ 0.839\\ 0.205\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.989\\ 0.451\\ 0.619\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.031\\ 0.778\\ 0.060\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Target Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.960}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.643}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.957\\ 0.984\\ 0.975\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.920\\ 0.850\\ 0.890\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.977\\ 0.638\\ 0.772\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.110\\ 0.740\\ 0.190\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.991\\ 0.999\\ 0.995\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.920\\ 0.580\\ 0.710\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{GloVe}     & \multicolumn{2}{c|}{Accuracy = 0.554}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.623}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.452}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.775\\ 0.637\\ 0.699\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.100\\ 0.190\\ 0.130\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.941\\ 0.641\\ 0.763\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.050\\ 0.320\\ 0.090\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.962\\ 0.457\\ 0.620\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.010\\ 0.210\\ 0.020\end{tabular}                                         &  &  \\ \cline{1-7}
%\end{tabular}}
%\end{center}
%\label{CoAID-news}
%\end{table*}


%Table \ref{CoAID-news} shows the result of CoAID news articles. For the July test dataset, both Text-GCN and target-based Word2Vec achieve decent precision, recall, and f1 scores on misinformation. However, Text-GCN has extremely poor performance on true information. For September, ELMo has the best precision and f1 score, while target based Word2Vec has the best recall score. As for November, both transfer learning and target-based Word2Vec obtain optimal precision score and Word2Vec also has the highest f1 score. Besides, VGCN-BERT has the highest recall score. We notice that target-based Word2Vec achieves overall high performance across all test datasets. This result \textbf{confirms hypothesis 6}, i.e., target-based embeddings can capture both global and local relationships to create an effective classifier. It also \textbf{confirms hypothesis 4}, i.e., the performance of graph-based approaches on lengthy texts is not as good as on short texts.  


Table \ref{CoAID-news} shows the result of CoAID news articles. For the July test dataset, both Text-GCN and target-based Word2Vec (DSPTM-based) achieve decent precision, recall, and f1 scores on misinformation. However, Text-GCN has extremely poor performance on true information. For September, ELMo has the best precision and f1 score, while Word2Vec (DSPTM-based) has the best recall score. As for November, both transfer learning and DSPTM-based Word2Vec obtain optimal precision score, and Word2Vec (DSPTM-based) has the highest f1 score. Besides, VGCN-BERT has the highest recall score. We notice that the DSPTM-based Word2Vec achieves overall high performance across all test datasets. Thus, the \textbf{non-graph DSPTM-based embeddings can capture both global and local relationships to create an effective classifier}. The performance of the graph-based DSPTM approach on lengthy texts is not as good as on short texts.  



\begin{table*}[!htb]
\caption{Study 3: CoAID Large Dataset (Dataset Size Dimension)}
\begin{center}
\scalebox{0.66}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train: May + July + September\\ Test: November\end{tabular}}} &
  \multicolumn{6}{c|}{\textbf{Tweet}} &
  \multicolumn{6}{c|}{\textbf{News Articles}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.928} &
  \multicolumn{6}{c|}{Accuracy = 0.992} \\ \cline{2-13} 
\multirow{-2}{*}{\textbf{Mixed-Domain Transfer Learning: BERT}} &
  \multicolumn{1}{l|}{1.00} &
  0.927 &
  0.962 &
  0.12 &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
  0.22 &
  \multicolumn{1}{l|}{0.994} &
  0.998 &
  0.996 &
  {\color[HTML]{FE0000} {\ul \textbf{0.883}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.719}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.787}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.985} &
  \multicolumn{6}{c|}{Accuracy = 0.986} \\ \cline{2-13} 
\multirow{-2}{*}{\textbf{DSPTMs - Non-Graph: Word2Vec}} &
  \multicolumn{1}{l|}{0.99} &
  0.995 &
  0.992 &
  {\color[HTML]{FE0000} {\ul \textbf{0.71}}} &
  {\color[HTML]{000000} 0.63} &
  {\color[HTML]{FE0000} {\ul \textbf{0.67}}} &
  \multicolumn{1}{l|}{0.992} &
  0.994 &
  0.993 &
  {\color[HTML]{000000} 0.71} &
  0.63 &
  {\color[HTML]{000000} 0.67} \\ \hline
\end{tabular}}
\end{center}
\label{CoAID-Big}
\end{table*}




%
%\begin{table*}[!htb]
%\caption{CoAID Large Dataset Experiment Result}
%\begin{center}
%\scalebox{0.56}{
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Train:} \\\textbf{May + July + September} \\ \textbf{Test: November}\end{tabular}} & \multicolumn{2}{c|}{\textbf{Tweet}}                                                                                                                                                                                      & \multicolumn{2}{c|}{\textbf{Tweet + Reply}}                                                                                                                                                                              & \multicolumn{2}{c|}{\textbf{News Articles}}                                                                                                                                                                              \\ \hline
%\multicolumn{1}{|l|}{}                                                                                      & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} \\ \hline
%\multicolumn{7}{|l|}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
%\multirow{2}{*}{BERT}                                                                                       & \multicolumn{2}{c|}{Accuracy = 0.928}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.981}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.992}                                                                                                                                                                           \\ \cline{2-7} 
%                                                                                                            & \begin{tabular}[c]{@{}c@{}}1.000\\ 0.927\\ 0.962\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.120\\ 1.000\\ 0.220\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 0.990\\ 0.990\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.789\\ 0.764\\ 0.773\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.994\\ 0.998\\ 0.996\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.883\\ 0.719\\ 0.787\end{tabular}                                         \\ \hline
%\multirow{2}{*}{Word2Vec (Target Based)}                                                                    & \multicolumn{2}{c|}{Accuracy = 0.985}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.961}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.986}                                                                                                                                                                           \\ \cline{2-7} 
%                                                                                                            & \begin{tabular}[c]{@{}c@{}}0.990\\ 0.995\\ 0.992\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.710\\ 0.630\\ 0.670\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.964\\ 0.980\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.710\\ 0.630\\ 0.670\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.992\\ 0.994\\ 0.993\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.710\\ 0.630\\ 0.670\end{tabular}                                         \\ \hline
%\end{tabular}}
%\end{center}
%\label{CoAID-Big}
%\end{table*}


%Table \ref{CoAID-Big} shows the results of large-dataset-based experiments. The performance of target-based Word2Vec further \textbf{confirms hypothesis 6}, i.e., the target-based text embeddings capture both global and local relationships if we increase the size of short-length training data (i.e., tweets). Its scores on misinformation for tweet or tweet and reply datasets increase significantly. 

Table \ref{CoAID-Big} shows the results of study 3, i.e., large-dataset-based experiments. The performance of DSPTM-based Word2Vec endorses the previous observation, i.e., \textbf{the non-graph DSPTM-based text embeddings capture both global and local relationships if we increase the size of short-length training data (i.e., tweets)}. Its F1 score on misinformation for tweet dataset increases significantly. 





\begin{table*}[!htb]
\caption{Study 4: CoAID Large Dataset (Various Transformer Models)}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.611} &
  \multicolumn{6}{c|}{Accuracy = 0.943} &
  \multicolumn{6}{c|}{Accuracy = 0.993} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{ALBERT}} &
  \multicolumn{1}{l|}{0.858} &
  0.625 &
  0.723 &
  0.25 &
  {\color[HTML]{000000} 0.547} &
  0.343 &
  \multicolumn{1}{l|}{0.96} &
  0.981 &
  0.97 &
  0.483 &
  0.298 &
  0.368 &
  \multicolumn{1}{l|}{0.996} &
  0.996 &
  0.996 &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.936} &
  \multicolumn{6}{c|}{Accuracy = 0.630} &
  \multicolumn{6}{c|}{Accuracy = 0.980} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{RoBERTa}} &
  \multicolumn{1}{l|}{0.937} &
  0.987 &
  0.962 &
  {\color[HTML]{FE0000} {\ul \textbf{0.925}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.711}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.804}}} &
  \multicolumn{1}{l|}{0.952} &
  0.641 &
  0.766 &
  {\color[HTML]{000000} 0.068} &
  0.447 &
  {\color[HTML]{000000} 0.118} &
  \multicolumn{1}{l|}{0.991} &
  0.989 &
  0.990 &
  0.55 &
  0.579 &
  0.564 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.97} &
  \multicolumn{6}{c|}{Accuracy = 0.456} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{XLNET}} &
  \multicolumn{1}{l|}{0.81} &
  1.00 &
  0.90 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.97} &
  1.00 &
  0.98 &
  {\color[HTML]{FE0000} {\ul \textbf{0.89}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.53}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.67}}} &
  \multicolumn{1}{l|}{0.97} &
  0.46 &
  0.62 &
  0.01 &
  0.26 &
  0.02 \\ \hline
\end{tabular}}
\end{center}
\label{CoAID-bert-variants}
\end{table*}

%\begin{table*}[!htb]
%\caption{CoAID - News Articles Using Variants of BERT and Transformer}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\multicolumn{1}{|l|}{\textbf{Train: May}} & \multicolumn{2}{c|}{\textbf{Test: July}}                                                                                                                                                                                 & \multicolumn{2}{c|}{\textbf{Test: September}}                                                                                                                                                                            & \multicolumn{2}{c|}{\textbf{Test: November}}                                                                                                                                                                             \\ \hline
%\multicolumn{1}{|l|}{}           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} \\ \hline
%\multicolumn{7}{|c|}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
%\multirow{2}{*}{ALBERT}          & \multicolumn{2}{c|}{Accuracy = 0.611}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.943}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.993}                                                                                                                                                                           \\ \cline{2-7} 
%                                 & \begin{tabular}[c]{@{}c@{}}0.858\\ 0.625\\ 0.723\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.250\\ 0.547\\ 0.343\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.960\\ 0.981\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.483\\ 0.298\\ 0.368\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.996\\ 0.996\\ 0.996\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.842\\ 0.842\\ 0.842\end{tabular}                                         \\ \hline
%\multirow{2}{*}{RoBERTa}         & \multicolumn{2}{c|}{Accuracy = 0.936}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.630}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.980}                                                                                                                                                                           \\ \cline{2-7} 
%                                 & \begin{tabular}[c]{@{}c@{}}0.937\\ 0.987\\ 0.962\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.925\\ 0.711\\ 0.804\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.952\\ 0.641\\ 0.766\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.068\\ 0.447\\ 0.118\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.991\\ 0.989\\ 0.990\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.550\\ 0.579\\ 0.564\end{tabular}                                         \\ \hline
%\multirow{2}{*}{XLNET}           & \multicolumn{2}{c|}{Accuracy = 0.814}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.970}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.456}                                                                                                                                                                           \\ \cline{2-7} 
%                                 & \begin{tabular}[c]{@{}c@{}}0.810\\ 1.000\\ 0.900\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.970\\ 1.000\\ 0.980\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.890\\ 0.530\\ 0.670\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.970\\ 0.460\\ 0.620\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.010\\ 0.260\\ 0.020\end{tabular}                                         \\ \hline
%\end{tabular}}
%\end{center}
%\label{CoAID-bert-variants}
%\end{table*}

Table \ref{CoAID-bert-variants} shows the results obtained from study 4. For the July test dataset misinformation detection, RoBERTa achieves the best performance, while XLNet shows the worst performance. However, for September misinformation, XLNet obtains the best performance, while the RoBERTa has the worst performance. As for November misinformation, ALBERT achieves the best performance, while XLNet has the worst performance. These results corroborate our previous observation on the mixed-domain transfer learning approach, i.e., it is not robust when context of the data changes. 


%These results \textbf{confirm hypothesis 2} because none of these models maintain the performance when the context in the data changes.




\subsubsection{Result: Fine-Grained CMU-MisCov19 Dataset}
\begin{figure*}[h]
  \centering
  %\includegraphics[width=\linewidth]{figures/cmu-result-graph.png}
  \includegraphics[width=4.5in]{figures/cmu-result-graph.png}
  \caption{Study 5: CMU-MisCov19 (Fine-Grained Classification)}
  \label{fig:cmu-graph}
\end{figure*}

%Figure \ref{fig:cmu-graph} shows the results obtained from study 3. The result \textbf{confirms hypotheses 3 and 6}. Specifically, all the transfer learning approaches perform poorly, but the target-based Word2Vec achieves the best performance.

Figure \ref{fig:cmu-graph} shows the results obtained from study 5. We see that the mixed-domain transfer learning approach performs poorly. The best performing model is the DSPTM-based Word2Vec. 


\subsection{Analysis}

Based on the results given in the above tables, we summarize our observations below. First, we discuss a model's generalizability for binary classification scenarios. Given the length of the text and the size of the dataset, we identify 4 cases.

\begin{itemize}
    \item Case 1: Length: Short \& Size: Small
    \item Case 2: Length: Long \& Size: Small
    \item Case 3: Length: Short \& Size: Large
    \item Case 4: Length: Long \& Size: Large
\end{itemize}



\paragraph{Case 1: Length: Short \& Size: Small}

For case 1 we do not find a single best-performing model. For the tweet dataset, following models perform slightly better: VGCN-BERT, GloVe (transfer learning and DSPTM-based), and Text GCN. There are two possible explanations for the poor performance of all models on the short-length tweet data. First, the number of test misinformation samples is significantly smaller. Second, the short length of the text (tweet and tweet+reply) and the small size of the training set might have influenced the context learning of the models. None of the models seem to have captured the context of the text well enough to make accurate predictions. 
    




%Table \ref{summary} shows that for the tweet and tweet+replies datasets following models perform slightly better: VGCN-BERT, GloVe (transfer learning and target based), and Text GCN.




%\begin{table*}[!htb]
%\caption{Effective Models: Binary Classification \\ *Performance measures are shown only for the misinformation class}
%\begin{center}
%\scalebox{0.8}{
%\begin{tabular}{|l|l|l|l|l|l|l|}
%\hline
%\textbf{} & \multicolumn{2}{l|}{\textbf{Test: July}} & \multicolumn{2}{l|}{\textbf{Test: September}} & \multicolumn{2}{l|}{\textbf{Test: November}} \\ \hline
%\textbf{} & \textbf{Precision}   & \textbf{Recall}   & \textbf{Precision}      & \textbf{Recall}     & \textbf{Precision}     & \textbf{Recall}     \\ \hline
%\multicolumn{7}{|c|}{\textbf{Tweets}}                                         \\ \hline
%\textbf{VGCN-BERT}                 & 0.49 & 0.019 & 0.287  & 0.029 &0.21      &0.389      \\ \hline
%\textbf{GloVe (Transfer Learning)} & 0.31 & 0.02  & 0.00&0.00      &1.00      &1.00      \\ \hline
%\textbf{Text GCN}                  & 0.029  & 0.00       & 0.95 & 1.00 & 0.99 & 1.00 \\ \hline
%\multicolumn{7}{|c|}{\textbf{Tweets + Replies}}                               \\ \hline
%\textbf{GloVe (Transfer Learning)} & 0.23 & 0.21  & 0.16 & 0.05 & 0.04 & 0.50 \\ \hline
%\textbf{GloVe}                     & 0.06     &0.04       &0.00      &0.00      & 0.18 & 0.50 \\ \hline
%\multicolumn{7}{|c|}{\textbf{News Articles}}                                  \\ \hline
%\textbf{Word2Vec}                  & 0.92 & 0.85  & 0.11 & 0.74 & 0.92 & 0.58 \\ \hline
%\textbf{ELMo (Transfer Learning)}  &0.11      &0.19       & 0.83 & 0.64 & 0.88 & 0.37 \\ \hline
%\end{tabular}}
%\end{center}
%%\label{summary}
%\end{table*}


%There are two possible explanations for the poor performance of all models on the short-length tweet data. 
%
%\begin{itemize}
%    \item \textbf{Small Size of Misinformation Test Set:} The number of test misinformation samples is significantly smaller. For example, in the 2020 July, September, and November Tweet test datasets the true information samples are larger than the misinformation samples by 46, 17, and 96 times, respectively. Both for the tweet and tweet+reply November subsets we have only 2 samples of misinformation. This might have caused low precision and recall for misinformation class.
%    
%    \item \textbf{Short Text Length \& Small Trained Dataset:} The short length of the text (tweet and tweet+reply) and the small size of the training set might have influenced the context learning of the models. None of the models seem to have captured the context of the text well enough to make accurate predictions. 
%    
%\end{itemize}


\paragraph{Case 2: Length: Long \& Size: Small}

For the news articles data, the best model is DSPTM-based Word2Vec for the July and November dataset. Both models achieved higher precision and recall on the misinformation class. For the September dataset, the ELMo outperforms DSPTM-based Word2Vec.

\paragraph{Case 3: Length: Short \& Size: Large}

For this case, both DSPTM-based Word2Vec and BERT-based transfer learning perform well. However, BERT's performance is not consistent. On the Tweet dataset (short-length text), the precision of BERT is poor. It indicates that even with larger training data BERT-based transfer learning does not provide an effective solution for short-length samples. One possible reason is that although the BERT model is good at capturing the local relationship (e.g., word order), it does not do equally well on capturing the global relationship or context from short-length data.



\paragraph{Case 4: Length: Long \& Size: Large}

Both DSPTM-based Word2Vec and BERT-based transfer learning perform well in this case. However, BERT's performance is slightly better.


The results from fine-grained classification show that DSPTM-based Word2Vec is the clear winner. It outperforms other approaches by a large margin.

\noindent Based on the insights garnered from the above analyses, we draw the following conclusions, summarized in Figure \ref{fig:framework}.
\begin{itemize}
   

    \item The \textbf{mixed-domain transfer learning} approach with the BERT SOTA model is effective in limited cases. Also, its performance is not consistent.
    
    \item The \textbf{graph-based DSPTM} approach does not yield an effective solution in any of the cases. The VGCN-BERT that combines the benefits of Text GCN with BERT is not effective either.
    
    %\item The \textbf{hybrid} approach that combines BERT embeddings with graph embeddings is not effective either.
    
     \item The \textbf{non-graph DSPTM-based} approach with the Word2Vec model generalizes well across the last three cases.
    
\end{itemize}


%Thus, there is no single generalizable approach for identifying COVID-19 social media misinformation. The choice of an effective approach is dependent on the length of the text, size of the dataset, and the distribution of the classes. 
%
%
%We use these insights to propose a generalizable framework.
%
%
%
%Figure \ref{fig:framework} illustrates our framework. The framework includes recommendations for two types of classification: binary and fine-grained. For a binary classification problem, the framework uses the data from two dimensions: length of the text and size of the dataset.
%
%\begin{itemize}
%    \item Length Short + Small Dataset: Graph-based methods such as Text GCN and transfer learning method based on pretrained GloVe embeddings
%    
%    \item Length Long + Small Dataset: Target-based Word2Vec embedding with a CNN classifier
%    
%    \item Length Short and Long + Large Dataset: Target-based Word2Vec embedding with a CNN classifier and transfer learning using BERT
%    
%    
%\end{itemize}
%
%We do not observe a single best-performing model on the short length and small size dataset. Thus, our framework makes a weak recommendation on this type of data.
%
%For the fine-grained data, the best model is the Target-based Word2Vec embedding with CNN classifier.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\linewidth]{figures/Framework.png}
  \caption{Framework for Misinformation Detection}
  \label{fig:framework}
\end{figure}




==> 2021-EMNLP-Camera Ready/4.Results.tex <==
\section{Results and Analysis}






\begin{table*}[!htb]

%\vspace{-4.00mm}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.942} &
  \multicolumn{6}{c|}{Accuracy = 0.990} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{BERT}} &
  \multicolumn{1}{l|}{0.981} &
  0.997 &
  0.989 &
  0.281 &
  {\color[HTML]{000000} 0.079} &
  0.116 &
  \multicolumn{1}{l|}{0.946} &
  0.996 &
  0.970 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{1.00} &
  0.990 &
  0.995 &
  0.500 &
  1.00 &
  0.670 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.941} &
  \multicolumn{6}{c|}{Accuracy = 0.990} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{ELMo}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.945} &
  0.995 &
  0.970 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.990} &
  1.00 &
  0.995 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.932} &
  \multicolumn{6}{c|}{Accuracy = 0.969} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.949} &
  0.980 &
  0.964 &
  0.20 &
  0.09 &
  0.12 &
  \multicolumn{1}{l|}{0.99} &
  0.979 &
  0.984 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.943} &
  \multicolumn{6}{c|}{Accuracy = 1.00} \\ \cline{2-19} 
%\multirow{-2}{*}{\textbf{GloVe}} &

\multirow{-2}{*}{\color[HTML]{FE0000} {\ul \textbf{GloVe}}}&




  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  0.31 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  0.998 &
  0.971 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{1.00} &
  1.00 &
  1.00 &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
   {\color[HTML]{FE0000} {\ul \textbf{1.00}}}  \\ \hline
\multicolumn{19}{|c|}{\textbf{DSMs: Graph-based}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Text GCN}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.029 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.95 &
  1.00 &
  0.97 &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.99 &
  1.00 &
  0.99 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.971} \\ \cline{2-19} 
%\multirow{-2}{*}{\textbf{VGCN-BERT}} &


\multirow{-2}{*}{\color[HTML]{FE0000} {\ul \textbf{VGCN-BERT}}}&


  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  {\color[HTML]{FE0000} {\ul \textbf{0.495}}} &
  0.019 &
  0.035 &
  \multicolumn{1}{l|}{0.947} &
  0.999 &
  0.972 &
  {\color[HTML]{FE0000} {\ul \textbf{0.287}}} &
  0.029 &
  0.052 &
  \multicolumn{1}{l|}{0.994} &
  0.977 &
  0.984 &
  0.21 &
  0.389 &
  0.246 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSMs: Non-Graph + CNN}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.977} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.979} &
  0.997 &
  0.988 &
  0.11 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  1.00 &
  0.972 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.99} &
  1.00 &
  0.995 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.979} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  0.23 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  1.00 &
  0.972 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.99} &
  0.99 &
  0.99 &
  0.00 &
  0.00 &
  0.00 \\ \hline
\end{tabular}}
\vspace{-2.00mm}	
\caption{Study 1 \& 2: CoAID - Tweet (Temporal \& Text Length Dimension). Best results, as well as the optimal models, are highlighted in red. \textbf{None of the models generalize well on the tweet data.}}
\label{CoAID-Tweet}
\end{center}
\vspace{-2.00mm}	
 

\end{table*}










\begin{table*}[!htb]

%\vspace{-4.00mm}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.646} &
  \multicolumn{6}{c|}{Accuracy = 0.503} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{BERT}} &
  \multicolumn{1}{l|}{0.814} &
  1.00 &
  0.898 &
  0.00 &
  {\color[HTML]{000000} 0.00} &
  0.00 &
  \multicolumn{1}{l|}{0.929} &
  0.676 &
  0.779 &
  0.018 &
  0.135 &
  0.036 &
  \multicolumn{1}{l|}{0.962} &
  0.511 &
  0.656 &
  0.009 &
  0.144 &
  0.009 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.559} &
  \multicolumn{6}{c|}{Accuracy = 0.973} &
  \multicolumn{6}{c|}{Accuracy = 0.985} \\ \cline{2-19} 
%\multirow{-2}{*}{\textbf{ELMo}} &

\multirow{-2}{*}{\color[HTML]{FE0000} {\ul \textbf{ELMo}}}&


  \multicolumn{1}{l|}{0.777} &
  0.642 &
  0.703 &
  0.11 &
  0.19 &
  0.14 &
  \multicolumn{1}{l|}{0.979} &
  0.993 &
  0.986 &
  {\color[HTML]{FE0000} {\ul \textbf{0.83}}} &
  0.64 &
  {\color[HTML]{FE0000} {\ul \textbf{0.72}}} &
  \multicolumn{1}{l|}{0.986} &
  0.99 &
  0.992 &
  0.88 &
  0.37 &
  0.52 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.851} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.98} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.846} &
  0.999 &
  0.916 &
  0.98 &
  0.20 &
  0.33 &
  \multicolumn{1}{l|}{0.948} &
  0.998 &
  0.972 &
  0.60 &
  0.06 &
  0.12 &
  \multicolumn{1}{l|}{0.98} &
  1.00 &
  0.99 &
  1.00 &
  0.11 &
  0.19 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.599} &
  \multicolumn{6}{c|}{Accuracy = 0.953} &
  \multicolumn{6}{c|}{Accuracy = 0.984} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.833} &
  0.635 &
  0.721 &
  0.22 &
  0.44 &
  0.29 &
  \multicolumn{1}{l|}{0.957} &
  0.995 &
  0.975 &
  0.73 &
  0.23 &
  0.35 &
  \multicolumn{1}{l|}{0.985} &
  0.999 &
  0.992 &
  {\color[HTML]{000000} 0.86} &
  {\color[HTML]{000000} 0.32} &
  0.46 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSMs: Graph-based}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.635} &
  \multicolumn{6}{c|}{Accuracy = 0.978} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Text GCN}} &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.81 &
  1.00 &
  0.90 &
  \multicolumn{1}{l|}{0.97} &
  0.633 &
  0.766 &
  0.095 &
  0.66 &
  0.165 &
  \multicolumn{1}{l|}{0.978} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.677} &
  \multicolumn{6}{c|}{Accuracy = 0.64} &
  \multicolumn{6}{c|}{Accuracy = 0.458} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{VGCN-BERT}} &
  \multicolumn{1}{l|}{0.971} &
  0.622 &
  0.758 &
  {\color[HTML]{000000} 0.356} &
  0.917 &
  0.513 &
  \multicolumn{1}{l|}{0.985} &
  0.628 &
  0.767 &
  {\color[HTML]{000000} 0.117} &
  0.839 &
  0.205 &
  \multicolumn{1}{l|}{0.989} &
  0.451 &
  0.619 &
  0.031 &
  0.778 &
  0.06 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSMs: Non-Graph + CNN}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.96} &
  \multicolumn{6}{c|}{Accuracy = 0.643} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
%\multirow{-2}{*}{\textbf{Word2Vec}} &

\multirow{-2}{*}{\color[HTML]{FE0000} {\ul \textbf{Word2Vec}}}&

  \multicolumn{1}{l|}{0.957} &
  0.984 &
  0.975 &
  {\color[HTML]{FE0000} {\ul \textbf{0.92}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.85}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.89}}} &
  \multicolumn{1}{l|}{0.977} &
  0.638 &
  0.772 &
  0.11 &
  {\color[HTML]{FE0000} {\ul \textbf{0.74}}} &
  0.19 &
  \multicolumn{1}{l|}{0.991} &
  0.99 &
  0.995 &
  {\color[HTML]{FE0000} {\ul \textbf{0.92}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.58}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.71}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.554} &
  \multicolumn{6}{c|}{Accuracy = 0.623} &
  \multicolumn{6}{c|}{Accuracy = 0.452} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.775} &
  0.637 &
  0.699 &
  0.10 &
  0.19 &
  0.13 &
  \multicolumn{1}{l|}{0.941} &
  0.641 &
  0.763 &
  0.05 &
  0.32 &
  0.09 &
  \multicolumn{1}{l|}{0.962} &
  0.457 &
  0.62 &
  0.01 &
  0.21 &
  0.02 \\ \hline
\end{tabular}}
\vspace{-2.00mm}	
\caption{Study 1 \& 2: CoAID - News Articles (Temporal \& Text Length Dimension). Best results, as well as the optimal models, are highlighted in red.}
\label{CoAID-news}
\end{center}
\vspace{-2.00mm}	

\end{table*}







%We present the results obtained from five studies. 

We evaluate the performance of the models based on the accuracy, precision, recall, and f1 score, with an emphasis on the misinformation class. For each experiment, we average the results for 10 runs. The experiments are done using Scikit-learn \cite{scikit-learn}, TensorFlow 2.0 \cite{tensorflow2015-whitepaper}, and PyTorch \cite{PyTorch} libraries. For creating the Word2Vec embeddings, we used the skip-gram model from the Gensim library \cite{gensim}. Finally, the GloVe embeddings are created using the model from \cite{glove}.


\paragraph{Results.} Table \ref{CoAID-Tweet} and Table \ref{CoAID-news} show the results from studies 1 and 2. 

\vspace{1.00mm}
From the results on the CoAID tweets, given in Table \ref{CoAID-Tweet}, we see that for the July tweet test dataset (Table \ref{CoAID-Tweet}), VGCN-BERT has the highest misinformation precision. However, misinformation recall and f1 scores for all models are poor. For September, the Text-GCN has outstanding performance for detecting misinformation, but its performance on true information is extremely poor. Other models perform badly on misinformation. For November, the GloVe-based transfer learning approach achieves excellent performance on both true information and misinformation, where precision, recall, and f1 scores are 1. Text-GCN also has decent scores on misinformation but fails to detect true information. The performance of BERT on both true information and misinformation is also good. However, we notice that no model performs well across three different test datasets. Thus, we see that \textbf{mixed-domain transfer learning is not robust when the context of the short-length data (tweets) changes}. This is also true for the DSM-based approach. 







\begin{table*}[htb!]

%\vspace{-4.00mm}
\begin{center}
\scalebox{0.66}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train: May + July + September\\ Test: November\end{tabular}}} &
  \multicolumn{6}{c|}{\textbf{Tweets}} &
  \multicolumn{6}{c|}{\textbf{News Articles}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.928} &
  \multicolumn{6}{c|}{Accuracy = 0.992} \\ \cline{2-13} 
\multirow{-2}{*}{\textbf{Mixed-Domain Transfer Learning: BERT}} &
  \multicolumn{1}{l|}{1.00} &
  0.927 &
  0.962 &
  0.12 &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
  0.22 &
  \multicolumn{1}{l|}{0.994} &
  0.998 &
  0.996 &
  {\color[HTML]{FE0000} {\ul \textbf{0.883}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.719}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.787}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.985} &
  \multicolumn{6}{c|}{Accuracy = 0.986} \\ \cline{2-13} 
\multirow{-2}{*}{\textbf{DSM (Non-Graph): Word2Vec + CNN}} &
  \multicolumn{1}{l|}{0.99} &
  0.995 &
  0.992 &
  {\color[HTML]{FE0000} {\ul \textbf{0.71}}} &
  {\color[HTML]{000000} 0.63} &
  {\color[HTML]{FE0000} {\ul \textbf{0.67}}} &
  \multicolumn{1}{l|}{0.992} &
  0.994 &
  0.993 &
  {\color[HTML]{000000} 0.71} &
  0.63 &
  {\color[HTML]{000000} 0.67} \\ \hline
\end{tabular}}
\vspace{-2.00mm}	
\caption{Study 3: CoAID Large Dataset (Dataset Size Dimension). Best results are highlighted in red.}
\label{CoAID-Big}
\end{center}
\vspace{-4.00mm}	

\end{table*}





Table \ref{CoAID-news} shows the results of CoAID news articles (lengthy text). For the July test dataset, both Text-GCN and  Word2Vec (DSM-based) achieve decent precision, recall, and f1 scores on misinformation. However, Text-GCN has extremely poor performance on true information. On the September data, ELMo exhibits the best misinformation precision, and f1 score, while Word2Vec (DSM-based) gives the best misinformation recall score. Both ELMo and Word2Vec perform well on the true information class as well. As for the November data, both transfer learning and DSM-based Word2Vec obtain optimal misinformation precision score and Word2Vec (DSM-based) obtains the highest f1 score. Besides, VGCN-BERT achieves the highest misinformation recall score. We notice that the DSM-based Word2Vec exhibits comparatively better performance across all test datasets. Thus, the \textbf{non-graph DSM+CNN can capture both global and local relationships from lengthy text relatively well}. The performance of the graph-based DSM approach on lengthy text is not as good as on short text. Also, BERT shows unreliable performance as it fails on the misinformation class.





Table \ref{CoAID-Big} shows the results of study 3, i.e., large-dataset-based experiments. The performance of DSM-based Word2Vec is consistent with its performance on the CoAID news articles data (Table \ref{CoAID-news}).  Its F1 score on tweets misinformation increases significantly compared to the small-data case (Table \ref{CoAID-Tweet}). \textbf{Thus, the non-graph DSM+CNN can capture both global and local relationships if we increase the size of short-length training data (i.e., tweets)}. 




\begin{table*}[htb!]

%\vspace{-4.00mm}
\begin{center}
\scalebox{0.62}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.611} &
  \multicolumn{6}{c|}{Accuracy = 0.943} &
  \multicolumn{6}{c|}{Accuracy = 0.993} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{ALBERT}} &
  \multicolumn{1}{l|}{0.858} &
  0.625 &
  0.723 &
  0.25 &
  {\color[HTML]{000000} 0.547} &
  0.343 &
  \multicolumn{1}{l|}{0.96} &
  0.981 &
  0.97 &
  0.483 &
  0.298 &
  0.368 &
  \multicolumn{1}{l|}{0.996} &
  0.996 &
  0.996 &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.936} &
  \multicolumn{6}{c|}{Accuracy = 0.630} &
  \multicolumn{6}{c|}{Accuracy = 0.980} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{RoBERTa}} &
  \multicolumn{1}{l|}{0.937} &
  0.987 &
  0.962 &
  {\color[HTML]{FE0000} {\ul \textbf{0.925}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.711}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.804}}} &
  \multicolumn{1}{l|}{0.952} &
  0.641 &
  0.766 &
  {\color[HTML]{000000} 0.068} &
  0.447 &
  {\color[HTML]{000000} 0.118} &
  \multicolumn{1}{l|}{0.991} &
  0.989 &
  0.990 &
  0.55 &
  0.579 &
  0.564 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.97} &
  \multicolumn{6}{c|}{Accuracy = 0.456} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{XLNET}} &
  \multicolumn{1}{l|}{0.81} &
  1.00 &
  0.90 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.97} &
  1.00 &
  0.98 &
  {\color[HTML]{FE0000} {\ul \textbf{0.89}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.53}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.67}}} &
  \multicolumn{1}{l|}{0.97} &
  0.46 &
  0.62 &
  0.01 &
  0.26 &
  0.02 \\ \hline
\end{tabular}}
\vspace{-2.00mm}	
\caption{Study 4: CoAID Large Dataset (Various-based Transformer Models). Best results are highlighted in red. \textbf{No single model performs well across three datasets}.}
\label{CoAID-bert-variants}
\vspace{-2.00mm}	
\end{center}


\end{table*}



\begin{figure*}[!ht]
  \centering
  %\includegraphics[width=\linewidth]{figures/cmu-result-graph.png}
  \includegraphics[width=4.3in]{figures/cmu-result-graph.png}
  \vspace{-2.00mm}	
  \caption{Study 5: CMU-MisCov19 (Fine-grained classification).}
   \vspace{-5.00mm}	
  \label{fig:cmu-graph}
\end{figure*}






Table \ref{CoAID-bert-variants} shows the results obtained from study 4. For the July test dataset misinformation detection, RoBERTa achieves the best performance, while XLNet shows the worst performance. However, for September misinformation, we observe the exact opposite scenario. As for November misinformation, ALBERT achieves the best performance, while XLNet's performance is the worst. \textbf{No single Transformer-based model performs well on the three datasets.} These results corroborate our previous observation on the mixed-domain transfer learning approach, i.e., it is not robust when the context of the data changes. 

%XLNet obtains the best performance, while the RoBERTa has the worst performance.

Figure \ref{fig:cmu-graph} shows the results obtained from study 5. We see that the mixed-domain transfer learning approach performs poorly on the fine-grained dataset. The only model that achieves decent performance is the non-graph DSM Word2Vec with CNN. 



\begin{figure*}[!htb]
  \centering
  %\includegraphics[width=\linewidth]{figures/Framework.png}
  \includegraphics[width=3.2in]{figures/Framework.png}
  \vspace{-2.00 mm}
  \caption{A framework for COVID-19 online misinformation detection.}
  \label{fig:framework}
 \vspace{-4.00 mm}
\end{figure*}


\paragraph{Analysis.}

Based on the results obtained from the studies, we summarize our observations below. First, we discuss a model's generalizability for binary classification scenarios. Given the length of the text and the size of the dataset, we identify 4 cases.

%\begin{itemize}
%    \item Case 1: Length: Short \& Size: Small
%    \item Case 2: Length: Long \& Size: Small
%    \item Case 3: Length: Short \& Size: Large
%    \item Case 4: Length: Long \& Size: Large
%\end{itemize}



\vspace{1.00mm}
\textbf{Case 1: Length=Short \& Size=Small} For case 1, we do not find a single best-performing model. For the tweet dataset, the following models perform slightly better: VGCN-BERT, GloVe (transfer learning and DSM-based), and Text GCN. There are two possible explanations for the poor performance of all models on the short-length tweet data. First, the number of test misinformation samples is significantly smaller. For example, in the 2020 July, September, and November tweet test datasets, the true information samples are larger than the misinformation samples by 46, 17, and 96 times, respectively. Second, the short length of the text and the small size of the training set might have influenced the scope of the context learning by the models. 

%None of the models seem to have captured the context of the text well enough to make accurate predictions. 
    

% \item \textbf{Small Size of Misinformation Test Set:} The number of test misinformation samples is significantly smaller. For example, in the 2020 July, September, and November Tweet test datasets the true information samples are larger than the misinformation samples by 46, 17, and 96 times, respectively. Both for the tweet and tweet+reply November subsets we have only 2 samples of misinformation. This might have caused low precision and recall for misinformation class.


\vspace{1.00mm}
\textbf{Case 2: Length=Long \& Size=Small} For the news articles data, the best model is DSM Word2Vec+CNN for the July and November datasets. It achieved the highest precision and recall on the misinformation class. For the September dataset, the ELMo outperforms DSM Word2Vec+CNN.

\vspace{1.00mm}
\textbf{Case 3: Length=Short \& Size=Large} Both DSM Word2Vec+CNN and BERT-based transfer learning performed well. However, BERT's performance is not consistent. On the tweet dataset (short-length text), the precision of BERT is poor. It indicates that even with larger training data, BERT-based transfer learning does not provide an effective solution for short-length samples. One possible reason is that \textbf{although BERT is good at capturing the local relationships (e.g., word order), it does not do equally well on capturing the global relationships from short-length data}.



\vspace{1.00mm}
\textbf{Case 4: Length=Long \& Size=Large} Both DSM Word2Vec+CNN and BERT-based transfer learning perform well in this case. BERT's performance is slightly better. This indicates that Transformer-based models are suitable when target data is large and texts are lengthy.

\vspace{1.00mm}
The results from fine-grained classification show that DSM Word2Vec+CNN  outperforms other approaches by a large margin. Apart from the case of binary short length and small size dataset, DSM Word2Vec+CNN is shown to achieve the most effective solution. 


One possible reason for the better generalization capability of the non-graph DSM+CNN-based approach is that its hierarchical feature-extraction mechanism is conducive for learning both the \textbf{local context} (the non-graph DSM, e.g., Word2Vec captures the local relationships of words in the target text) and the \textbf{global context} (the CNN learns global relationships from the word embeddings), which \textbf{validates our hypothesis}.




%One possible reason for the better generalization capability of the non-graph DSM+CNN-based approach is: the non-graph DSM (e.g., Word2Vec) embeddings capture mostly \textbf{local relationships} among the words of the target text. From these embeddings, the CNN learns \textbf{global relationships} via the extracted higher-level features. Thus, the hierarchical feature-extraction mechanism of the non-graph DSM+CNN may have contributed towards its optimal performance. 
%






\vspace{2.00mm}
Based on the insights garnered from the above analysis, we draw the following conclusions, summarized in the framework in Figure \ref{fig:framework}.



\begin{itemize}
   

    \item The Transformer-based \textbf{mixed-domain transfer learning} approach is effective in limited cases. Also, its performance is not consistent.
    %\vspace{-2.00mm}
    
    \item The \textbf{graph-based DSM} approach does not yield an effective solution in any of the cases. The VGCN-BERT that combines the benefits of Text GCN with BERT is not effective either.
    %\vspace{-6.00mm}
    
    %\item The \textbf{hybrid} approach that combines BERT embeddings with graph embeddings is not effective either.
    
     \item The \textbf{non-graph DSM + CNN} approach generalizes well across the last three cases.
     %\vspace{-2.00mm}
    
\end{itemize}
%\vspace{-2.00mm}





%\subsection{Limitations}

Our study suffers from \textbf{some limitations}. The lack of labeled data narrowed the scope of our investigation. The data scarcity affected our study in two ways. First, due to the small size of the test data, we obtained noisy estimates for the short length and small size data. Second, we could not conduct a multi-dimensional study on the fine-grained classification problem.

%\begin{itemize}
%    \item \textbf{Misinformation Samples:} In our binary classification CoAID dataset the number of misinformation samples is significantly smaller. For example, in the test subsets, misinformation samples are $46 \sim 96$ times smaller. In the November tweet and tweet+reply datasets, we have only 2 samples of misinformation. In the November news articles subset, this number is 19. The lack of misinformation data limits the evaluation of the models. We obtained noisy estimates for the short length and small size data. Thus, we were unable to make a confident recommendation for this type of data.
%    
%    \item \textbf{Fine-grained Dataset:} We could not conduct a multi-dimensional study on the fine-grained classification problem due to a lack of labeled data. Our plan was to investigate the multi-class scenario by varying both the size of the dataset and the length of the text (for both tweets and news articles). The scarcity of labeled fine-grained data forced us to conduct only a one-dimensional analysis. Thus, we could not evaluate the generalizability of the models along the temporal dimension.
%    
%    
%\end{itemize}





==> 2021-EMNLP-Camera Ready/5.Conclusion.tex <==
\section{Conclusion}

\vspace{-1.50mm}
When an unanticipated pandemic like COVID-19 breaks out, various types of misinformation emerge and propagate at warp speed over online social media. For detecting such misinformation, NLP techniques require to capture the context of the discourse from its evolving narrative. We argue that irrespective of the success of the deep learning based mixed-domain transfer learning approach for solving various NLP tasks, it does not yield a generalizable solution. We emphasize the importance of learning the context (both local and global) directly from the target domain via the DSM-based approach. A feasible way to implement a DSM is to utilize shallow neural networks that capture the local relationships in the target data. Representations learned from this type of model can then be used by shallow CNNs to learn global relationships as high-level features. Thus, a combination of non-graph DSM and CNN may lend a more generalizable solution. We perform an extensive study using Twitter-based COVID-19 social media data that includes tweets and news articles referred to in the tweets. Our investigation is performed along the following dimensions of the data: temporal dimension (evolving context), length dimension (varying text length), size dimension (varying size of datasets), and classification-level dimension (binary vs. multi-class data). We show that the mixed-domain transfer learning approach does not always work well. We found the combination of the non-graph DSM (for capturing local relationships) and CNN (for extracting global relationships) to be a promising approach towards creating a generalizable solution for detecting COVID-19 online misinformation.

% We found the combination of the Word2Vecnon-graph DSM (for creating embeddings) and CNN (for extracting high-level features)  to be most effective across the majority of the dimensions of our study.

In the future, we plan to investigate the generalizability of the DSM models created using deep learning architectures such as BERT. 

%Also, we plan to extend our investigation by including multi-modal social media COVID-19 data (e.g., image, video). 




%Due to the small size of the labeled target data, shallow neural models such as Word2Vec is suitable to build DSMs. 




==> 2021-EMNLP-Camera Ready/dataset_analysis.tex <==
\section{Dataset}

We describe the sample distribution of both the CoAID (binary) and CMU datasets. Then, we analyze context evolution in the CoAID new articles dataset. 



\begin{figure}[!htb]
  \centering
\includegraphics[width=\linewidth]{figures/news.png}
 % \includegraphics[width=3.7in]{figures/tweets.png}
  \caption{CoAID Tweets: Sample distribution (0: misinformation, 1: true information).}
  \label{fig:coaid-tweet}
\end{figure}

%\begin{figure}[!htb]
%  \centering
%  \includegraphics[width=\linewidth]{figures/reply.png}
%  \caption{CoAID: Distribution of Replies.}
%  \label{fig:coaid-reply}
%\end{figure}

\label{coaid}
\begin{figure}[!htb]
  \centering
  \includegraphics[width=\linewidth]{figures/news.png}
 % \includegraphics[width=3.0in]{figures/news.png}
  \caption{CoAID News Articles: Sample distribution (0: misinformation, 1: true information).}
  \label{fig:coaid-news}
\end{figure}


\begin{figure}[htb!]
  \centering
 % \includegraphics[width=\linewidth]{figures/cmu.png}
  %\includegraphics[width=3.6in]{figures/CMU-class-distribution-names.png} 
  \includegraphics[width=\linewidth]{figures/CMU-class-distribution-names.png} 
  %\vspace{-4.00 mm}
  \caption{CMU-MisCov19 Dataset: Sample distribution.}
 % \vspace{-5.00 mm}
  \label{fig:cmu}
\end{figure}


\begin{figure*}[htb!]
    \begin{center}
        \subfigure[May]{\label{news-may}\includegraphics[width=2.20in]{figures/coaid-may-news-frequency.png}} \quad	
        \subfigure[July]{\label{news-july}\includegraphics[width=2.20in]{figures/coaid-july-news-frequency.png}} \\	
        \subfigure[September]{\label{news-sept}\includegraphics[width=2.20in]{figures/coaid-sept-news-frequency.png}} \quad
        \subfigure[November]{\label{news-nov}\includegraphics[width=2.20in]{figures/coaid-nove-news-frequency.png}} \quad
        \caption{CoAID News Articles: Frequency of top 10 words.}
        \label{news-top10}
       % \vspace{-6.00mm}
    \end{center}
\end{figure*}


\begin{figure*}[htb!]
    \begin{center}
        \subfigure[May]{\label{news-wordcloud-may}\includegraphics[width=2.20in]{figures/CoAID-May-News-WordCloud.png}} \quad	
        \subfigure[July]{\label{news-wordcloud-july}\includegraphics[width=2.20in]{figures/CoAID-July-News-WordCloud.png}} \\	
        \subfigure[September]{\label{news-wordcloud-sept}\includegraphics[width=2.20in]{figures/CoAID-Sept-News-WordCloud.png}} \quad
        \subfigure[November]{\label{news-wordcloud-nov}\includegraphics[width=2.20in]{figures/CoAID-Nove-News-WordCloud.png}} \quad
        \caption{CoAID News Articles: Word Clouds for the four datasets.}
        \label{news-wordcloud}
        %\vspace{-6.00mm}
    \end{center}
\end{figure*}


\paragraph{CoAID Sample Distribution.}

Figures \ref{fig:coaid-tweet} and \ref{fig:coaid-news} show the distributions of tweets and news articles per category, respectively. We see that the datasets contain significantly more true information than misinformation. Thus, the CoAID data is \textbf{heavily skewed}. For the tweets dataset, the sizes of May and July data are larger than that of September and November. Also, the number of misinformation tweets during September and November are negligibly smaller, making it challenging to use these as test datasets.




\paragraph{CMU Sample Distribution.}

The CMU-MisCov19 or CMU short-length text dataset misinformation categories are fine-grained comprising of 17 classes. It consists of 4,573 annotated tweets from 3,629 users with an average of 1.24 tweets per user. Figure \ref{fig:cmu} shows the \textbf{heavily skewed} distribution of 4,292 tweets for all categories that were extracted after some pre-processing. Class 7 (calling out or correction) has the most tweets, while class 2 (true treatment) has 0 tweets. 

%The test data is created by randomly sampling 20\% of the data.




\begin{table*}[!htb]
\begin{center}
\scalebox{1.0}{
\begin{tabular}{|p{2.0cm}|p{2.0cm}|p{1.4cm}|p{2.4cm}|p{2.2cm}|p{1.7cm}|p{1.6cm}|}  
\hline
     					& Embedding Dimension 		& \# Hidden Layers 			& Batch Size 		& Optimizer 		& Learning Rate \\ \hline
BERT         			&  768                   			&   12              			   	& 32           		& AdamW          	& 2e-5              \\ \hline
ELMo         			& 1024                    			&   5               			    	& 128           		& Adam          		& 0.001             \\ \hline
RoBERTa      			& 768                    			&   12             				&  16          		& AdamW           	& 2e-6             \\ \hline
ALBERT       			& 128                    			&   12             			  	& 6           			& Adam        		& 3e-5              \\ \hline
XLNet        			& 768                    			&  12                			  	&  32          		& AdamW          	& 2e-5               \\ \hline
Text GCN     			& 200                   			&   2              			 	& N/A          		& Adam           		& 0.02            \\ \hline
VGCN BERT    		        & N/A                    			&   18              			        & 16           		& Adam           		& 2e-5            \\ \hline
Word2Vec     			& 300                   			&   2              			        & 128           		& Adam          		& 0.001              \\ \hline
GloVe        			& 300                    			&   N/A              			        & N/A           		& AdaGrad       		& N/A               \\ \hline
\end{tabular}}
\caption{Experimental setting.}
\label{experimental_setting}
 \end{center}
\end{table*}



\subsubsection{CoAID News Articles: Study of Context Evolution}






Figure \ref{news-top10} shows context evolution in the news articles category via the evolution of the distribution of the top ten high-frequency terms. We see, similar to the tweet dataset, context changes over time in the news articles datasets. For example, The May and July datasets have only 4 common high-frequency words: covid, coronavirus, health, data. In the July dataset, we observe the emergence of three new high-frequency words attack, security, and protect, which indicates a change in context. The context in the September dataset seems to be similar to that of the July dataset. These two datasets have eight high-frequency words in common: covid, service, online, attack, security, health, information, coronavirus. The November dataset shares seven common words with the September dataset: covid, service, online, attack, people, health, coronavirus. However, we notice an increase in the frequency in some words such as protect and attack. Also, a new word pandemic is seen to emerge. We gather similar observations about the context evolution from the word clouds in Figure \ref{news-wordcloud}.






==> 2021-EMNLP-Camera Ready/training_statistics.tex <==

%
%\begin{table*}[bp]
%\begin{center}
%\scalebox{0.8}{
%\begin{tabular}{|p{2.0cm}|p{2.0cm}|p{1.4cm}|p{2.4cm}|p{2.2cm}|p{1.7cm}|p{1.6cm}|}  
%\hline
%     					& Embedding Dimension 		& \# Hidden Layers 			& Batch Size 		& Optimizer 		& Learning Rate \\ \hline
%BERT         			&  768                   			&   12              			   	& 32           		& AdamW          	& 2e-5              \\ \hline
%ELMo         			& 1024                    			&   5               			    	& 128           		& Adam          		& 0.001             \\ \hline
%RoBERTa      			& 768                    			&   12             				&  16          		& AdamW           	& 2e-6             \\ \hline
%ALBERT       			& 128                    			&   12             			  	& 6           			& Adam        		& 3e-5              \\ \hline
%XLNet        			& 768                    			&  12                			  	&  32          		& AdamW          	& 2e-5               \\ \hline
%Text GCN     			& 200                   			&   2              			 	& N/A          		& Adam           		& 0.02            \\ \hline
%VGCN BERT    		        & N/A                    			&   18              			        & 16           		& Adam           		& 2e-5            \\ \hline
%Word2Vec     			& 300                   			&   2              			        & 128           		& Adam          		& 0.001              \\ \hline
%GloVe        			& 300                    			&   N/A              			        & N/A           		& AdaGrad       		& N/A               \\ \hline
%\end{tabular}}
%\caption{Experimental setting.}
%\label{experimental_setting}
% \end{center}
%\end{table*}

\section{Experimental Setting \& Training Statistics}

We provide the experimental setting for conducting our studies as well as the training statistics.

\paragraph{Experimental Setting.} Table \ref{experimental_setting} shows the experimental setting for the studies. We used the default learning rate and batch size for all experiments.




%\begin{table}[!htb]
%\caption{Convergence Epochs: Datasets}
%\begin{center}
%\begin{tabular}{|l|l|}
%\hline
%                      			& Epochs 		\\ \hline
%CoAID (Tweet)         		& 5     		 \\ \hline
%%CoAID (Tweet + Reply) 	& 4     		 \\ \hline
%CoAID (News Articles) 	& 10     		\\ \hline
%CMU-MisCov19          	& 10     		\\ \hline
%\end{tabular}
%\label{epochs}
%\end{center}
%\end{table}






\begin{table*}[!htb]
\begin{center}
\scalebox{0.9}{
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Model}              & \textbf{\#Parameters} & \textbf{Dataset}                 & \textbf{Avg. Training Time} \\ \hline
\textbf{BERT PTM}           & 110M                  & CoAID News Articles (large data) & 1.25 mins                   \\ \hline
\textbf{BERT PTM}           & 110M                  & CoAID Tweets (large data)        & 1.66 hours                  \\ \hline
\textbf{BERT PTM}           & 110M                  & CoAID News Articles (small data) & 30 sec                         \\ \hline
\textbf{BERT PTM}           & 110M                  & CoAID Tweets (small data)        & 1.06 hours                  \\ \hline
\textbf{Word2Vec DSM + CNN} & \begin{tabular}[c]{@{}l@{}}Word2Vec: 6.7M\\ CNN: 160,301\end{tabular}   & CoAID News Articles (large data) & 3.48 mins  \\ \hline
\textbf{Word2Vec DSM + CNN} & \begin{tabular}[c]{@{}l@{}}Word2Vec: 155.9M\\ CNN: 160,301\end{tabular} & CoAID Tweets (large data)        & 1.17 hours \\ \hline
\textbf{Word2Vec DSM + CNN} & \begin{tabular}[c]{@{}l@{}}Word2Vec: 5.1M\\ CNN: 160,301\end{tabular}   & CoAID News Articles (small data) & 1.3 mins   \\ \hline
\textbf{Word2Vec DSM + CNN} & \begin{tabular}[c]{@{}l@{}}Word2Vec: 7.8M\\ CNN: 160,301\end{tabular}   & CoAID Tweets (small data)        & 46 mins    \\ \hline
\textbf{Word2Vec PTM + CNN} & 160,301               & CoAID News Articles (small data) & 2.05 mins                   \\ \hline
\textbf{Word2Vec PTM + CNN} & 160,301               & CoAID Tweets (small data)        & 2.2 hours                   \\ \hline
\textbf{GloVe DSM + CNN}    & \begin{tabular}[c]{@{}l@{}}GloVe: 4.6M\\ CNN: 160,301\end{tabular}      & CoAID News Articles (small data) & 1.33 mins  \\ \hline
\textbf{GloVe DSM + CNN}    & \begin{tabular}[c]{@{}l@{}}GloVe: 100.6M\\ CNN: 160,301\end{tabular}    & CoAID Tweets (small data)        & 45.25 mins \\ \hline
\textbf{GloVe PTM + CNN}    & 160,301               & CoAID News Articles (small data) & 2.08 mins                   \\ \hline
\textbf{GloVe PTM + CNN}    & 160,301               & CoAID Tweets (small data)        & 2.43 hours                  \\ \hline
\textbf{ELMo PTM + CNN}     & 160,301               & CoAID News Articles (small data) & 8.23 mins                   \\ \hline
\textbf{ELMo PTM + CNN}     & 160,301               & CoAID Tweets (small data)        & 8.63 hours                  \\ \hline
\textbf{Text GCN}           & N/A                   & CoAID Tweets (small data)        & 8.8 mins                    \\ \hline
\textbf{VGCN BERT}          & N/A                   & CoAID Tweets (small data)        & 33 hours                    \\ \hline
\textbf{Text GCN}           & N/A                   & CoAID News Articles (small data) & 7.32                        \\ \hline
\textbf{VGCN BERT}          & N/A                   & CoAID News Articles (small data) & 15.26 mins                  \\ \hline
\textbf{RoBERTa}            & 125M                  & CoAID News Articles (small data) & 5.39 mins                   \\ \hline
\textbf{ALBERT}             & 11M                   & CoAID News Articles (small data) & 6.8 hours                   \\ \hline
\textbf{XLNet}              & 110M                  & CoAID News Articles (small data) & 35 sec                      \\ \hline
\textbf{BERT PTM}           & 110M                  & CMU                              & 6 mins                      \\ \hline
\textbf{Word2Vec DSM + CNN} & \begin{tabular}[c]{@{}l@{}}Word2Vec: 8.7M\\ CNN: 160,301\end{tabular}   & CMU                              & 3 mins     \\ \hline
\textbf{Word2Vec PTM + CNN} & 160,301               & CMU                              & 30 sec                      \\ \hline
\textbf{GloVe DSM + CNN}    & \begin{tabular}[c]{@{}l@{}}GloVe: 8.6M\\ CNN: 160,301\end{tabular}      & CMU                              & 3.77 mins  \\ \hline
\textbf{GloVe PTM + CNN}    & 160,301               & CMU                              & 9.17 mins                   \\ \hline
\textbf{ELMo PTM + CNN}     & 160,301               & CMU                              & 1.05 mins                   \\ \hline
\end{tabular}}
\caption{Training Statistics - DSM: Domain-Specific Model, PTM: Pre-Trained Model}
\label{training_statistics}
\end{center}
\end{table*}


\paragraph{Training Statistics.}

Table \ref{training_statistics} shows the training statistics that include the number of parameters for each model, dataset, and the average training time. The inference time is not significant, thus not reported. All experiments were done on a Tesla V100 GPU, except the Text GCN and VGCN BERT based experiments, which were conducted using a CPU. For DSM and CNN based experiments, the CNN was trained for 5 epochs on the CoAID tweet data, 10 epochs on the CoAID news articles data, and 10 epochs on the CMU fine-grained data. The number of epochs was chosen based on the convergence behavior of the models.  


%Each model is trained in parallel on these two GPUs. The training time per-epoch for the large-scale dataset, i.e., Serengeti is 120 minutes on average (there is variance depending on the number of parameters in the model). The CIFAR experiments were conducted on Google Colab. Only 1 GPU is used for Colab experiments since the datasets were smaller in size and did not require big compute or storage.




==> 4.Results-Old.tex <==
\section{Results \& Analysis}

%Domain-Specific Pre-Trained Models (DSPTMs)

%We conduct extensive experiments to implement the studies described in the previous chapter. 
%
%The experiments for this research involve two steps: get the text embeddings (either from a pretrained model using a source dataset or create embeddings using the target dataset) and fine-tune or train a classifier. For the classifier model, we use CNN with 1D convolutional kernels. More specifically, in the transfer learning approach, we use the pretrained embeddings to fine-tune the model with the target data. We also use the pretrained embeddings to train a classifier. For the graph-based method, we create the graph embeddings using the target dataset, then train a classifier. Finally, for the target-based method, we create embeddings using the target dataset, then train a classifier. The experiments use diverse ML models.
%
%\begin{itemize}
%    \item Mixed-Domain Transfer Learning: we obtain the following PTMs - BERT, RoBERTa, ALBERT, XLNet, ELMo, Word2Vec, GloVe. Then, fine-tune the PTM (BERT, RoBERTa, ALBERT, XLNet) or fine-tune a CNN model using the embeddings from the PTM (ELMo, Word2Vec, GloVe)
%    
%    \item DSPTMs - Graph-based: Text GCN and VGCN BERT
%    
%    \item DSPTMs - Non-Graph: (a) for creating text embeddings, we use Word2Vec and GloVe; (b) then, using these embeddings train a single hidden layer CNN
%\end{itemize}
%
%We evaluate the performance of the models based on the accuracy, precision, recall, and f1 score. For each experiment, we average the results for 10 runs. The experiments are done using python's Scikit-learn \cite{scikit-learn} and TensorFlow 2.0 \cite{tensorflow2015-whitepaper} libraries. For training the Word2Vec model, we used the Gensim \cite{gensim} library. 

%\subsection{Experimental Setting}
%
%Table \ref{experimental_setting} and \ref{epochs} show the experimental setting for the studies. 
%
%\begin{table}[!htb]
%\caption{Experimental Setting}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|p{2.0cm}|p{2.0cm}|p{2.0cm}|p{2.4cm}|p{1.2cm}|p{1.7cm}|p{1.6cm}|}  
%\hline
%     					& Embedding Dimension 		& \# Hidden Layers 		& \# Neurons (hidden, final) 	& Batch Size 		& Optimizer 		& Learning Rate \\ \hline
%BERT         			&  768                   			&   12              			&      (768,2)                         	& 32           		& AdamW          	& 2e-5              \\ \hline
%ELMo         			& 1024                    			&   5               			&      (1024,2)                        	& 128           		& Adam          		& 0.001             \\ \hline
%RoBERTa      			& 768                    			&   12             			&      (768,2)                  		&  16          		& AdamW           	& 2e-6             \\ \hline
%ALBERT       			& 128                    			&   12             			&      (128,2)                        	& 6           			& Adam        		& 3e-5              \\ \hline
%XLNet        			& 768                    			&  12                			&      (768,2)                        	&  32          		& AdamW          	& 2e-5               \\ \hline
%Text GCN     			& 200                   			&   2              			&      (200,2)                      		& NA          		& Adam           		& 0.02            \\ \hline
%VGCN BERT    		& 216                    			&   18              			&      (216,2)                      		& 16           		& Adam           		& 2e-5            \\ \hline
%Word2Vec     			& 300                   			&   2              			&      (300,2)                      		& 128           		& Adam          		& 0.001              \\ \hline
%GloVe        			& 300                    			&   2               			&      (300,2)                       	& 128           		& Adam       		& 0.001               \\ \hline
%\end{tabular}}
%\label{experimental_setting}
% \end{center}
%\end{table}
%
%\begin{table}[!htb]
%\caption{Epochs: Datasets}
%\begin{center}
%\begin{tabular}{|l|l|}
%\hline
%                      			& Epochs 		\\ \hline
%CoAID (Tweet)         	& 5     		 \\ \hline
%CoAID (Tweet + Reply) 	& 4     		 \\ \hline
%CoAID (News Articles) 	& 10     		\\ \hline
%CMU-MisCov19          	& 10     		\\ \hline
%\end{tabular}
%\label{epochs}
%\end{center}
%\end{table}
%

%\subsection{Results}

We describe the results obtained from five studies. We evaluate the performance of the models based on the accuracy, precision, recall, and f1 score. For each experiment, we average the results for 10 runs. The experiments are done using python's Scikit-learn \cite{scikit-learn} and TensorFlow 2.0 \cite{tensorflow2015-whitepaper} libraries. For training the Word2Vec model, we used the Gensim \cite{gensim} library. 

%The description is divided into two parts, based on two datasets, i.e., CoAID (for binary classification) and CMU-MisCov19 (for fine-grained classification).

%\subsection{Binary Classification: CoAID Dataset}


%Table \ref{CoAID-Tweet}, Table \ref{CoAID-Reply}, and Table \ref{CoAID-news} show the results from studies 1 and 2. 



%Table \ref{CoAID-Tweet} and Table \ref{CoAID-news} show the results from studies 1 and 2. 


\begin{table*}[!htb]
\caption{Study 1 \& 2: CoAID - Tweet (Temporal \& Text Length Dimension)}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.942} &
  \multicolumn{6}{c|}{Accuracy = 0.990} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{BERT}} &
  \multicolumn{1}{l|}{0.981} &
  0.997 &
  0.989 &
  0.281 &
  {\color[HTML]{000000} 0.079} &
  0.116 &
  \multicolumn{1}{l|}{0.946} &
  0.996 &
  0.970 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{1.00} &
  0.990 &
  0.995 &
  0.500 &
  1.00 &
  0.670 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.941} &
  \multicolumn{6}{c|}{Accuracy = 0.990} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{ELMo}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.945} &
  0.995 &
  0.970 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.990} &
  1.00 &
  0.995 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.932} &
  \multicolumn{6}{c|}{Accuracy = 0.969} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.949} &
  0.980 &
  0.964 &
  0.20 &
  0.09 &
  0.12 &
  \multicolumn{1}{l|}{0.99} &
  0.979 &
  0.984 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.943} &
  \multicolumn{6}{c|}{Accuracy = 1.00} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  0.31 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  0.998 &
  0.971 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{1.00} &
  1.00 &
  1.00 &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
   {\color[HTML]{FE0000} {\ul \textbf{1.00}}}  \\ \hline
\multicolumn{19}{|c|}{\textbf{DSPTMs - Graph-based}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.979} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Text GCN}} &
  \multicolumn{1}{l|}{0.979} &
  1.00 &
  0.989 &
  0.029 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.95 &
  1.00 &
  0.97 &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.99 &
  1.00 &
  0.99 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.971} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{VGCN-BERT}} &
  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  {\color[HTML]{FE0000} {\ul \textbf{0.495}}} &
  0.019 &
  0.035 &
  \multicolumn{1}{l|}{0.947} &
  0.999 &
  0.972 &
  {\color[HTML]{FE0000} {\ul \textbf{0.287}}} &
  0.029 &
  0.052 &
  \multicolumn{1}{l|}{0.994} &
  0.977 &
  0.984 &
  0.21 &
  0.389 &
  0.246 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSPTMs - Non-Graph}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.977} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.979} &
  0.997 &
  0.988 &
  0.11 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  1.00 &
  0.972 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.99} &
  1.00 &
  0.995 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.978} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.979} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.979} &
  0.999 &
  0.989 &
  0.23 &
  0.02 &
  0.03 &
  \multicolumn{1}{l|}{0.946} &
  1.00 &
  0.972 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.99} &
  0.99 &
  0.99 &
  0.00 &
  0.00 &
  0.00 \\ \hline
\end{tabular}}
\end{center}
\label{CoAID-Tweet}
\end{table*}







%\begin{table*}[!htb]
%\caption{Study 1: CoAID - Tweet}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|c|c|c|c|c|c|c|cc}
%\cline{1-7}
%\textbf{Train: May}                 & \multicolumn{2}{c|}{\textbf{Test: July}}                                                                                                                                                                                 & \multicolumn{2}{c|}{\textbf{Test: September}}                                                                                                                                                                            & \multicolumn{2}{c|}{\textbf{Test: November}}                                                                                                                                                                             &  &  \\ \cline{1-7}
%                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          &  &  \\ \cline{1-7}
%\multirow{2}{*}{BERT}      & \multicolumn{2}{c|}{Accuracy = 0.978}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.942}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.981\\ 0.997\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.281\\ 0.079\\ 0.116\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.946\\ 0.996\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}1.000\\ 0.990\\ 0.995\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.500\\ 1.000\\ 0.670\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{ELMo}      & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.941}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 1.000\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.945\\ 0.995\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 1.000\\ 0.995\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.932}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.969}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 1.000\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 0.980\\ 0.964\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.200\\ 0.090\\ 0.120\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 0.979\\ 0.984\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%GloVe                      & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.943}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 1.000}                                                                                                                                                                           &  &  \\ \cline{1-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.999\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.310\\ 0.020\\ 0.030\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.946\\ 0.998\\ 0.971\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}1.000\\ 1.000\\ 1.000\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}1.000\\ 1.000\\ 1.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Graph Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &  &  \\ \cline{1-7}
%\multirow{2}{*}{Text-GCN}  & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 1.000\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.029\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.950\\ 1.000\\ 0.970\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.990\\ 1.000\\ 0.990\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{VGCN-BERT} & \multicolumn{2}{c|}{Accuracy = 0.978}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.971}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.999\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.495\\ 0.019\\ 0.035\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.947\\ 0.999\\ 0.972\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.287\\ 0.029\\ 0.052\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.994\\ 0.977\\ 0.984\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.210\\ 0.389\\ 0.246\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Target Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.977}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.997\\ 0.988\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.110\\ 0.020\\ 0.030\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.946\\ 1.000\\ 0.972\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 1.000\\ 0.995\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{GloVe}     & \multicolumn{2}{c|}{Accuracy = 0.978}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.979}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.999\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.230\\ 0.020\\ 0.030\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.946\\ 1.000\\ 0.972\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 0.990\\ 0.990\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\end{tabular}}
%\end{center}
%\label{CoAID-Tweet}
%\end{table*}
%

%\end{tabular}
% \end{table}
% \label{coaid-tweet}
% }

%For the July tweet test dataset (Table \ref{CoAID-Tweet}), VGCN-BERT has the highest precision, and BERT has the highest recall and f1 scores that are slightly better than other models. For September, the Text-GCN has outstanding performance for detecting misinformation, but its performance on true information is extremely poor. In addition, other models perform poorly on misinformation. For November, the transfer learning approach GloVe has an excellent performance on both true information and misinformation, where precision, recall, and f1 scores are 1. Text-GCN also has decent scores on misinformation, and BERT performance on both true information and misinformation is also good. However, we notice that no model performs well across three different test datasets. This observation \textbf{confirms hypothesis 2}, i.e., transfer learning is not robust when there is context change happened in the data. It also \textbf{confirms hypothesis 5}, i.e., the hybrid method VGCN-BERT does not significantly improve the performance as compared to BERT and Text-GCN.

Table \ref{CoAID-Tweet} and Table \ref{CoAID-news} show the results from studies 1 and 2. For the July tweet test dataset (Table \ref{CoAID-Tweet}), VGCN-BERT has the highest precision, and BERT has the highest recall and f1 scores. These scores are slightly better than other models. For September, the Text-GCN has outstanding performance for detecting misinformation, but its performance on true information is extremely poor. In addition to this, other models perform poorly on misinformation. For November, the GloVe-based transfer learning approach achieves an excellent performance on both true information and misinformation, where precision, recall, and f1 scores are 1. Text-GCN also has decent scores on misinformation. The performance of BERT on both true information and misinformation is also good. However, we notice that no model performs well across three different test datasets. Thus we see that \textbf{mixed-domain transfer learning is not robust when context of the data changes}. 

%We also notice that the hybrid method VGCN-BERT does not significantly improve the performance as compared to BERT and Text-GCN.



%\begin{table}[!htb]
%\caption{Study 1: CoAID - Tweet\&Reply}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|c|c|c|c|c|c|c|cc}
%\cline{1-7}
%\textbf{Train: May}                 & \multicolumn{2}{c|}{\textbf{Test: July}}                                                                                                                                                                                 & \multicolumn{2}{c|}{\textbf{Test: September}}                                                                                                                                                                            & \multicolumn{2}{c|}{\textbf{Test: November}}                                                                                                                                                                             &  &  \\ \cline{1-7}
%                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          &  &  \\ \cline{1-7}
%\multirow{2}{*}{BERT}      & \multicolumn{2}{c|}{Accuracy = 0.962}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.941}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.937}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.978\\ 0.983\\ 0.981\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.101\\ 0.078\\ 0.089\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 0.991\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.033\\ 0.006\\ 0.010\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.939\\ 0.967\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.049\\ 0.500\\ 0.088\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{ELMo}      & \multicolumn{2}{c|}{Accuracy = 0.977}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.949}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.994}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.977\\ 1.000\\ 0.988\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 1.000\\ 0.974\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.994\\ 1.000\\ 0.997\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.964}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.919}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.951}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.984\\ 0.982\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.160\\ 0.130\\ 0.150\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.948\\ 0.968\\ 0.958\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.020\\ 0.020\\ 0.020\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.954\\ 0.975\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.060\\ 0.500\\ 0.110\end{tabular}                                         &  &  \\ \cline{1-7}
%GloVe                      & \multicolumn{2}{c|}{Accuracy = 0.965}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.939}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.915}                                                                                                                                                                           &  &  \\ \cline{1-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.981\\ 0.983\\ 0.982\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.230\\ 0.210\\ 0.220\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.951\\ 0.987\\ 0.969\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.160\\ 0.050\\ 0.070\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.918\\ 0.956\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.040\\ 0.500\\ 0.070\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Graph Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &  &  \\ \cline{1-7}
%\multirow{2}{*}{Text-GCN}  & \multicolumn{2}{c|}{Accuracy = 0.977}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.949}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.994}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.977\\ 1.000\\ 0.988\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 1.000\\ 0.974\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.994\\ 1.000\\ 0.997\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{VGCN-BERT} & \multicolumn{2}{c|}{Accuracy = 0.976}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.942}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.987}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.978\\ 0.998\\ 0.988\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.282\\ 0.039\\ 0.067\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.950\\ 0.991\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.115\\ 0.015\\ 0.022\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.995\\ 0.992\\ 0.993\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.111\\ 0.194\\ 0.134\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Target Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.972}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.939}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.975}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.977\\ 0.994\\ 0.986\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.070\\ 0.020\\ 0.030\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 0.989\\ 0.969\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.995\\ 0.979\\ 0.987\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.070\\ 0.250\\ 0.110\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{GloVe}     & \multicolumn{2}{c|}{Accuracy = 0.962}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.939}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.984}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.977\\ 0.984\\ 0.981\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.060\\ 0.040\\ 0.050\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.949\\ 0.989\\ 0.969\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.987\\ 0.992\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.180\\ 0.500\\ 0.270\end{tabular}                                         &  &  \\ \cline{1-7}
%\end{tabular}}
%\end{center}
%\label{CoAID-Reply}
%\end{table}


%Table \ref{CoAID-Reply} shows the result of the CoAID tweet and reply. For July, the transfer learning approach GloVe has the highest recall, and f1 scores for misinformation and VGCN-BERT has the highest precision. For September, the transfer learning approach GloVe has the highest precision, recall, and f1 scores for misinformation. For November, the transfer learning approaches BERT, GloVe, and Word2Vec as well as target-based approach GloVe has the highest recall score for misinformation. In addition, the target-based approach GloVe also has the highest precision and f1 score. However, there is \textbf{no single model that provides an effective solution for misinformation detection for all three different test datasets}. This result \textbf{confirms hypothesis 2}, i.e., the transfer learning approaches do not improve the performance significantly after we increase the training size. It also further \textbf{confirms hypothesis 5}, i.e., the hybrid method VGCN-BERT is slightly better than that of both BERT and Text-GCN for misinformation classification.






\begin{table*}[!htb]
\caption{Study 1 \& 2: CoAID - News Articles (Temporal \& Text Length Dimension))}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.646} &
  \multicolumn{6}{c|}{Accuracy = 0.503} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{BERT}} &
  \multicolumn{1}{l|}{0.814} &
  1.00 &
  0.898 &
  0.00 &
  {\color[HTML]{000000} 0.00} &
  0.00 &
  \multicolumn{1}{l|}{0.929} &
  0.676 &
  0.779 &
  0.018 &
  0.135 &
  0.036 &
  \multicolumn{1}{l|}{0.962} &
  0.511 &
  0.656 &
  0.009 &
  0.144 &
  0.009 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.559} &
  \multicolumn{6}{c|}{Accuracy = 0.973} &
  \multicolumn{6}{c|}{Accuracy = 0.985} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{ELMo}} &
  \multicolumn{1}{l|}{0.777} &
  0.642 &
  0.703 &
  0.11 &
  0.19 &
  0.14 &
  \multicolumn{1}{l|}{0.979} &
  0.993 &
  0.986 &
  {\color[HTML]{FE0000} {\ul \textbf{0.83}}} &
  0.64 &
  {\color[HTML]{FE0000} {\ul \textbf{0.72}}} &
  \multicolumn{1}{l|}{0.986} &
  0.99 &
  0.992 &
  0.88 &
  0.37 &
  0.52 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.851} &
  \multicolumn{6}{c|}{Accuracy = 0.946} &
  \multicolumn{6}{c|}{Accuracy = 0.98} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.846} &
  0.999 &
  0.916 &
  0.98 &
  0.20 &
  0.33 &
  \multicolumn{1}{l|}{0.948} &
  0.998 &
  0.972 &
  0.60 &
  0.06 &
  0.12 &
  \multicolumn{1}{l|}{0.98} &
  1.00 &
  0.99 &
  1.00 &
  0.11 &
  0.19 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.599} &
  \multicolumn{6}{c|}{Accuracy = 0.953} &
  \multicolumn{6}{c|}{Accuracy = 0.984} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.833} &
  0.635 &
  0.721 &
  0.22 &
  0.44 &
  0.29 &
  \multicolumn{1}{l|}{0.957} &
  0.995 &
  0.975 &
  0.73 &
  0.23 &
  0.35 &
  \multicolumn{1}{l|}{0.985} &
  0.999 &
  0.992 &
  {\color[HTML]{000000} 0.86} &
  {\color[HTML]{000000} 0.32} &
  0.46 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSPTMs - Graph-based}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.635} &
  \multicolumn{6}{c|}{Accuracy = 0.978} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Text GCN}} &
  \multicolumn{1}{l|}{0.00} &
  0.00 &
  0.00 &
  0.81 &
  1.00 &
  0.90 &
  \multicolumn{1}{l|}{0.97} &
  0.633 &
  0.766 &
  0.095 &
  0.66 &
  0.165 &
  \multicolumn{1}{l|}{0.978} &
  1.00 &
  0.989 &
  0.00 &
  0.00 &
  0.00 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.677} &
  \multicolumn{6}{c|}{Accuracy = 0.64} &
  \multicolumn{6}{c|}{Accuracy = 0.458} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{VGCN-BERT}} &
  \multicolumn{1}{l|}{0.971} &
  0.622 &
  0.758 &
  {\color[HTML]{000000} 0.356} &
  0.917 &
  0.513 &
  \multicolumn{1}{l|}{0.985} &
  0.628 &
  0.767 &
  {\color[HTML]{000000} 0.117} &
  0.839 &
  0.205 &
  \multicolumn{1}{l|}{0.989} &
  0.451 &
  0.619 &
  0.031 &
  0.778 &
  0.06 \\ \hline
\multicolumn{19}{|c|}{\textbf{DSPTMs - Non-Graph}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.96} &
  \multicolumn{6}{c|}{Accuracy = 0.643} &
  \multicolumn{6}{c|}{Accuracy = 0.99} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{Word2Vec}} &
  \multicolumn{1}{l|}{0.957} &
  0.984 &
  0.975 &
  {\color[HTML]{FE0000} {\ul \textbf{0.92}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.85}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.89}}} &
  \multicolumn{1}{l|}{0.977} &
  0.638 &
  0.772 &
  0.11 &
  {\color[HTML]{FE0000} {\ul \textbf{0.74}}} &
  0.19 &
  \multicolumn{1}{l|}{0.991} &
  0.99 &
  0.995 &
  {\color[HTML]{FE0000} {\ul \textbf{0.92}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.58}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.71}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.554} &
  \multicolumn{6}{c|}{Accuracy = 0.623} &
  \multicolumn{6}{c|}{Accuracy = 0.452} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{GloVe}} &
  \multicolumn{1}{l|}{0.775} &
  0.637 &
  0.699 &
  0.10 &
  0.19 &
  0.13 &
  \multicolumn{1}{l|}{0.941} &
  0.641 &
  0.763 &
  0.05 &
  0.32 &
  0.09 &
  \multicolumn{1}{l|}{0.962} &
  0.457 &
  0.62 &
  0.01 &
  0.21 &
  0.02 \\ \hline
\end{tabular}}
\end{center}
\label{CoAID-news}
\end{table*}










%\begin{table*}[!htb]
%\caption{Study 1: CoAID - News Articles}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|c|c|c|c|c|c|c|cc}
%\cline{1-7}
%\textbf{Train: May}                 & \multicolumn{2}{c|}{\textbf{Test: July}}                                                                                                                                                                                 & \multicolumn{2}{c|}{\textbf{Test: September}}                                                                                                                                                                            & \multicolumn{2}{c|}{\textbf{Test: November}}                                                                                                                                                                             &  &  \\ \cline{1-7}
%                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          &  &  \\ \cline{1-7}
%\multirow{2}{*}{BERT}      & \multicolumn{2}{c|}{Accuracy = 0.814}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.646}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.503}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.814\\ 1.000\\ 0.898\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.929\\ 0.676\\ 0.779\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.018\\ 0.135\\ 0.036\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.962\\ 0.511\\ 0.656\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.009\\ 0.144\\ 0.009\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{ELMo}      & \multicolumn{2}{c|}{Accuracy = 0.559}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.973}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.985}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.777\\ 0.642\\ 0.703\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.110\\ 0.190\\ 0.140\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.979\\ 0.993\\ 0.986\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.830\\ 0.640\\ 0.720\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.986\\ 0.999\\ 0.992\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.880\\ 0.370\\ 0.520\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.851}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.946}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.980}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.846\\ 0.999\\ 0.916\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.980\\ 0.200\\ 0.330\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.948\\ 0.998\\ 0.972\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.600\\ 0.060\\ 0.120\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.980\\ 1.000\\ 0.990\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}1.000\\ 0.110\\ 0.190\end{tabular}                                         &  &  \\ \cline{1-7}
%GloVe                      & \multicolumn{2}{c|}{Accuracy = 0.599}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.953}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.984}                                                                                                                                                                           &  &  \\ \cline{1-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.833\\ 0.635\\ 0.721\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.220\\ 0.440\\ 0.290\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.957\\ 0.995\\ 0.975\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.730\\ 0.230\\ 0.350\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.985\\ 0.999\\ 0.992\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.860\\ 0.320\\ 0.460\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Graph Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                &  &  \\ \cline{1-7}
%\multirow{2}{*}{Text-GCN}  & \multicolumn{2}{c|}{Accuracy = 0.814}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.635}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.978}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.810\\ 1.000\\ 0.900\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.970\\ 0.633\\ 0.766\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.095\\ 0.660\\ 0.165\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.978\\ 1.000\\ 0.989\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{VGCN-BERT} & \multicolumn{2}{c|}{Accuracy = 0.677}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.640}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.458}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.971\\ 0.622\\ 0.758\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.356\\ 0.917\\ 0.513\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.985\\ 0.628\\ 0.767\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.117\\ 0.839\\ 0.205\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.989\\ 0.451\\ 0.619\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.031\\ 0.778\\ 0.060\end{tabular}                                         &  &  \\ \cline{1-7}
%\multicolumn{7}{|c|}{\textbf{Target Based}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               &  &  \\ \cline{1-7}
%\multirow{2}{*}{Word2Vec}  & \multicolumn{2}{c|}{Accuracy = 0.960}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.643}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.990}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.957\\ 0.984\\ 0.975\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.920\\ 0.850\\ 0.890\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.977\\ 0.638\\ 0.772\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.110\\ 0.740\\ 0.190\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.991\\ 0.999\\ 0.995\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.920\\ 0.580\\ 0.710\end{tabular}                                         &  &  \\ \cline{1-7}
%\multirow{2}{*}{GloVe}     & \multicolumn{2}{c|}{Accuracy = 0.554}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.623}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.452}                                                                                                                                                                           &  &  \\ \cline{2-7}
%                           & \begin{tabular}[c]{@{}c@{}}0.775\\ 0.637\\ 0.699\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.100\\ 0.190\\ 0.130\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.941\\ 0.641\\ 0.763\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.050\\ 0.320\\ 0.090\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.962\\ 0.457\\ 0.620\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.010\\ 0.210\\ 0.020\end{tabular}                                         &  &  \\ \cline{1-7}
%\end{tabular}}
%\end{center}
%\label{CoAID-news}
%\end{table*}


%Table \ref{CoAID-news} shows the result of CoAID news articles. For the July test dataset, both Text-GCN and target-based Word2Vec achieve decent precision, recall, and f1 scores on misinformation. However, Text-GCN has extremely poor performance on true information. For September, ELMo has the best precision and f1 score, while target based Word2Vec has the best recall score. As for November, both transfer learning and target-based Word2Vec obtain optimal precision score and Word2Vec also has the highest f1 score. Besides, VGCN-BERT has the highest recall score. We notice that target-based Word2Vec achieves overall high performance across all test datasets. This result \textbf{confirms hypothesis 6}, i.e., target-based embeddings can capture both global and local relationships to create an effective classifier. It also \textbf{confirms hypothesis 4}, i.e., the performance of graph-based approaches on lengthy texts is not as good as on short texts.  


Table \ref{CoAID-news} shows the result of CoAID news articles. For the July test dataset, both Text-GCN and target-based Word2Vec (DSPTM-based) achieve decent precision, recall, and f1 scores on misinformation. However, Text-GCN has extremely poor performance on true information. For September, ELMo has the best precision and f1 score, while Word2Vec (DSPTM-based) has the best recall score. As for November, both transfer learning and DSPTM-based Word2Vec obtain optimal precision score, and Word2Vec (DSPTM-based) has the highest f1 score. Besides, VGCN-BERT has the highest recall score. We notice that the DSPTM-based Word2Vec achieves overall high performance across all test datasets. Thus, the \textbf{non-graph DSPTM-based embeddings can capture both global and local relationships to create an effective classifier}. The performance of the graph-based DSPTM approach on lengthy texts is not as good as on short texts.  



\begin{table*}[!htb]
\caption{Study 3: CoAID Large Dataset (Dataset Size Dimension)}
\begin{center}
\scalebox{0.66}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train: May + July + September\\ Test: November\end{tabular}}} &
  \multicolumn{6}{c|}{\textbf{Tweet}} &
  \multicolumn{6}{c|}{\textbf{News Articles}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.928} &
  \multicolumn{6}{c|}{Accuracy = 0.992} \\ \cline{2-13} 
\multirow{-2}{*}{\textbf{Mixed-Domain Transfer Learning: BERT}} &
  \multicolumn{1}{l|}{1.00} &
  0.927 &
  0.962 &
  0.12 &
  {\color[HTML]{FE0000} {\ul \textbf{1.00}}} &
  0.22 &
  \multicolumn{1}{l|}{0.994} &
  0.998 &
  0.996 &
  {\color[HTML]{FE0000} {\ul \textbf{0.883}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.719}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.787}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.985} &
  \multicolumn{6}{c|}{Accuracy = 0.986} \\ \cline{2-13} 
\multirow{-2}{*}{\textbf{DSPTMs - Non-Graph: Word2Vec}} &
  \multicolumn{1}{l|}{0.99} &
  0.995 &
  0.992 &
  {\color[HTML]{FE0000} {\ul \textbf{0.71}}} &
  {\color[HTML]{000000} 0.63} &
  {\color[HTML]{FE0000} {\ul \textbf{0.67}}} &
  \multicolumn{1}{l|}{0.992} &
  0.994 &
  0.993 &
  {\color[HTML]{000000} 0.71} &
  0.63 &
  {\color[HTML]{000000} 0.67} \\ \hline
\end{tabular}}
\end{center}
\label{CoAID-Big}
\end{table*}




%
%\begin{table*}[!htb]
%\caption{CoAID Large Dataset Experiment Result}
%\begin{center}
%\scalebox{0.56}{
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Train:} \\\textbf{May + July + September} \\ \textbf{Test: November}\end{tabular}} & \multicolumn{2}{c|}{\textbf{Tweet}}                                                                                                                                                                                      & \multicolumn{2}{c|}{\textbf{Tweet + Reply}}                                                                                                                                                                              & \multicolumn{2}{c|}{\textbf{News Articles}}                                                                                                                                                                              \\ \hline
%\multicolumn{1}{|l|}{}                                                                                      & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} \\ \hline
%\multicolumn{7}{|l|}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
%\multirow{2}{*}{BERT}                                                                                       & \multicolumn{2}{c|}{Accuracy = 0.928}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.981}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.992}                                                                                                                                                                           \\ \cline{2-7} 
%                                                                                                            & \begin{tabular}[c]{@{}c@{}}1.000\\ 0.927\\ 0.962\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.120\\ 1.000\\ 0.220\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.990\\ 0.990\\ 0.990\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.789\\ 0.764\\ 0.773\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.994\\ 0.998\\ 0.996\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.883\\ 0.719\\ 0.787\end{tabular}                                         \\ \hline
%\multirow{2}{*}{Word2Vec (Target Based)}                                                                    & \multicolumn{2}{c|}{Accuracy = 0.985}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.961}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.986}                                                                                                                                                                           \\ \cline{2-7} 
%                                                                                                            & \begin{tabular}[c]{@{}c@{}}0.990\\ 0.995\\ 0.992\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.710\\ 0.630\\ 0.670\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.997\\ 0.964\\ 0.980\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.710\\ 0.630\\ 0.670\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.992\\ 0.994\\ 0.993\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.710\\ 0.630\\ 0.670\end{tabular}                                         \\ \hline
%\end{tabular}}
%\end{center}
%\label{CoAID-Big}
%\end{table*}


%Table \ref{CoAID-Big} shows the results of large-dataset-based experiments. The performance of target-based Word2Vec further \textbf{confirms hypothesis 6}, i.e., the target-based text embeddings capture both global and local relationships if we increase the size of short-length training data (i.e., tweets). Its scores on misinformation for tweet or tweet and reply datasets increase significantly. 

Table \ref{CoAID-Big} shows the results of study 3, i.e., large-dataset-based experiments. The performance of DSPTM-based Word2Vec endorses the previous observation, i.e., \textbf{the non-graph DSPTM-based text embeddings capture both global and local relationships if we increase the size of short-length training data (i.e., tweets)}. Its F1 score on misinformation for tweet dataset increases significantly. 





\begin{table*}[!htb]
\caption{Study 4: CoAID Large Dataset (Various Transformer Models)}
\begin{center}
\scalebox{0.6}{
\begin{tabular}{|l|c|l|l|l|l|l|c|l|l|l|l|l|c|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Train: May}} &
  \multicolumn{6}{c|}{\textbf{Test: July}} &
  \multicolumn{6}{c|}{\textbf{Test: September}} &
  \multicolumn{6}{c|}{\textbf{Test: November}} \\ \hline
\textbf{Model} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} &
  \multicolumn{3}{c|}{\textbf{True Information}} &
  \multicolumn{3}{c|}{\textbf{Misinformation}} \\ \hline
 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 &
  \multicolumn{1}{l|}{P} &
  R &
  F1 &
  P &
  R &
  F1 \\ \hline
\multicolumn{19}{|c|}{\textbf{Mixed-Domain Transfer Learning}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.611} &
  \multicolumn{6}{c|}{Accuracy = 0.943} &
  \multicolumn{6}{c|}{Accuracy = 0.993} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{ALBERT}} &
  \multicolumn{1}{l|}{0.858} &
  0.625 &
  0.723 &
  0.25 &
  {\color[HTML]{000000} 0.547} &
  0.343 &
  \multicolumn{1}{l|}{0.96} &
  0.981 &
  0.97 &
  0.483 &
  0.298 &
  0.368 &
  \multicolumn{1}{l|}{0.996} &
  0.996 &
  0.996 &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.842}}} \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.936} &
  \multicolumn{6}{c|}{Accuracy = 0.630} &
  \multicolumn{6}{c|}{Accuracy = 0.980} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{RoBERTa}} &
  \multicolumn{1}{l|}{0.937} &
  0.987 &
  0.962 &
  {\color[HTML]{FE0000} {\ul \textbf{0.925}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.711}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.804}}} &
  \multicolumn{1}{l|}{0.952} &
  0.641 &
  0.766 &
  {\color[HTML]{000000} 0.068} &
  0.447 &
  {\color[HTML]{000000} 0.118} &
  \multicolumn{1}{l|}{0.991} &
  0.989 &
  0.990 &
  0.55 &
  0.579 &
  0.564 \\ \hline
 &
  \multicolumn{6}{c|}{Accuracy = 0.814} &
  \multicolumn{6}{c|}{Accuracy = 0.97} &
  \multicolumn{6}{c|}{Accuracy = 0.456} \\ \cline{2-19} 
\multirow{-2}{*}{\textbf{XLNET}} &
  \multicolumn{1}{l|}{0.81} &
  1.00 &
  0.90 &
  0.00 &
  0.00 &
  0.00 &
  \multicolumn{1}{l|}{0.97} &
  1.00 &
  0.98 &
  {\color[HTML]{FE0000} {\ul \textbf{0.89}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.53}}} &
  {\color[HTML]{FE0000} {\ul \textbf{0.67}}} &
  \multicolumn{1}{l|}{0.97} &
  0.46 &
  0.62 &
  0.01 &
  0.26 &
  0.02 \\ \hline
\end{tabular}}
\end{center}
\label{CoAID-bert-variants}
\end{table*}

%\begin{table*}[!htb]
%\caption{CoAID - News Articles Using Variants of BERT and Transformer}
%\begin{center}
%\scalebox{0.6}{
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\multicolumn{1}{|l|}{\textbf{Train: May}} & \multicolumn{2}{c|}{\textbf{Test: July}}                                                                                                                                                                                 & \multicolumn{2}{c|}{\textbf{Test: September}}                                                                                                                                                                            & \multicolumn{2}{c|}{\textbf{Test: November}}                                                                                                                                                                             \\ \hline
%\multicolumn{1}{|l|}{}           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}True Information\\ Precision\\ Recall\\ F1\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Misinformation\\ Precision\\ Recall\\ F1\end{tabular}} \\ \hline
%\multicolumn{7}{|c|}{\textbf{Transfer Learning}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
%\multirow{2}{*}{ALBERT}          & \multicolumn{2}{c|}{Accuracy = 0.611}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.943}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.993}                                                                                                                                                                           \\ \cline{2-7} 
%                                 & \begin{tabular}[c]{@{}c@{}}0.858\\ 0.625\\ 0.723\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.250\\ 0.547\\ 0.343\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.960\\ 0.981\\ 0.970\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.483\\ 0.298\\ 0.368\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.996\\ 0.996\\ 0.996\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.842\\ 0.842\\ 0.842\end{tabular}                                         \\ \hline
%\multirow{2}{*}{RoBERTa}         & \multicolumn{2}{c|}{Accuracy = 0.936}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.630}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.980}                                                                                                                                                                           \\ \cline{2-7} 
%                                 & \begin{tabular}[c]{@{}c@{}}0.937\\ 0.987\\ 0.962\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.925\\ 0.711\\ 0.804\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.952\\ 0.641\\ 0.766\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.068\\ 0.447\\ 0.118\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.991\\ 0.989\\ 0.990\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.550\\ 0.579\\ 0.564\end{tabular}                                         \\ \hline
%\multirow{2}{*}{XLNET}           & \multicolumn{2}{c|}{Accuracy = 0.814}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.970}                                                                                                                                                                           & \multicolumn{2}{c|}{Accuracy = 0.456}                                                                                                                                                                           \\ \cline{2-7} 
%                                 & \begin{tabular}[c]{@{}c@{}}0.810\\ 1.000\\ 0.900\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.000\\ 0.000\\ 0.000\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.970\\ 1.000\\ 0.980\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.890\\ 0.530\\ 0.670\end{tabular}                                         & \begin{tabular}[c]{@{}c@{}}0.970\\ 0.460\\ 0.620\end{tabular}                                           & \begin{tabular}[c]{@{}c@{}}0.010\\ 0.260\\ 0.020\end{tabular}                                         \\ \hline
%\end{tabular}}
%\end{center}
%\label{CoAID-bert-variants}
%\end{table*}

Table \ref{CoAID-bert-variants} shows the results obtained from study 4. For the July test dataset misinformation detection, RoBERTa achieves the best performance, while XLNet shows the worst performance. However, for September misinformation, XLNet obtains the best performance, while the RoBERTa has the worst performance. As for November misinformation, ALBERT achieves the best performance, while XLNet has the worst performance. These results corroborate our previous observation on the mixed-domain transfer learning approach, i.e., it is not robust when context of the data changes. 


%These results \textbf{confirm hypothesis 2} because none of these models maintain the performance when the context in the data changes.




\subsubsection{Result: Fine-Grained CMU-MisCov19 Dataset}
\begin{figure*}[h]
  \centering
  %\includegraphics[width=\linewidth]{figures/cmu-result-graph.png}
  \includegraphics[width=4.5in]{figures/cmu-result-graph.png}
  \caption{Study 5: CMU-MisCov19 (Fine-Grained Classification)}
  \label{fig:cmu-graph}
\end{figure*}

%Figure \ref{fig:cmu-graph} shows the results obtained from study 3. The result \textbf{confirms hypotheses 3 and 6}. Specifically, all the transfer learning approaches perform poorly, but the target-based Word2Vec achieves the best performance.

Figure \ref{fig:cmu-graph} shows the results obtained from study 5. We see that the mixed-domain transfer learning approach performs poorly. The best performing model is the DSPTM-based Word2Vec. 


\subsection{Analysis}

Based on the results given in the above tables, we summarize our observations below. First, we discuss a model's generalizability for binary classification scenarios. Given the length of the text and the size of the dataset, we identify 4 cases.

\begin{itemize}
    \item Case 1: Length: Short \& Size: Small
    \item Case 2: Length: Long \& Size: Small
    \item Case 3: Length: Short \& Size: Large
    \item Case 4: Length: Long \& Size: Large
\end{itemize}



\paragraph{Case 1: Length: Short \& Size: Small}

For case 1 we do not find a single best-performing model. For the tweet dataset, following models perform slightly better: VGCN-BERT, GloVe (transfer learning and DSPTM-based), and Text GCN. There are two possible explanations for the poor performance of all models on the short-length tweet data. First, the number of test misinformation samples is significantly smaller. Second, the short length of the text (tweet and tweet+reply) and the small size of the training set might have influenced the context learning of the models. None of the models seem to have captured the context of the text well enough to make accurate predictions. 
    




%Table \ref{summary} shows that for the tweet and tweet+replies datasets following models perform slightly better: VGCN-BERT, GloVe (transfer learning and target based), and Text GCN.




%\begin{table*}[!htb]
%\caption{Effective Models: Binary Classification \\ *Performance measures are shown only for the misinformation class}
%\begin{center}
%\scalebox{0.8}{
%\begin{tabular}{|l|l|l|l|l|l|l|}
%\hline
%\textbf{} & \multicolumn{2}{l|}{\textbf{Test: July}} & \multicolumn{2}{l|}{\textbf{Test: September}} & \multicolumn{2}{l|}{\textbf{Test: November}} \\ \hline
%\textbf{} & \textbf{Precision}   & \textbf{Recall}   & \textbf{Precision}      & \textbf{Recall}     & \textbf{Precision}     & \textbf{Recall}     \\ \hline
%\multicolumn{7}{|c|}{\textbf{Tweets}}                                         \\ \hline
%\textbf{VGCN-BERT}                 & 0.49 & 0.019 & 0.287  & 0.029 &0.21      &0.389      \\ \hline
%\textbf{GloVe (Transfer Learning)} & 0.31 & 0.02  & 0.00&0.00      &1.00      &1.00      \\ \hline
%\textbf{Text GCN}                  & 0.029  & 0.00       & 0.95 & 1.00 & 0.99 & 1.00 \\ \hline
%\multicolumn{7}{|c|}{\textbf{Tweets + Replies}}                               \\ \hline
%\textbf{GloVe (Transfer Learning)} & 0.23 & 0.21  & 0.16 & 0.05 & 0.04 & 0.50 \\ \hline
%\textbf{GloVe}                     & 0.06     &0.04       &0.00      &0.00      & 0.18 & 0.50 \\ \hline
%\multicolumn{7}{|c|}{\textbf{News Articles}}                                  \\ \hline
%\textbf{Word2Vec}                  & 0.92 & 0.85  & 0.11 & 0.74 & 0.92 & 0.58 \\ \hline
%\textbf{ELMo (Transfer Learning)}  &0.11      &0.19       & 0.83 & 0.64 & 0.88 & 0.37 \\ \hline
%\end{tabular}}
%\end{center}
%%\label{summary}
%\end{table*}


%There are two possible explanations for the poor performance of all models on the short-length tweet data. 
%
%\begin{itemize}
%    \item \textbf{Small Size of Misinformation Test Set:} The number of test misinformation samples is significantly smaller. For example, in the 2020 July, September, and November Tweet test datasets the true information samples are larger than the misinformation samples by 46, 17, and 96 times, respectively. Both for the tweet and tweet+reply November subsets we have only 2 samples of misinformation. This might have caused low precision and recall for misinformation class.
%    
%    \item \textbf{Short Text Length \& Small Trained Dataset:} The short length of the text (tweet and tweet+reply) and the small size of the training set might have influenced the context learning of the models. None of the models seem to have captured the context of the text well enough to make accurate predictions. 
%    
%\end{itemize}


\paragraph{Case 2: Length: Long \& Size: Small}

For the news articles data, the best model is DSPTM-based Word2Vec for the July and November dataset. Both models achieved higher precision and recall on the misinformation class. For the September dataset, the ELMo outperforms DSPTM-based Word2Vec.

\paragraph{Case 3: Length: Short \& Size: Large}

For this case, both DSPTM-based Word2Vec and BERT-based transfer learning perform well. However, BERT's performance is not consistent. On the Tweet dataset (short-length text), the precision of BERT is poor. It indicates that even with larger training data BERT-based transfer learning does not provide an effective solution for short-length samples. One possible reason is that although the BERT model is good at capturing the local relationship (e.g., word order), it does not do equally well on capturing the global relationship or context from short-length data.



\paragraph{Case 4: Length: Long \& Size: Large}

Both DSPTM-based Word2Vec and BERT-based transfer learning perform well in this case. However, BERT's performance is slightly better.


The results from fine-grained classification show that DSPTM-based Word2Vec is the clear winner. It outperforms other approaches by a large margin.

\noindent Based on the insights garnered from the above analyses, we draw the following conclusions, summarized in Figure \ref{fig:framework}.
\begin{itemize}
   

    \item The \textbf{mixed-domain transfer learning} approach with the BERT SOTA model is effective in limited cases. Also, its performance is not consistent.
    
    \item The \textbf{graph-based DSPTM} approach does not yield an effective solution in any of the cases. The VGCN-BERT that combines the benefits of Text GCN with BERT is not effective either.
    
    %\item The \textbf{hybrid} approach that combines BERT embeddings with graph embeddings is not effective either.
    
     \item The \textbf{non-graph DSPTM-based} approach with the Word2Vec model generalizes well across the last three cases.
    
\end{itemize}


%Thus, there is no single generalizable approach for identifying COVID-19 social media misinformation. The choice of an effective approach is dependent on the length of the text, size of the dataset, and the distribution of the classes. 
%
%
%We use these insights to propose a generalizable framework.
%
%
%
%Figure \ref{fig:framework} illustrates our framework. The framework includes recommendations for two types of classification: binary and fine-grained. For a binary classification problem, the framework uses the data from two dimensions: length of the text and size of the dataset.
%
%\begin{itemize}
%    \item Length Short + Small Dataset: Graph-based methods such as Text GCN and transfer learning method based on pretrained GloVe embeddings
%    
%    \item Length Long + Small Dataset: Target-based Word2Vec embedding with a CNN classifier
%    
%    \item Length Short and Long + Large Dataset: Target-based Word2Vec embedding with a CNN classifier and transfer learning using BERT
%    
%    
%\end{itemize}
%
%We do not observe a single best-performing model on the short length and small size dataset. Thus, our framework makes a weak recommendation on this type of data.
%
%For the fine-grained data, the best model is the Target-based Word2Vec embedding with CNN classifier.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=\linewidth]{figures/Framework.png}
  \caption{Framework for Misinformation Detection}
  \label{fig:framework}
\end{figure}



